HAT-P-44b, HAT-P-45b, and HAT-P-46b: Three Transiting Hot Jupiters in Possible Multi-Planet Systems

We report the discovery by the HATNet survey of three new transiting extrasolar planets orbiting moderately bright (V=13.2, 12.8 and 11.9) stars. The planets have orbital periods of 4.3012, 3.1290, and 4.4631 days, masses of 0.39, 0.89, and 0.49 Mjup, and radii of 1.28, 1.43, and 1.28 Rjup. The stellar hosts have masses of 0.94, 1.26, and 1.28 Msun. Each system shows significant systematic variations in its residual radial velocities indicating the possible presence of additional components. Based on its Bayesian evidence, the preferred model for HAT-P-44 consists of two planets, including the transiting component, with the outer planet having a period of 220 d and a minimum mass of 1.6 Mjup. Due to aliasing we cannot rule out an alternative solution for the outer planet having a period of 438 d and a minimum mass of 3.7 Mjup. For HAT-P-45 at present there is not enough data to justify the additional free parameters included in a multi-planet model, in this case a single-planet solution is preferred, but the required jitter of 22.5 +- 6.3 m/s is relatively high for a star of this type. For HAT-P-46 the preferred solution includes a second planet having a period of 78 d and a minimum mass of 2.0 Mjup, however the preference for this model over a single-planet model is not very strong. While substantial uncertainties remain as to the presence and/or properties of the outer planetary companions in these systems, the inner transiting planets are well characterized with measured properties that are fairly robust against changes in the assumed models for the outer planets. Continued RV monitoring is necessary to fully characterize these three planetary systems, the properties of which may have important implications for understanding the formation of hot Jupiters.

==> HTR146-002.mod8.tex <==
\newcommand{\hatcurhtrxxxxAmH}{HTR146-002}                             % Original HTR name of target
\newcommand{\hatcurfieldxxxxAmH}{146}                                  % Original HTR field
\newcommand{\hatcurCCraxxxxAmH}{\ensuremath{14^{\mathrm h}12^{\mathrm m}34.56{\mathrm s}}}                           % Right Ascension
\newcommand{\hatcurCCdecxxxxAmH}{\ensuremath{+47{\arcdeg}00{\arcmin}52.9{\arcsec}}}                          % Declination
\newcommand{\hatcurCCmagxxxxAmH}{13.212}                               % apparent V-band magnitude
\newcommand{\hatcurCCtwomassxxxxAmH}{2MASS~14123457+4700528}           % 2MASS identifier
\newcommand{\hatcurCCgscxxxxAmH}{GSC~3465-00123}                       % GSC(1.2) identifier
\newcommand{\hatcurCCtassmvxxxxAmH}{13.212}                            % TASS V-band magnitude
%% --------------------------------------------------------------------
\newcommand{\hatcurCCtwomassJmagxxxxAmH}{\ensuremath{11.729\pm0.021}}  % 2MASS ORIG MAG
\newcommand{\hatcurCCtwomassHmagxxxxAmH}{\ensuremath{11.360\pm0.019}}  % 2MASS ORIG MAG
\newcommand{\hatcurCCtwomassKmagxxxxAmH}{\ensuremath{11.275\pm0.018}}  % 2MASS ORIG MAG
\newcommand{\hatcurCCcitJmagxxxxAmH}{\ensuremath{11.741\pm0.022}}      % 2MASS CIT MAG
\newcommand{\hatcurCCcitHmagxxxxAmH}{\ensuremath{11.354\pm0.020}}      % 2MASS CIT MAG
\newcommand{\hatcurCCcitKmagxxxxAmH}{\ensuremath{11.299\pm0.018}}      % 2MASS CIT MAG
\newcommand{\hatcurCCbbJmagxxxxAmH}{\ensuremath{11.797\pm0.023}}       % 2MASS BB MAG
\newcommand{\hatcurCCbbHmagxxxxAmH}{\ensuremath{11.376\pm0.020}}       % 2MASS BB MAG
\newcommand{\hatcurCCbbKmagxxxxAmH}{\ensuremath{11.319\pm0.018}}       % 2MASS BB MAG
\newcommand{\hatcurCCesoJmagxxxxAmH}{\ensuremath{11.801\pm0.025}}      % 2MASS ESO MAG
\newcommand{\hatcurCCesoHmagxxxxAmH}{\ensuremath{11.371\pm0.024}}      % 2MASS ESO MAG
\newcommand{\hatcurCCesoKmagxxxxAmH}{\ensuremath{11.318\pm0.019}}      % 2MASS ESO MAG
\newcommand{\hatcurCCesoJHmagxxxxAmH}{\ensuremath{0.429\pm0.032}}      % 2MASS ESO JH COLOR
\newcommand{\hatcurCCesoJKmagxxxxAmH}{\ensuremath{0.484\pm0.031}}      % 2MASS ESO JK COLOR
\newcommand{\hatcurCCesoHKmagxxxxAmH}{\ensuremath{0.054\pm0.030}}      % 2MASS ESO HK COLOR
%% --------------------------------------------------------------------
\newcommand{\hatcurLCdipxxxxAmH}{\ensuremath{22.0}}                    % BLS detected dip (mmag)
\newcommand{\hatcurLCrprstarxxxxAmH}{\ensuremath{0.1338\pm0.0005}}     % Rp/R*
\newcommand{\hatcurLCbsqxxxxAmH}{\ensuremath{0.015_{-0.009}^{+0.027}}} % impact parameter square
\newcommand{\hatcurLCimpxxxxAmH}{\ensuremath{0.122_{-0.051}^{+0.072}}} % impact parameter
\newcommand{\hatcurLCzetaxxxxAmH}{\ensuremath{17.48\pm0.04}}           % zeta/R*
\newcommand{\hatcurLCdurxxxxAmH}{\ensuremath{0.1300\pm0.0004}}         % transit duration (days)
\newcommand{\hatcurLCdurshortxxxxAmH}{\ensuremath{0.1300}}             % transit duration (days)
\newcommand{\hatcurLCdurhrxxxxAmH}{\ensuremath{3.119\pm0.008}}         % transit duration (hours)
\newcommand{\hatcurLCdurhrshortxxxxAmH}{\ensuremath{3.119}}            % transit duration (hours)
\newcommand{\hatcurLCqxxxxAmH}{\ensuremath{0.0302\pm0.0001}}           % fractional transit duration (days)
\newcommand{\hatcurLCqshortxxxxAmH}{\ensuremath{0.030}}                % fractional transit duration (days)
\newcommand{\hatcurLCingdurxxxxAmH}{\ensuremath{0.0155\pm0.0004}}      % ingress/egress duration (days)
\newcommand{\hatcurLCPxxxxAmH}{\ensuremath{4.301212\pm0.000007}}       % period (days)
\newcommand{\hatcurLCPprecxxxxAmH}{\ensuremath{4.3012125}}             % period (days)
\newcommand{\hatcurLCPshortxxxxAmH}{\ensuremath{4.3012}}               % period (days)
\newcommand{\hatcurLCTxxxxAmH}{\ensuremath{2455696.93691\pm0.00012}}   % epoch (BJD)
\newcommand{\hatcurLCTAxxxxAmH}{\ensuremath{2455322.73142\pm0.00059}}  % TA (BJD)
\newcommand{\hatcurLCTBxxxxAmH}{\ensuremath{2455709.84054\pm0.00012}}  % TB (BJD)
\newcommand{\hatcurLChatnetmAxxxxAmH}{\ensuremath{12.3041\pm0.0003}}   % HATNet OOT level
\newcommand{\hatcurLCiblendAxxxxAmH}{\ensuremath{1.27\pm0.17}}         % HATNet iblend factor
\newcommand{\hatcurLChatnetmBxxxxAmH}{\ensuremath{12.9595\pm0.0001}}   % HATNet OOT level
\newcommand{\hatcurLCiblendBxxxxAmH}{\ensuremath{0.79\pm0.03}}         % HATNet iblend factor
%% --------------------------------------------------------------------
\newcommand{\hatcurSMEiteffxxxxAmH}{\ensuremath{5295\pm100}}           % Ini SME, stellar effective temperature
\newcommand{\hatcurSMEizfehxxxxAmH}{\ensuremath{0.33\pm0.1}}           % Ini SME, stellar metallicity
\newcommand{\hatcurSMEizfehshortxxxxAmH}{\ensuremath{0.33}}            % Ini SME, stellar metallicity
\newcommand{\hatcurSMEiloggxxxxAmH}{\ensuremath{4.42\pm0.1}}           % Ini SME, stellar surface gravity
\newcommand{\hatcurSMEivsinxxxxAmH}{\ensuremath{0.2\pm0.5}}            % Ini SME, stellar rotational velocity
\newcommand{\hatcurSMEivmacxxxxAmH}{\ensuremath{3.28}}                 % Ini SME, stellar macroturbulence
\newcommand{\hatcurSMEivmicxxxxAmH}{\ensuremath{0.85}}                 % Ini SME, stellar microturbulence
\newcommand{\hatcurSMEiiteffxxxxAmH}{\ensuremath{5295\pm100}}          % Final SME, stellar effective temperature
\newcommand{\hatcurSMEiizfehxxxxAmH}{\ensuremath{0.33\pm0.10}}         % Final SME, stellar metallicity
\newcommand{\hatcurSMEiizfehshortxxxxAmH}{\ensuremath{0.33}}           % Final SME, stellar metallicity
\newcommand{\hatcurSMEiiloggxxxxAmH}{\ensuremath{4.42\pm0.1}}          % Final SME, stellar surface gravity
\newcommand{\hatcurSMEiivsinxxxxAmH}{\ensuremath{0.2\pm0.5}}           % Final SME, stellar rotational velocity
\newcommand{\hatcurSMEiivmacxxxxAmH}{\ensuremath{3.28}}                % Final SME, stellar macroturbulence
\newcommand{\hatcurSMEiivmicxxxxAmH}{\ensuremath{0.85}}                % Final SME, stellar microturbulence
%% --------------------------------------------------------------------
\newcommand{\hatcurDSteffxxxxAmH}{\ensuremath{NULL\pmNULL}}            % DS stellar effective temperature
\newcommand{\hatcurDSzfehxxxxAmH}{\ensuremath{NULL\pmNULL}}            % DS stellar metallicity
\newcommand{\hatcurDSloggxxxxAmH}{\ensuremath{NULL\pmNULL}}            % DS stellar surface gravity
\newcommand{\hatcurDSvsinixxxxAmH}{\ensuremath{NULL\pmNULL}}           % DS stellar rotational velocity
\newcommand{\hatcurDSgammaxxxxAmH}{\ensuremath{NULL\pmNULL}}           % DS absolute gamma velocity
\newcommand{\hatcurDSnumspecxxxxAmH}{\ensuremath{0}}                   % DS number of spectra
\newcommand{\hatcurDSspanxxxxAmH}{\ensuremath{0}}                      % DS stellar surface gravity
\newcommand{\hatcurDSrvrmsxxxxAmH}{\ensuremath{0.00}}                  % DS rms of RV values [km/s]
%% --------------------------------------------------------------------
\newcommand{\hatcurTRESteffxxxxAmH}{\ensuremath{5250\pm100}}           % TRES stellar effective temperature
\newcommand{\hatcurTRESzfehxxxxAmH}{\ensuremath{NULL\pmNULL}}          % TRES stellar metallicity
\newcommand{\hatcurTRESloggxxxxAmH}{\ensuremath{4.5\pm0.5}}            % TRES stellar surface gravity
\newcommand{\hatcurTRESvsinixxxxAmH}{\ensuremath{2.0\pm0.5}}           % TRES stellar rotational velocity
\newcommand{\hatcurTRESgammaxxxxAmH}{\ensuremath{-33.45\pm0.05}}       % TRES absolute gamma velocity
\newcommand{\hatcurTRESnumspecxxxxAmH}{\ensuremath{2}}                 % TRES number of spectra
\newcommand{\hatcurTRESspanxxxxAmH}{\ensuremath{27}}                   % TRES stellar surface gravity
\newcommand{\hatcurTRESrvrmsxxxxAmH}{\ensuremath{0.05}}                % TRES rms of RV values [km/s]
%% --------------------------------------------------------------------
\newcommand{\hatcurFIESteffxxxxAmH}{\ensuremath{NULL\pmNULL}}          % FIES stellar effective temperature
\newcommand{\hatcurFIESzfehxxxxAmH}{\ensuremath{NULL\pmNULL}}          % FIES stellar metallicity
\newcommand{\hatcurFIESloggxxxxAmH}{\ensuremath{NULL\pmNULL}}          % FIES stellar surface gravity
\newcommand{\hatcurFIESvsinixxxxAmH}{\ensuremath{NULL\pmNULL}}         % FIES stellar rotational velocity
\newcommand{\hatcurFIESgammaxxxxAmH}{\ensuremath{NULL\pmNULL}}         % FIES absolute gamma velocity
\newcommand{\hatcurFIESnumspecxxxxAmH}{\ensuremath{0}}                 % FIES number of spectra
\newcommand{\hatcurFIESspanxxxxAmH}{\ensuremath{0}}                    % FIES stellar surface gravity
\newcommand{\hatcurFIESrvrmsxxxxAmH}{\ensuremath{0.00}}                % FIES rms of RV values [km/s]
%% --------------------------------------------------------------------
\newcommand{\hatcurLBizxxxxAmH}{\ensuremath{0.2806}}                   % Limb darkening parameters, Gamma1, z-band
\newcommand{\hatcurLBiizxxxxAmH}{\ensuremath{0.3000}}                  % Limb darkening parameters, Gamma2, z-band
\newcommand{\hatcurLBiixxxxAmH}{\ensuremath{0.3648}}                   % Limb darkening parameters, Gamma1, i-band
\newcommand{\hatcurLBiiixxxxAmH}{\ensuremath{0.2817}}                  % Limb darkening parameters, Gamma2, i-band
\newcommand{\hatcurLBiIxxxxAmH}{\ensuremath{0.3373}}                   % Limb darkening parameters, Gamma1, I-band
\newcommand{\hatcurLBiiIxxxxAmH}{\ensuremath{0.2876}}                  % Limb darkening parameters, Gamma2, I-band
\newcommand{\hatcurLBigxxxxAmH}{\ensuremath{0.7194}}                   % Limb darkening parameters, Gamma1, g-band
\newcommand{\hatcurLBiigxxxxAmH}{\ensuremath{0.1078}}                  % Limb darkening parameters, Gamma2, g-band
\newcommand{\hatcurLBirxxxxAmH}{\ensuremath{0.4837}}                   % Limb darkening parameters, Gamma1, r-band
\newcommand{\hatcurLBiirxxxxAmH}{\ensuremath{0.2493}}                  % Limb darkening parameters, Gamma2, r-band
\newcommand{\hatcurLBiRxxxxAmH}{\ensuremath{0.4510}}                   % Limb darkening parameters, Gamma1, R-band
\newcommand{\hatcurLBiiRxxxxAmH}{\ensuremath{0.2591}}                  % Limb darkening parameters, Gamma2, R-band
\newcommand{\hatcurLBikepxxxxAmH}{\ensuremath{}}               % darkening parameters, Gamma1, Kep-band
\newcommand{\hatcurLBiikepxxxxAmH}{\ensuremath{}}              % darkening parameters, Gamma2, Kep-band
%% --------------------------------------------------------------------
\newcommand{\hatcurISOmxxxxAmH}{\ensuremath{0.94\pm0.04}}              % stellar mass
\newcommand{\hatcurISOmshortxxxxAmH}{\ensuremath{0.94}}                % stellar mass
\newcommand{\hatcurISOmlongxxxxAmH}{\ensuremath{0.937\pm0.041}}        % stellar mass
\newcommand{\hatcurISOrxxxxAmH}{\ensuremath{0.98_{-0.04}^{+0.05}}}     % stellar radius
\newcommand{\hatcurISOrshortxxxxAmH}{\ensuremath{0.98}}                % stellar radius
\newcommand{\hatcurISOrlongxxxxAmH}{\ensuremath{0.980_{-0.037}^{+0.051}}} % stellar radius
\newcommand{\hatcurISOrhoxxxxAmH}{\ensuremath{1.40\pm0.17}}            % stellar density (cgs)
\newcommand{\hatcurISOloggxxxxAmH}{\ensuremath{4.43\pm0.06}}           % stellar surface gravity from isochrones
\newcommand{\hatcurISOlumxxxxAmH}{\ensuremath{0.68_{-0.08}^{+0.10}}}   % stellar luminosity
\newcommand{\hatcurISOlumshortxxxxAmH}{\ensuremath{0.68}}              % stellar luminosity
\newcommand{\hatcurISOmvxxxxAmH}{\ensuremath{5.34\pm0.17}}             % stellar absolute magnitude
\newcommand{\hatcurISOvixxxxAmH}{\ensuremath{0.846\pm0.027}}           % stellar V-I index
\newcommand{\hatcurISOagexxxxAmH}{\ensuremath{8.9\pm3.1}}              % stellar age
\newcommand{\hatcurISOsigmaxxxxAmH}{\ensuremath{0.00060\pm0.00009}}    % system mass-correction sigma parameter
\newcommand{\hatcurISOMJxxxxAmH}{\ensuremath{3.93\pm0.12}}             % stellar absolute J magnitude
\newcommand{\hatcurISOMHxxxxAmH}{\ensuremath{3.50\pm0.11}}             % stellar absolute H magnitude
\newcommand{\hatcurISOMKxxxxAmH}{\ensuremath{3.43\pm0.11}}             % stellar absolute K magnitude
\newcommand{\hatcurISOJKxxxxAmH}{\ensuremath{0.50\pm0.02}}             % J-K color index from isochrones.
\newcommand{\hatcurISOspecxxxxAmH}{G9}                                 % stellar spectral type
%% --------------------------------------------------------------------
\newcommand{\hatcurRVKxxxxAmH}{\ensuremath{53.4\pm2.1}}                % RV semi-amplitude [m/s]
\newcommand{\hatcurRVrkxxxxAmH}{\ensuremath{-0.009\pm0.083}}           % sqrt(e)*cos(omega)
\newcommand{\hatcurRVrhxxxxAmH}{\ensuremath{0.248_{-0.105}^{+0.079}}}  % sqrt(e)*sin(omega)
\newcommand{\hatcurRVkxxxxAmH}{\ensuremath{-0.002_{-0.025}^{+0.019}}}  % e*cos(omega)
\newcommand{\hatcurRVhxxxxAmH}{\ensuremath{0.065_{-0.035}^{+0.047}}}   % e*sin(omega)
\newcommand{\hatcurRVtronexxxxAmH}{\ensuremath{0.0000\pm0.0000}}       % RV linear trend tr1 factor
\newcommand{\hatcurRVtrtwoxxxxAmH}{\ensuremath{0.0000\pm0.0000}}       % RV linear trend tr2 factor
\newcommand{\hatcurRVgammaxxxxAmH}{\ensuremath{1.9\pm2.2}}             % RV gamma velocity, relative scale
\newcommand{\hatcurRVjitterxxxxAmH}{\ensuremath{6.6\pm1.7}}            % RV jitter (m/s)
\newcommand{\hatcurRVfitrmsxxxxAmH}{\ensuremath{10.5}}                 % RVfitrms
\newcommand{\hatcurRVeccenxxxxAmH}{\ensuremath{0.069\pm0.040}}         % eccentricity
\newcommand{\hatcurRVomegaxxxxAmH}{\ensuremath{92\pm28}}               % argument of pericenter
%% --------------------------------------------------------------------
\newcommand{\hatcurPPixxxxAmH}{\ensuremath{89.3_{-0.4}^{+0.3}}}        % orbital inclination
\newcommand{\hatcurPPgxxxxAmH}{\ensuremath{6.2\pm0.5}}                 % planetary surface gravity (m/s^2)
\newcommand{\hatcurPPloggxxxxAmH}{\ensuremath{2.79\pm0.04}}            % planetary surface gravity (log cgs)
\newcommand{\hatcurPParxxxxAmH}{\ensuremath{11.10\pm0.47}}             % relative orbital radius (a/R*)
\newcommand{\hatcurPParelxxxxAmH}{\ensuremath{0.0507\pm0.0007}}        % semimajor axis (AU)
\newcommand{\hatcurPPrhoxxxxAmH}{\ensuremath{0.24\pm0.03}}             % planetary density (cgs)
\newcommand{\hatcurPPmxxxxAmH}{\ensuremath{0.41\pm0.02}}               % planetary mass (M_jup)
\newcommand{\hatcurPPmshortxxxxAmH}{\ensuremath{0.41}}                 % planetary mass (M_jup)
\newcommand{\hatcurPPmlongxxxxAmH}{\ensuremath{0.407\pm0.019}}         % planetary mass (M_jup)
\newcommand{\hatcurPPmexxxxAmH}{\ensuremath{129.5\pm6.2}}              % planetary mass (M_earth)
\newcommand{\hatcurPPmeshortxxxxAmH}{\ensuremath{129.5}}               % planetary mass (M_earth)
\newcommand{\hatcurPPmelongxxxxAmH}{\ensuremath{129.50\pm6.16}}        % planetary mass (M_earth)
\newcommand{\hatcurPPrxxxxAmH}{\ensuremath{1.28_{-0.05}^{+0.07}}}      % planetary radius (R_jup)
\newcommand{\hatcurPPrshortxxxxAmH}{\ensuremath{1.28}}                 % planetary radius (R_jup)
\newcommand{\hatcurPPrlongxxxxAmH}{\ensuremath{1.278_{-0.046}^{+0.066}}} % planetary radius (R_jup)
\newcommand{\hatcurPPrexxxxAmH}{\ensuremath{14.3_{-0.5}^{+0.7}}}       % planetary radius (R_earth)
\newcommand{\hatcurPPreshortxxxxAmH}{\ensuremath{14.3}}                % planetary radius (R_earth)
\newcommand{\hatcurPPrelongxxxxAmH}{\ensuremath{14.32_{-0.52}^{+0.74}}} % planetary radius (R_earth)
\newcommand{\hatcurPPmrcorrxxxxAmH}{\ensuremath{0.33}}                 % mass/radius correlation
\newcommand{\hatcurPPteffxxxxAmH}{\ensuremath{1126\pm33}}              % planetary temperature (K)
\newcommand{\hatcurPPthetaxxxxAmH}{\ensuremath{0.034\pm0.002}}         % Safranov number
\newcommand{\hatcurPPfluxperixxxxAmH}{\ensuremath{4.17_{-0.61}^{+1.05}}} % flux @ periastron (CGS)
\newcommand{\hatcurPPfluxperidimxxxxAmH}{\ensuremath{8}}               % flux @ periastron (CGS) units.
\newcommand{\hatcurPPfluxapxxxxAmH}{\ensuremath{3.16\pm0.25}}          % flux @ apastron (CGS)
\newcommand{\hatcurPPfluxapdimxxxxAmH}{\ensuremath{8}}                 % flux @ apastron (CGS) units.
\newcommand{\hatcurPPfluxavgxxxxAmH}{\ensuremath{3.63_{-0.37}^{+0.49}}} % flux on average (CGS)
\newcommand{\hatcurPPfluxavgdimxxxxAmH}{\ensuremath{8}}                % flux average (CGS) units.
%% --------------------------------------------------------------------
\newcommand{\hatcurXsecphasexxxxAmH}{\ensuremath{0.4988\pm0.0142}}     % Phase of secondary eclipse
\newcommand{\hatcurXsecondaryxxxxAmH}{\ensuremath{2455699.082\pm0.061}} % Secondary eclipse epoch
\newcommand{\hatcurXsecdurxxxxAmH}{\ensuremath{0.1477\pm0.0125}}       % sec eclipse duration (days)
\newcommand{\hatcurXsecingdurxxxxAmH}{\ensuremath{0.0179\pm0.0017}}    % sec I/E duration (days)
\newcommand{\hatcurPPphiconjxxxxAmH}{\ensuremath{-0.0045\pm0.0680}}    % phase diff between conjunction and periastron
\newcommand{\hatcurPPperixxxxAmH}{\ensuremath{2455696.96\pm0.29}}      % time of periastron passage.
\newcommand{\hatcurPPaequivxxxxAmH}{\ensuremath{0.0614\pm0.0035}}      % equivalent semi-major axis
\newcommand{\hatcurPPtcircxxxxAmH}{\ensuremath{187.9\pm43.5}}          % circularization timescale
\newcommand{\hatcurPPtinfallxxxxAmH}{\ensuremath{6918749.5_{-2013876.0}^{+6170156.4}}} % infall timescale
%% --------------------------------------------------------------------
\newcommand{\hatcurcLCdurxxxxAmH}{\ensuremath{0.504\pm0.019}}          % transit duration (days)
\newcommand{\hatcurcLCdurshortxxxxAmH}{\ensuremath{0.504}}             % transit duration (days)
\newcommand{\hatcurcLCdurhrxxxxAmH}{\ensuremath{12.1\pm0.5}}           % transit duration (hours)
\newcommand{\hatcurcLCdurhrshortxxxxAmH}{\ensuremath{12.1}}            % transit duration (hours)
\newcommand{\hatcurcLCqxxxxAmH}{\ensuremath{0.0023\pm0.0001}}          % fractional transit duration (days)
\newcommand{\hatcurcLCqshortxxxxAmH}{\ensuremath{0.002}}               % fractional transit duration (days)
\newcommand{\hatcurcLCingdurxxxxAmH}{\ensuremath{0.0477\pm0.0007}}     % ingress/egress duration (days)
\newcommand{\hatcurcLCPxxxxAmH}{\ensuremath{217.0\pm3.3}}              % period (days)
\newcommand{\hatcurcLCPprecxxxxAmH}{\ensuremath{217.01}}               % period (days)
\newcommand{\hatcurcLCPshortxxxxAmH}{\ensuremath{217}}                 % period (days)
\newcommand{\hatcurcLCTxxxxAmH}{\ensuremath{2455685.9\pm2.1}}          % epoch (BJD)
\newcommand{\hatcurcRVKxxxxAmH}{\ensuremath{57\pm3}}                   % RV semi-amplitude [m/s]
\newcommand{\hatcurcRVrkxxxxAmH}{\ensuremath{0}}                       % sqrt(e)*cos(omega)
\newcommand{\hatcurcRVrhxxxxAmH}{\ensuremath{0}}                       % sqrt(e)*sin(omega)
\newcommand{\hatcurcRVkxxxxAmH}{\ensuremath{0}}                        % e*cos(omega)
\newcommand{\hatcurcRVhxxxxAmH}{\ensuremath{0}}                        % e*sin(omega)
\newcommand{\hatcurcRVkcorrxxxxAmH}{\ensuremath{0.000\pm0.000}}        % e*cos(omega) corrected
\newcommand{\hatcurcRVhcorrxxxxAmH}{\ensuremath{0.000\pm0.000}}        % e*sin(omega) corrected
\newcommand{\hatcurcRVckhxxxxAmH}{\ensuremath{1.000\pm0.000}}          % eccentricity correction (C_{rm kh})
\newcommand{\hatcurcRVeccenxxxxAmH}{\ensuremath{0}}                    % eccentricity
\newcommand{\hatcurcRVomegaxxxxAmH}{\ensuremath{0}}                    % argument of pericenter
%% --------------------------------------------------------------------
\newcommand{\hatcurcPPixxxxAmH}{\ensuremath{90.0\pm0.0}}               % orbital inclination
\newcommand{\hatcurcPPgxxxxAmH}{\ensuremath{40.0\pm2.8}}               % planetary surface gravity (m/s^2)
\newcommand{\hatcurcPPloggxxxxAmH}{\ensuremath{3.60\pm0.03}}           % planetary surface gravity (log cgs)
\newcommand{\hatcurcPParxxxxAmH}{\ensuremath{151.47\pm7.10}}           % relative orbital radius (a/R*)
\newcommand{\hatcurcPParelxxxxAmH}{\ensuremath{0.692\pm0.012}}         % semimajor axis (AU)
\newcommand{\hatcurcPPrhoxxxxAmH}{\ensuremath{2.002\pm0.141}}          % planetary density (cgs)
\newcommand{\hatcurcPPmxxxxAmH}{\ensuremath{1.6\pm0.1}}                % planetary mass (M_jup)
\newcommand{\hatcurcPPmshortxxxxAmH}{\ensuremath{1.6}}                 % planetary mass (M_jup)
\newcommand{\hatcurcPPmlongxxxxAmH}{\ensuremath{1.6\pm0.1}}            % planetary mass (M_jup)
\newcommand{\hatcurcPPmexxxxAmH}{\ensuremath{512.9\pm36.2}}            % planetary mass (M_earth)
\newcommand{\hatcurcPPmeshortxxxxAmH}{\ensuremath{512.9}}              % planetary mass (M_earth)
\newcommand{\hatcurcPPmelongxxxxAmH}{\ensuremath{512.93\pm36.22}}      % planetary mass (M_earth)
\newcommand{\hatcurcPPrxxxxAmH}{\ensuremath{1.00\pm0.00}}              % planetary radius (R_jup)
\newcommand{\hatcurcPPrshortxxxxAmH}{\ensuremath{1.00}}                % planetary radius (R_jup)
\newcommand{\hatcurcPPrlongxxxxAmH}{\ensuremath{1.000\pm0.000}}        % planetary radius (R_jup)
\newcommand{\hatcurcPPrexxxxAmH}{\ensuremath{11.2\pm0.0}}              % planetary radius (R_earth)
\newcommand{\hatcurcPPreshortxxxxAmH}{\ensuremath{11.2}}               % planetary radius (R_earth)
\newcommand{\hatcurcPPrelongxxxxAmH}{\ensuremath{11.21\pm0.00}}        % planetary radius (R_earth)
\newcommand{\hatcurcPPmrcorrxxxxAmH}{\ensuremath{0.00}}                % mass/radius correlation
\newcommand{\hatcurcPPteffxxxxAmH}{\ensuremath{304\pm9}}               % planetary temperature (K)
\newcommand{\hatcurcPPthetaxxxxAmH}{\ensuremath{2.384\pm0.159}}        % Safranov number
\newcommand{\hatcurcPPfluxavgxxxxAmH}{\ensuremath{1.94\pm0.242}}       % flux on average (CGS)
\newcommand{\hatcurcPPfluxavgdimxxxxAmH}{\ensuremath{6}}               % flux average (CGS) units.
%% --------------------------------------------------------------------
\newcommand{\hatcurcXsecphasexxxxAmH}{\ensuremath{0.5}}                % Phase of secondary eclipse
\newcommand{\hatcurcXsecondaryxxxxAmH}{\ensuremath{2455848.6\pm3.1}}   % Secondary eclipse epoch
\newcommand{\hatcurcXsecdurxxxxAmH}{\ensuremath{0.504\pm0.019}}        % sec eclipse duration (days)
\newcommand{\hatcurcXsecingdurxxxxAmH}{\ensuremath{0.0477\pm0.0007}}   % sec I/E duration (days)
\newcommand{\hatcurcPPphiconjxxxxAmH}{\ensuremath{0.2500\pm0.0000}}    % phase diff between conjunction and periastron
\newcommand{\hatcurcPPperixxxxAmH}{\ensuremath{2455631.68\pm2.27}}     % time of periastron passage.
\newcommand{\hatcurcPPaequivxxxxAmH}{\ensuremath{0.8382\pm0.0508}}     % equivalent semi-major axis
\newcommand{\hatcurcPPtcircxxxxAmH}{\ensuremath{62770941872.0\pm7305668436.7}} % circularization timescale
\newcommand{\hatcurcPPtinfallxxxxAmH}{\ensuremath{0.0\pm0.0}}          % infall timescale
%% --------------------------------------------------------------------
\newcommand{\hatcurdLCdurxxxxAmH}{\ensuremath{0.218\pm0.009}}          % transit duration (days)
\newcommand{\hatcurdLCdurshortxxxxAmH}{\ensuremath{0.218}}             % transit duration (days)
\newcommand{\hatcurdLCdurhrxxxxAmH}{\ensuremath{5.2\pm0.2}}            % transit duration (hours)
\newcommand{\hatcurdLCdurhrshortxxxxAmH}{\ensuremath{5.2}}             % transit duration (hours)
\newcommand{\hatcurdLCqxxxxAmH}{\ensuremath{0.0124\pm0.0005}}          % fractional transit duration (days)
\newcommand{\hatcurdLCqshortxxxxAmH}{\ensuremath{0.012}}               % fractional transit duration (days)
\newcommand{\hatcurdLCingdurxxxxAmH}{\ensuremath{0.0206\pm0.0003}}     % ingress/egress duration (days)
\newcommand{\hatcurdLCPxxxxAmH}{\ensuremath{17.5\pm0.1}}               % period (days)
\newcommand{\hatcurdLCPprecxxxxAmH}{\ensuremath{17.49}}                % period (days)
\newcommand{\hatcurdLCPshortxxxxAmH}{\ensuremath{17}}                  % period (days)
\newcommand{\hatcurdLCTxxxxAmH}{\ensuremath{2455699.9\pm0.6}}          % epoch (BJD)
\newcommand{\hatcurdRVKxxxxAmH}{\ensuremath{11\pm2}}                   % RV semi-amplitude [m/s]
\newcommand{\hatcurdRVrkxxxxAmH}{\ensuremath{0}}                       % sqrt(e)*cos(omega)
\newcommand{\hatcurdRVrhxxxxAmH}{\ensuremath{0}}                       % sqrt(e)*sin(omega)
\newcommand{\hatcurdRVkxxxxAmH}{\ensuremath{0}}                        % e*cos(omega)
\newcommand{\hatcurdRVhxxxxAmH}{\ensuremath{0}}                        % e*sin(omega)
\newcommand{\hatcurdRVkcorrxxxxAmH}{\ensuremath{0.000\pm0.000}}        % e*cos(omega) corrected
\newcommand{\hatcurdRVhcorrxxxxAmH}{\ensuremath{0.000\pm0.000}}        % e*sin(omega) corrected
\newcommand{\hatcurdRVckhxxxxAmH}{\ensuremath{1.000\pm0.000}}          % eccentricity correction (C_{rm kh})
\newcommand{\hatcurdRVeccenxxxxAmH}{\ensuremath{0}}                    % eccentricity
\newcommand{\hatcurdRVomegaxxxxAmH}{\ensuremath{0}}                    % argument of pericenter
%% --------------------------------------------------------------------
\newcommand{\hatcurdPPixxxxAmH}{\ensuremath{90.0\pm0.0}}               % orbital inclination
\newcommand{\hatcurdPPgxxxxAmH}{\ensuremath{3.6\pm0.8}}                % planetary surface gravity (m/s^2)
\newcommand{\hatcurdPPloggxxxxAmH}{\ensuremath{2.56_{-0.14}^{+0.08}}}  % planetary surface gravity (log cgs)
\newcommand{\hatcurdPParxxxxAmH}{\ensuremath{28.29\pm1.18}}            % relative orbital radius (a/R*)
\newcommand{\hatcurdPParelxxxxAmH}{\ensuremath{0.129\pm0.002}}         % semimajor axis (AU)
\newcommand{\hatcurdPPrhoxxxxAmH}{\ensuremath{0.180\pm0.042}}          % planetary density (cgs)
\newcommand{\hatcurdPPmxxxxAmH}{\ensuremath{0.1\pm0.0}}                % planetary mass (M_jup)
\newcommand{\hatcurdPPmshortxxxxAmH}{\ensuremath{0.1}}                 % planetary mass (M_jup)
\newcommand{\hatcurdPPmlongxxxxAmH}{\ensuremath{0.1\pm0.0}}            % planetary mass (M_jup)
\newcommand{\hatcurdPPmexxxxAmH}{\ensuremath{46.1\pm10.7}}             % planetary mass (M_earth)
\newcommand{\hatcurdPPmeshortxxxxAmH}{\ensuremath{46.1}}               % planetary mass (M_earth)
\newcommand{\hatcurdPPmelongxxxxAmH}{\ensuremath{46.11\pm10.65}}       % planetary mass (M_earth)
\newcommand{\hatcurdPPrxxxxAmH}{\ensuremath{1.00\pm0.00}}              % planetary radius (R_jup)
\newcommand{\hatcurdPPrshortxxxxAmH}{\ensuremath{1.00}}                % planetary radius (R_jup)
\newcommand{\hatcurdPPrlongxxxxAmH}{\ensuremath{1.000\pm0.000}}        % planetary radius (R_jup)
\newcommand{\hatcurdPPrexxxxAmH}{\ensuremath{11.2\pm0.0}}              % planetary radius (R_earth)
\newcommand{\hatcurdPPreshortxxxxAmH}{\ensuremath{11.2}}               % planetary radius (R_earth)
\newcommand{\hatcurdPPrelongxxxxAmH}{\ensuremath{11.21\pm0.00}}        % planetary radius (R_earth)
\newcommand{\hatcurdPPmrcorrxxxxAmH}{\ensuremath{0.00}}                % mass/radius correlation
\newcommand{\hatcurdPPteffxxxxAmH}{\ensuremath{705\pm20}}              % planetary temperature (K)
\newcommand{\hatcurdPPthetaxxxxAmH}{\ensuremath{0.040\pm0.009}}        % Safranov number
\newcommand{\hatcurdPPfluxavgxxxxAmH}{\ensuremath{5.58\pm0.649}}       % flux on average (CGS)
\newcommand{\hatcurdPPfluxavgdimxxxxAmH}{\ensuremath{7}}               % flux average (CGS) units.
%% --------------------------------------------------------------------
\newcommand{\hatcurdXsecphasexxxxAmH}{\ensuremath{0.5}}                % Phase of secondary eclipse
\newcommand{\hatcurdXsecondaryxxxxAmH}{\ensuremath{2455713.0\pm0.6}}   % Secondary eclipse epoch
\newcommand{\hatcurdXsecdurxxxxAmH}{\ensuremath{0.218\pm0.009}}        % sec eclipse duration (days)
\newcommand{\hatcurdXsecingdurxxxxAmH}{\ensuremath{0.0206\pm0.0003}}   % sec I/E duration (days)
\newcommand{\hatcurdPPphiconjxxxxAmH}{\ensuremath{0.2500\pm0.0000}}    % phase diff between conjunction and periastron
\newcommand{\hatcurdPPperixxxxAmH}{\ensuremath{2455695.53_{-0.45}^{+0.72}}} % time of periastron passage.
\newcommand{\hatcurdPPaequivxxxxAmH}{\ensuremath{0.1565\pm0.0088}}     % equivalent semi-major axis
\newcommand{\hatcurdPPtcircxxxxAmH}{\ensuremath{102562.8\pm24001.0}}   % circularization timescale
\newcommand{\hatcurdPPtinfallxxxxAmH}{\ensuremath{0.0\pm0.0}}          % infall timescale
%% --------------------------------------------------------------------
\newcommand{\hatcureLCdurxxxxAmH}{\ensuremath{0.198\pm0.008}}          % transit duration (days)
\newcommand{\hatcureLCdurshortxxxxAmH}{\ensuremath{0.198}}             % transit duration (days)
\newcommand{\hatcureLCdurhrxxxxAmH}{\ensuremath{4.8\pm0.2}}            % transit duration (hours)
\newcommand{\hatcureLCdurhrshortxxxxAmH}{\ensuremath{4.8}}             % transit duration (hours)
\newcommand{\hatcureLCqxxxxAmH}{\ensuremath{0.0149\pm0.0006}}          % fractional transit duration (days)
\newcommand{\hatcureLCqshortxxxxAmH}{\ensuremath{0.015}}               % fractional transit duration (days)
\newcommand{\hatcureLCingdurxxxxAmH}{\ensuremath{0.0188\pm0.0003}}     % ingress/egress duration (days)
\newcommand{\hatcureLCPxxxxAmH}{\ensuremath{13.3\pm0.1}}               % period (days)
\newcommand{\hatcureLCPprecxxxxAmH}{\ensuremath{13.28}}                % period (days)
\newcommand{\hatcureLCPshortxxxxAmH}{\ensuremath{13}}                  % period (days)
\newcommand{\hatcureLCTxxxxAmH}{\ensuremath{2455606.9\pm0.9}}          % epoch (BJD)
\newcommand{\hatcureRVKxxxxAmH}{\ensuremath{9\pm2}}                    % RV semi-amplitude [m/s]
\newcommand{\hatcureRVrkxxxxAmH}{\ensuremath{0}}                       % sqrt(e)*cos(omega)
\newcommand{\hatcureRVrhxxxxAmH}{\ensuremath{0}}                       % sqrt(e)*sin(omega)
\newcommand{\hatcureRVkxxxxAmH}{\ensuremath{0}}                        % e*cos(omega)
\newcommand{\hatcureRVhxxxxAmH}{\ensuremath{0}}                        % e*sin(omega)
\newcommand{\hatcureRVkcorrxxxxAmH}{\ensuremath{0.000\pm0.000}}        % e*cos(omega) corrected
\newcommand{\hatcureRVhcorrxxxxAmH}{\ensuremath{0.000\pm0.000}}        % e*sin(omega) corrected
\newcommand{\hatcureRVckhxxxxAmH}{\ensuremath{1.000\pm0.000}}          % eccentricity correction (C_{rm kh})
\newcommand{\hatcureRVeccenxxxxAmH}{\ensuremath{0}}                    % eccentricity
\newcommand{\hatcureRVomegaxxxxAmH}{\ensuremath{0}}                    % argument of pericenter
%% --------------------------------------------------------------------
\newcommand{\hatcurePPixxxxAmH}{\ensuremath{90.0\pm0.0}}               % orbital inclination
\newcommand{\hatcurePPgxxxxAmH}{\ensuremath{2.5\pm0.8}}                % planetary surface gravity (m/s^2)
\newcommand{\hatcurePPloggxxxxAmH}{\ensuremath{2.40_{-0.20}^{+0.11}}}  % planetary surface gravity (log cgs)
\newcommand{\hatcurePParxxxxAmH}{\ensuremath{23.53\pm0.98}}            % relative orbital radius (a/R*)
\newcommand{\hatcurePParelxxxxAmH}{\ensuremath{0.107\pm0.002}}         % semimajor axis (AU)
\newcommand{\hatcurePPrhoxxxxAmH}{\ensuremath{0.127\pm0.040}}          % planetary density (cgs)
\newcommand{\hatcurePPmxxxxAmH}{\ensuremath{0.1\pm0.0}}                % planetary mass (M_jup)
\newcommand{\hatcurePPmshortxxxxAmH}{\ensuremath{0.1}}                 % planetary mass (M_jup)
\newcommand{\hatcurePPmlongxxxxAmH}{\ensuremath{0.1\pm0.0}}            % planetary mass (M_jup)
\newcommand{\hatcurePPmexxxxAmH}{\ensuremath{32.6\pm10.2}}             % planetary mass (M_earth)
\newcommand{\hatcurePPmeshortxxxxAmH}{\ensuremath{32.6}}               % planetary mass (M_earth)
\newcommand{\hatcurePPmelongxxxxAmH}{\ensuremath{32.61\pm10.24}}       % planetary mass (M_earth)
\newcommand{\hatcurePPrxxxxAmH}{\ensuremath{1.00\pm0.00}}              % planetary radius (R_jup)
\newcommand{\hatcurePPrshortxxxxAmH}{\ensuremath{1.00}}                % planetary radius (R_jup)
\newcommand{\hatcurePPrlongxxxxAmH}{\ensuremath{1.000\pm0.000}}        % planetary radius (R_jup)
\newcommand{\hatcurePPrexxxxAmH}{\ensuremath{11.2\pm0.0}}              % planetary radius (R_earth)
\newcommand{\hatcurePPreshortxxxxAmH}{\ensuremath{11.2}}               % planetary radius (R_earth)
\newcommand{\hatcurePPrelongxxxxAmH}{\ensuremath{11.21\pm0.00}}        % planetary radius (R_earth)
\newcommand{\hatcurePPmrcorrxxxxAmH}{\ensuremath{0.00}}                % mass/radius correlation
\newcommand{\hatcurePPteffxxxxAmH}{\ensuremath{773\pm22}}              % planetary temperature (K)
\newcommand{\hatcurePPthetaxxxxAmH}{\ensuremath{0.024\pm0.007}}        % Safranov number
\newcommand{\hatcurePPfluxavgxxxxAmH}{\ensuremath{8.06\pm0.937}}       % flux on average (CGS)
\newcommand{\hatcurePPfluxavgdimxxxxAmH}{\ensuremath{7}}               % flux average (CGS) units.
%% --------------------------------------------------------------------
\newcommand{\hatcureXsecphasexxxxAmH}{\ensuremath{0.5}}                % Phase of secondary eclipse
\newcommand{\hatcureXsecondaryxxxxAmH}{\ensuremath{2455616.9\pm0.9}}   % Secondary eclipse epoch
\newcommand{\hatcureXsecdurxxxxAmH}{\ensuremath{0.198\pm0.008}}        % sec eclipse duration (days)
\newcommand{\hatcureXsecingdurxxxxAmH}{\ensuremath{0.0188\pm0.0003}}   % sec I/E duration (days)
\newcommand{\hatcurePPphiconjxxxxAmH}{\ensuremath{0.2500\pm0.0000}}    % phase diff between conjunction and periastron
\newcommand{\hatcurePPperixxxxAmH}{\ensuremath{2455603.63\pm0.91}}     % time of periastron passage.
\newcommand{\hatcurePPaequivxxxxAmH}{\ensuremath{0.1302\pm0.0073}}     % equivalent semi-major axis
\newcommand{\hatcurePPtcircxxxxAmH}{\ensuremath{21908.7\pm7012.1}}     % circularization timescale
\newcommand{\hatcurePPtinfallxxxxAmH}{\ensuremath{0.0\pm0.0}}          % infall timescale
%% --------------------------------------------------------------------
\newcommand{\hatcurXdistxxxxAmH}{\ensuremath{377\pm19}}                % distance (pc), no reddenning correction
\newcommand{\hatcurXAvxxxxAmH}{\ensuremath{0.000\pm0.081}}             % Av (mag)
\newcommand{\hatcurXdistredxxxxAmH}{\ensuremath{374\pm18}}             % distance with Av correction (pc)
\newcommand{\hatcurXEBVxxxxAmH}{\ensuremath{0.000\pm0.026}}            % E(B-V) (mag)
\newcommand{\hatcurXmvisoredxxxxAmH}{\ensuremath{13.254\pm0.064}}      % Expected m_v with reddening (mag)
\newcommand{\hatcurXmiisoredxxxxAmH}{\ensuremath{12.390\pm0.041}}      % Expected m_i with reddening (mag)
\newcommand{\hatcurXmjisoredxxxxAmH}{\ensuremath{11.812\pm0.018}}      % Expected m_j with reddening (mag)
\newcommand{\hatcurXmhisoredxxxxAmH}{\ensuremath{11.379\pm0.014}}      % Expected m_h with reddening (mag)
\newcommand{\hatcurXmkisoredxxxxAmH}{\ensuremath{11.305\pm0.014}}      % Expected m_k with reddening (mag)
\newcommand{\hatcurXviisoredxxxxAmH}{\ensuremath{0.861_{-0.023}^{+0.040}}} % Expected V-I with reddening (mag)
\newcommand{\hatcurXvkisoredxxxxAmH}{\ensuremath{1.950\pm0.069}}       % Expected V-K with reddening (mag)
\newcommand{\hatcurXjhisoredxxxxAmH}{\ensuremath{0.433\pm0.017}}       % Expected J-H with reddening (mag)
\newcommand{\hatcurXjkisoredxxxxAmH}{\ensuremath{0.508\pm0.019}}       % Expected J-K with reddening (mag)
\newcommand{\hatcurCCpmraxxxxAmH}{\ensuremath{-29.0\pm12.6}}           % proper motion, in RA
\newcommand{\hatcurCCpmdecxxxxAmH}{\ensuremath{12.3\pm11.4}}           % proper motion, in DEC
\newcommand{\hatcurCCpmxxxxAmH}{\ensuremath{31.5006\pm16.9918}}        % proper motion


==> data/HTR146-002_phfu_tab.tex <==
$ 55640.84396 $ & $  -0.00143 $ & $   0.00122 $ & $  12.01460 $ & $ i$\\
$ 55640.84597 $ & $   0.00034 $ & $   0.00119 $ & $  12.01570 $ & $ i$\\
$ 55640.84767 $ & $  -0.00081 $ & $   0.00119 $ & $  12.01670 $ & $ i$\\
$ 55640.84922 $ & $   0.00007 $ & $   0.00122 $ & $  12.01650 $ & $ i$\\
$ 55640.85109 $ & $  -0.00137 $ & $   0.00119 $ & $  12.01450 $ & $ i$\\
$ 55640.85271 $ & $   0.00200 $ & $   0.00122 $ & $  12.01870 $ & $ i$\\
$ 55640.85427 $ & $  -0.00050 $ & $   0.00121 $ & $  12.01580 $ & $ i$\\
$ 55640.85593 $ & $  -0.00410 $ & $   0.00122 $ & $  12.01310 $ & $ i$\\
$ 55640.85747 $ & $  -0.00288 $ & $   0.00122 $ & $  12.01370 $ & $ i$\\
$ 55640.85902 $ & $  -0.00104 $ & $   0.00119 $ & $  12.01550 $ & $ i$\\
$ 55640.86056 $ & $   0.00331 $ & $   0.00120 $ & $  12.01990 $ & $ i$\\
$ 55640.86211 $ & $   0.00068 $ & $   0.00122 $ & $  12.01770 $ & $ i$\\
$ 55640.86365 $ & $  -0.00190 $ & $   0.00120 $ & $  12.01410 $ & $ i$\\
$ 55640.86520 $ & $   0.00242 $ & $   0.00121 $ & $  12.01930 $ & $ i$\\
$ 55640.86674 $ & $   0.00317 $ & $   0.00120 $ & $  12.01960 $ & $ i$\\
$ 55640.86829 $ & $  -0.00001 $ & $   0.00119 $ & $  12.01760 $ & $ i$\\
$ 55640.87001 $ & $   0.00409 $ & $   0.00119 $ & $  12.02130 $ & $ i$\\
$ 55640.87156 $ & $  -0.00135 $ & $   0.00121 $ & $  12.01610 $ & $ i$\\
$ 55640.87310 $ & $   0.00060 $ & $   0.00120 $ & $  12.01770 $ & $ i$\\
$ 55640.87465 $ & $   0.00048 $ & $   0.00121 $ & $  12.01670 $ & $ i$\\
$ 55640.87620 $ & $   0.00128 $ & $   0.00119 $ & $  12.01890 $ & $ i$\\
$ 55640.87776 $ & $  -0.00161 $ & $   0.00118 $ & $  12.01630 $ & $ i$\\
$ 55640.87933 $ & $  -0.00088 $ & $   0.00120 $ & $  12.01740 $ & $ i$\\
$ 55640.88086 $ & $  -0.00272 $ & $   0.00119 $ & $  12.01430 $ & $ i$\\
$ 55640.88240 $ & $   0.00093 $ & $   0.00117 $ & $  12.01840 $ & $ i$\\
$ 55640.88396 $ & $  -0.00069 $ & $   0.00118 $ & $  12.01810 $ & $ i$\\
$ 55640.88553 $ & $  -0.00064 $ & $   0.00120 $ & $  12.01700 $ & $ i$\\
$ 55640.88707 $ & $   0.00212 $ & $   0.00116 $ & $  12.02050 $ & $ i$\\
$ 55640.88861 $ & $   0.00256 $ & $   0.00119 $ & $  12.02020 $ & $ i$\\
$ 55640.89014 $ & $  -0.00023 $ & $   0.00118 $ & $  12.01610 $ & $ i$\\
$ 55640.89170 $ & $  -0.00158 $ & $   0.00119 $ & $  12.01540 $ & $ i$\\
$ 55640.89333 $ & $  -0.00239 $ & $   0.00118 $ & $  12.01290 $ & $ i$\\
$ 55640.89487 $ & $   0.00200 $ & $   0.00129 $ & $  12.01610 $ & $ i$\\
$ 55640.90234 $ & $   0.00085 $ & $   0.00117 $ & $  12.01920 $ & $ i$\\
$ 55640.90389 $ & $  -0.00434 $ & $   0.00119 $ & $  12.01340 $ & $ i$\\
$ 55640.90543 $ & $   0.00058 $ & $   0.00119 $ & $  12.01800 $ & $ i$\\
$ 55640.90700 $ & $   0.00062 $ & $   0.00118 $ & $  12.01930 $ & $ i$\\
$ 55640.90854 $ & $   0.00182 $ & $   0.00119 $ & $  12.02030 $ & $ i$\\
$ 55640.91009 $ & $   0.00272 $ & $   0.00119 $ & $  12.02070 $ & $ i$\\
$ 55640.91163 $ & $   0.00286 $ & $   0.00116 $ & $  12.02090 $ & $ i$\\
$ 55640.91318 $ & $   0.00156 $ & $   0.00118 $ & $  12.02000 $ & $ i$\\
$ 55640.91490 $ & $  -0.00093 $ & $   0.00119 $ & $  12.01810 $ & $ i$\\
$ 55640.91652 $ & $  -0.00227 $ & $   0.00119 $ & $  12.01580 $ & $ i$\\
$ 55640.91824 $ & $   0.00004 $ & $   0.00118 $ & $  12.01810 $ & $ i$\\
$ 55640.91977 $ & $   0.00299 $ & $   0.00118 $ & $  12.02170 $ & $ i$\\
$ 55640.92134 $ & $  -0.00279 $ & $   0.00118 $ & $  12.01630 $ & $ i$\\
$ 55640.92289 $ & $  -0.00040 $ & $   0.00118 $ & $  12.01710 $ & $ i$\\
$ 55640.92445 $ & $  -0.00332 $ & $   0.00118 $ & $  12.01550 $ & $ i$\\
$ 55640.92618 $ & $   0.00138 $ & $   0.00118 $ & $  12.01870 $ & $ i$\\
$ 55640.92770 $ & $   0.00261 $ & $   0.00118 $ & $  12.01950 $ & $ i$\\
$ 55640.92925 $ & $  -0.00367 $ & $   0.00118 $ & $  12.01450 $ & $ i$\\
$ 55640.93079 $ & $  -0.00162 $ & $   0.00115 $ & $  12.01580 $ & $ i$\\
$ 55640.93236 $ & $   0.00031 $ & $   0.00118 $ & $  12.01800 $ & $ i$\\
$ 55640.93392 $ & $   0.00110 $ & $   0.00117 $ & $  12.01820 $ & $ i$\\
$ 55640.93546 $ & $   0.00179 $ & $   0.00118 $ & $  12.01960 $ & $ i$\\
$ 55640.93697 $ & $   0.00033 $ & $   0.00117 $ & $  12.01790 $ & $ i$\\
$ 55640.93854 $ & $   0.00081 $ & $   0.00117 $ & $  12.01780 $ & $ i$\\
$ 55640.94010 $ & $   0.00037 $ & $   0.00117 $ & $  12.01790 $ & $ i$\\
$ 55640.94165 $ & $   0.00010 $ & $   0.00118 $ & $  12.01940 $ & $ i$\\
$ 55640.94319 $ & $   0.00039 $ & $   0.00119 $ & $  12.01850 $ & $ i$\\
$ 55640.94474 $ & $  -0.00135 $ & $   0.00117 $ & $  12.01550 $ & $ i$\\
$ 55640.94630 $ & $  -0.00272 $ & $   0.00117 $ & $  12.01530 $ & $ i$\\
$ 55640.94786 $ & $   0.00216 $ & $   0.00117 $ & $  12.01880 $ & $ i$\\
$ 55640.94952 $ & $   0.00398 $ & $   0.00118 $ & $  12.02100 $ & $ i$\\
$ 55640.95107 $ & $   0.00259 $ & $   0.00117 $ & $  12.02020 $ & $ i$\\
$ 55640.95263 $ & $  -0.00105 $ & $   0.00119 $ & $  12.01680 $ & $ i$\\
$ 55640.95418 $ & $   0.00195 $ & $   0.00117 $ & $  12.01900 $ & $ i$\\
$ 55640.95586 $ & $  -0.00253 $ & $   0.00115 $ & $  12.01500 $ & $ i$\\
$ 55640.95741 $ & $  -0.00213 $ & $   0.00117 $ & $  12.01450 $ & $ i$\\
$ 55640.95896 $ & $   0.00056 $ & $   0.00119 $ & $  12.01710 $ & $ i$\\
$ 55640.96050 $ & $  -0.00023 $ & $   0.00118 $ & $  12.01700 $ & $ i$\\
$ 55640.96204 $ & $   0.00521 $ & $   0.00118 $ & $  12.02170 $ & $ i$\\
$ 55640.96369 $ & $   0.00776 $ & $   0.00119 $ & $  12.02500 $ & $ i$\\
$ 55640.96539 $ & $   0.01236 $ & $   0.00119 $ & $  12.02920 $ & $ i$\\
$ 55640.96694 $ & $   0.01059 $ & $   0.00119 $ & $  12.02740 $ & $ i$\\
$ 55640.96850 $ & $   0.01405 $ & $   0.00116 $ & $  12.03030 $ & $ i$\\
$ 55640.97006 $ & $   0.01372 $ & $   0.00119 $ & $  12.03080 $ & $ i$\\
$ 55640.97161 $ & $   0.01901 $ & $   0.00119 $ & $  12.03550 $ & $ i$\\
$ 55640.97325 $ & $   0.01724 $ & $   0.00119 $ & $  12.03410 $ & $ i$\\
$ 55640.97481 $ & $   0.01556 $ & $   0.00119 $ & $  12.03240 $ & $ i$\\
$ 55640.97636 $ & $   0.01831 $ & $   0.00119 $ & $  12.03590 $ & $ i$\\
$ 55640.97791 $ & $   0.02257 $ & $   0.00122 $ & $  12.04010 $ & $ i$\\
$ 55640.97958 $ & $   0.01865 $ & $   0.00121 $ & $  12.03550 $ & $ i$\\
$ 55640.98112 $ & $   0.01933 $ & $   0.00119 $ & $  12.03670 $ & $ i$\\
$ 55640.98266 $ & $   0.02298 $ & $   0.00121 $ & $  12.03860 $ & $ i$\\
$ 55640.98421 $ & $   0.02416 $ & $   0.00120 $ & $  12.04130 $ & $ i$\\
$ 55640.98575 $ & $   0.02097 $ & $   0.00123 $ & $  12.03800 $ & $ i$\\
$ 55640.98730 $ & $   0.01989 $ & $   0.00121 $ & $  12.03720 $ & $ i$\\
$ 55640.98884 $ & $   0.02275 $ & $   0.00120 $ & $  12.03910 $ & $ i$\\
$ 55640.99040 $ & $   0.02255 $ & $   0.00122 $ & $  12.03910 $ & $ i$\\
$ 55640.99193 $ & $   0.02032 $ & $   0.00120 $ & $  12.03760 $ & $ i$\\
$ 55640.99349 $ & $   0.02074 $ & $   0.00121 $ & $  12.03730 $ & $ i$\\
$ 55640.99514 $ & $   0.01838 $ & $   0.00120 $ & $  12.03560 $ & $ i$\\
$ 55640.99697 $ & $   0.02309 $ & $   0.00121 $ & $  12.03920 $ & $ i$\\
$ 55640.99852 $ & $   0.02275 $ & $   0.00120 $ & $  12.03940 $ & $ i$\\
$ 55641.00009 $ & $   0.02193 $ & $   0.00120 $ & $  12.03740 $ & $ i$\\
$ 55641.00162 $ & $   0.02088 $ & $   0.00120 $ & $  12.03800 $ & $ i$\\
$ 55641.00317 $ & $   0.02234 $ & $   0.00121 $ & $  12.03790 $ & $ i$\\
$ 55641.00472 $ & $   0.02549 $ & $   0.00121 $ & $  12.04150 $ & $ i$\\
$ 55641.00628 $ & $   0.02283 $ & $   0.00122 $ & $  12.03800 $ & $ i$\\
$ 55641.00781 $ & $   0.02287 $ & $   0.00121 $ & $  12.03800 $ & $ i$\\
$ 55641.00937 $ & $   0.02411 $ & $   0.00121 $ & $  12.04070 $ & $ i$\\
$ 55641.01101 $ & $   0.02174 $ & $   0.00121 $ & $  12.03620 $ & $ i$\\
$ 55641.01255 $ & $   0.02305 $ & $   0.00120 $ & $  12.03880 $ & $ i$\\
$ 55641.01409 $ & $   0.02263 $ & $   0.00124 $ & $  12.03810 $ & $ i$\\
$ 55641.01563 $ & $   0.02555 $ & $   0.00124 $ & $  12.04100 $ & $ i$\\
$ 55641.01719 $ & $   0.02675 $ & $   0.00123 $ & $  12.04230 $ & $ i$\\
$ 55641.01876 $ & $   0.02337 $ & $   0.00123 $ & $  12.03840 $ & $ i$\\
$ 55641.02040 $ & $   0.02442 $ & $   0.00122 $ & $  12.03950 $ & $ i$\\
$ 55641.02193 $ & $   0.02247 $ & $   0.00121 $ & $  12.03680 $ & $ i$\\
$ 55641.02349 $ & $   0.02524 $ & $   0.00124 $ & $  12.04010 $ & $ i$\\
$ 55641.02504 $ & $   0.02639 $ & $   0.00126 $ & $  12.04120 $ & $ i$\\
$ 55666.71920 $ & $  -0.00142 $ & $   0.00153 $ & $  11.49470 $ & $ r$\\
$ 55666.72072 $ & $   0.00043 $ & $   0.00149 $ & $  11.49620 $ & $ r$\\
$ 55666.72223 $ & $  -0.00300 $ & $   0.00151 $ & $  11.49030 $ & $ r$\\
$ 55666.72375 $ & $   0.00441 $ & $   0.00155 $ & $  11.50020 $ & $ r$\\
$ 55666.72527 $ & $   0.00010 $ & $   0.00161 $ & $  11.49530 $ & $ r$\\
$ 55666.72678 $ & $  -0.00166 $ & $   0.00170 $ & $  11.49320 $ & $ r$\\
$ 55666.72830 $ & $   0.00332 $ & $   0.00148 $ & $  11.49710 $ & $ r$\\
$ 55666.72982 $ & $   0.00002 $ & $   0.00150 $ & $  11.49390 $ & $ r$\\
$ 55666.73134 $ & $   0.00084 $ & $   0.00165 $ & $  11.49300 $ & $ r$\\
$ 55666.73286 $ & $  -0.00788 $ & $   0.00165 $ & $  11.48550 $ & $ r$\\
$ 55666.73438 $ & $  -0.00174 $ & $   0.00160 $ & $  11.49360 $ & $ r$\\
$ 55666.73589 $ & $   0.00330 $ & $   0.00192 $ & $  11.49860 $ & $ r$\\
$ 55666.73739 $ & $  -0.00471 $ & $   0.00176 $ & $  11.49010 $ & $ r$\\
$ 55666.74043 $ & $  -0.00116 $ & $   0.00166 $ & $  11.49300 $ & $ r$\\
$ 55666.74195 $ & $  -0.00606 $ & $   0.00170 $ & $  11.48990 $ & $ r$\\
$ 55666.74344 $ & $   0.00612 $ & $   0.00196 $ & $  11.50020 $ & $ r$\\
$ 55666.74495 $ & $  -0.00262 $ & $   0.00184 $ & $  11.49290 $ & $ r$\\
$ 55666.74649 $ & $  -0.00496 $ & $   0.00163 $ & $  11.48880 $ & $ r$\\
$ 55666.74802 $ & $   0.00276 $ & $   0.00197 $ & $  11.49350 $ & $ r$\\
$ 55666.74955 $ & $  -0.00107 $ & $   0.00159 $ & $  11.49450 $ & $ r$\\
$ 55666.75104 $ & $   0.00312 $ & $   0.00156 $ & $  11.49760 $ & $ r$\\
$ 55666.75258 $ & $   0.00038 $ & $   0.00158 $ & $  11.49460 $ & $ r$\\
$ 55666.75408 $ & $   0.00096 $ & $   0.00175 $ & $  11.49640 $ & $ r$\\
$ 55666.75561 $ & $   0.00411 $ & $   0.00175 $ & $  11.50020 $ & $ r$\\
$ 55666.75713 $ & $  -0.00394 $ & $   0.00158 $ & $  11.49100 $ & $ r$\\
$ 55666.75868 $ & $   0.00184 $ & $   0.00160 $ & $  11.49630 $ & $ r$\\
$ 55666.76021 $ & $   0.00148 $ & $   0.00167 $ & $  11.49570 $ & $ r$\\
$ 55666.76171 $ & $   0.00112 $ & $   0.00157 $ & $  11.49700 $ & $ r$\\
$ 55666.76323 $ & $   0.00333 $ & $   0.00147 $ & $  11.49850 $ & $ r$\\
$ 55666.76475 $ & $   0.00256 $ & $   0.00154 $ & $  11.49820 $ & $ r$\\
$ 55666.76630 $ & $   0.00457 $ & $   0.00148 $ & $  11.50080 $ & $ r$\\
$ 55666.76780 $ & $   0.00218 $ & $   0.00145 $ & $  11.49710 $ & $ r$\\
$ 55666.76933 $ & $   0.00269 $ & $   0.00151 $ & $  11.49740 $ & $ r$\\
$ 55666.77082 $ & $   0.00843 $ & $   0.00148 $ & $  11.49950 $ & $ r$\\
$ 55666.77388 $ & $   0.01139 $ & $   0.00151 $ & $  11.50770 $ & $ r$\\
$ 55666.77538 $ & $   0.01764 $ & $   0.00159 $ & $  11.51280 $ & $ r$\\
$ 55666.77689 $ & $   0.01720 $ & $   0.00155 $ & $  11.51250 $ & $ r$\\
$ 55666.77843 $ & $   0.01961 $ & $   0.00159 $ & $  11.51540 $ & $ r$\\
$ 55666.77995 $ & $   0.02214 $ & $   0.00160 $ & $  11.51850 $ & $ r$\\
$ 55666.78152 $ & $   0.01715 $ & $   0.00139 $ & $  11.51280 $ & $ r$\\
$ 55666.78302 $ & $   0.01874 $ & $   0.00155 $ & $  11.51380 $ & $ r$\\
$ 55666.78453 $ & $   0.01282 $ & $   0.00146 $ & $  11.50760 $ & $ r$\\
$ 55666.78606 $ & $   0.01892 $ & $   0.00148 $ & $  11.51450 $ & $ r$\\
$ 55666.78758 $ & $   0.02155 $ & $   0.00161 $ & $  11.51800 $ & $ r$\\
$ 55666.78911 $ & $   0.02181 $ & $   0.00194 $ & $  11.51700 $ & $ r$\\
$ 55666.79064 $ & $   0.01302 $ & $   0.00154 $ & $  11.50990 $ & $ r$\\
$ 55666.79215 $ & $   0.02159 $ & $   0.00155 $ & $  11.51650 $ & $ r$\\
$ 55666.79366 $ & $   0.02159 $ & $   0.00153 $ & $  11.51630 $ & $ r$\\
$ 55666.79517 $ & $   0.02377 $ & $   0.00148 $ & $  11.51890 $ & $ r$\\
$ 55666.79668 $ & $   0.02174 $ & $   0.00152 $ & $  11.51610 $ & $ r$\\
$ 55666.79819 $ & $   0.02381 $ & $   0.00171 $ & $  11.51860 $ & $ r$\\
$ 55666.79970 $ & $   0.02401 $ & $   0.00150 $ & $  11.51880 $ & $ r$\\
$ 55666.80275 $ & $   0.02408 $ & $   0.00139 $ & $  11.52120 $ & $ r$\\
$ 55666.80426 $ & $   0.02224 $ & $   0.00136 $ & $  11.51860 $ & $ r$\\
$ 55666.80579 $ & $   0.02353 $ & $   0.00146 $ & $  11.51880 $ & $ r$\\
$ 55666.80882 $ & $   0.02386 $ & $   0.00141 $ & $  11.52110 $ & $ r$\\
$ 55666.81033 $ & $   0.02110 $ & $   0.00148 $ & $  11.51610 $ & $ r$\\
$ 55666.81183 $ & $   0.03006 $ & $   0.00159 $ & $  11.52850 $ & $ r$\\
$ 55666.81334 $ & $   0.02377 $ & $   0.00178 $ & $  11.51880 $ & $ r$\\
$ 55666.81484 $ & $   0.02007 $ & $   0.00147 $ & $  11.51390 $ & $ r$\\
$ 55666.81635 $ & $   0.02372 $ & $   0.00147 $ & $  11.51830 $ & $ r$\\
$ 55666.81788 $ & $   0.02551 $ & $   0.00167 $ & $  11.52140 $ & $ r$\\
$ 55666.81941 $ & $   0.02798 $ & $   0.00153 $ & $  11.52350 $ & $ r$\\
$ 55666.82094 $ & $   0.02194 $ & $   0.00146 $ & $  11.51800 $ & $ r$\\
$ 55666.82245 $ & $   0.03112 $ & $   0.00144 $ & $  11.52630 $ & $ r$\\
$ 55666.82397 $ & $   0.02650 $ & $   0.00148 $ & $  11.52190 $ & $ r$\\
$ 55666.82549 $ & $   0.02028 $ & $   0.00138 $ & $  11.51630 $ & $ r$\\
$ 55666.82700 $ & $   0.02122 $ & $   0.00147 $ & $  11.51680 $ & $ r$\\
$ 55666.82852 $ & $   0.02223 $ & $   0.00133 $ & $  11.51760 $ & $ r$\\
$ 55666.83002 $ & $   0.02042 $ & $   0.00129 $ & $  11.51520 $ & $ r$\\
$ 55666.83153 $ & $   0.02173 $ & $   0.00132 $ & $  11.51680 $ & $ r$\\
$ 55666.83307 $ & $   0.02408 $ & $   0.00143 $ & $  11.51730 $ & $ r$\\
$ 55666.83458 $ & $   0.02660 $ & $   0.00134 $ & $  11.52070 $ & $ r$\\
$ 55666.83612 $ & $   0.02593 $ & $   0.00132 $ & $  11.52070 $ & $ r$\\
$ 55666.83766 $ & $   0.02555 $ & $   0.00133 $ & $  11.51980 $ & $ r$\\
$ 55666.83918 $ & $   0.02724 $ & $   0.00129 $ & $  11.52280 $ & $ r$\\
$ 55666.84069 $ & $   0.02389 $ & $   0.00126 $ & $  11.52000 $ & $ r$\\
$ 55666.84221 $ & $   0.02548 $ & $   0.00128 $ & $  11.52170 $ & $ r$\\
$ 55666.84373 $ & $   0.02032 $ & $   0.00134 $ & $  11.51610 $ & $ r$\\
$ 55666.84524 $ & $   0.02379 $ & $   0.00135 $ & $  11.51900 $ & $ r$\\
$ 55666.84676 $ & $   0.02515 $ & $   0.00134 $ & $  11.52170 $ & $ r$\\
$ 55666.84827 $ & $   0.02452 $ & $   0.00133 $ & $  11.52100 $ & $ r$\\
$ 55666.84981 $ & $   0.02019 $ & $   0.00134 $ & $  11.51700 $ & $ r$\\
$ 55666.85133 $ & $   0.01728 $ & $   0.00128 $ & $  11.51270 $ & $ r$\\
$ 55666.85285 $ & $   0.02010 $ & $   0.00132 $ & $  11.51700 $ & $ r$\\
$ 55666.85435 $ & $   0.02276 $ & $   0.00137 $ & $  11.51780 $ & $ r$\\
$ 55666.85590 $ & $   0.02413 $ & $   0.00136 $ & $  11.52030 $ & $ r$\\
$ 55666.85745 $ & $   0.02226 $ & $   0.00130 $ & $  11.51820 $ & $ r$\\
$ 55666.85897 $ & $   0.02193 $ & $   0.00131 $ & $  11.51800 $ & $ r$\\
$ 55666.86049 $ & $   0.02160 $ & $   0.00130 $ & $  11.51700 $ & $ r$\\
$ 55666.86199 $ & $   0.02463 $ & $   0.00132 $ & $  11.52070 $ & $ r$\\
$ 55666.86352 $ & $   0.01739 $ & $   0.00126 $ & $  11.51390 $ & $ r$\\
$ 55666.86501 $ & $   0.02016 $ & $   0.00132 $ & $  11.51620 $ & $ r$\\
$ 55666.86653 $ & $   0.02094 $ & $   0.00131 $ & $  11.51670 $ & $ r$\\
$ 55666.86802 $ & $   0.02118 $ & $   0.00133 $ & $  11.51580 $ & $ r$\\
$ 55666.86953 $ & $   0.01899 $ & $   0.00142 $ & $  11.51480 $ & $ r$\\
$ 55666.87103 $ & $   0.01800 $ & $   0.00140 $ & $  11.51200 $ & $ r$\\
$ 55666.87253 $ & $   0.01638 $ & $   0.00134 $ & $  11.51240 $ & $ r$\\
$ 55666.87406 $ & $   0.02083 $ & $   0.00133 $ & $  11.51770 $ & $ r$\\
$ 55666.87560 $ & $   0.02210 $ & $   0.00136 $ & $  11.51820 $ & $ r$\\
$ 55666.87715 $ & $   0.01682 $ & $   0.00142 $ & $  11.51370 $ & $ r$\\
$ 55666.87867 $ & $   0.01469 $ & $   0.00141 $ & $  11.51100 $ & $ r$\\
$ 55666.88016 $ & $   0.01668 $ & $   0.00145 $ & $  11.51330 $ & $ r$\\
$ 55666.88168 $ & $   0.01514 $ & $   0.00131 $ & $  11.51160 $ & $ r$\\
$ 55666.88320 $ & $   0.00597 $ & $   0.00127 $ & $  11.50170 $ & $ r$\\
$ 55666.88471 $ & $   0.00851 $ & $   0.00131 $ & $  11.50490 $ & $ r$\\
$ 55666.88622 $ & $   0.00913 $ & $   0.00133 $ & $  11.50470 $ & $ r$\\
$ 55666.88772 $ & $   0.00398 $ & $   0.00128 $ & $  11.50070 $ & $ r$\\
$ 55666.88925 $ & $   0.00208 $ & $   0.00131 $ & $  11.49900 $ & $ r$\\
$ 55666.89076 $ & $   0.00097 $ & $   0.00129 $ & $  11.49550 $ & $ r$\\
$ 55666.89228 $ & $  -0.00034 $ & $   0.00133 $ & $  11.49550 $ & $ r$\\
$ 55666.89383 $ & $   0.00064 $ & $   0.00132 $ & $  11.49700 $ & $ r$\\
$ 55666.89536 $ & $   0.00471 $ & $   0.00134 $ & $  11.50120 $ & $ r$\\
$ 55666.89688 $ & $  -0.00188 $ & $   0.00128 $ & $  11.49330 $ & $ r$\\
$ 55666.89842 $ & $   0.00046 $ & $   0.00127 $ & $  11.49630 $ & $ r$\\
$ 55666.89993 $ & $   0.00241 $ & $   0.00127 $ & $  11.49780 $ & $ r$\\
$ 55666.90147 $ & $   0.00429 $ & $   0.00132 $ & $  11.50030 $ & $ r$\\
$ 55666.90298 $ & $   0.00526 $ & $   0.00147 $ & $  11.50150 $ & $ r$\\
$ 55666.90451 $ & $   0.00103 $ & $   0.00134 $ & $  11.49720 $ & $ r$\\
$ 55666.90604 $ & $   0.00179 $ & $   0.00134 $ & $  11.49750 $ & $ r$\\
$ 55666.90754 $ & $   0.00141 $ & $   0.00129 $ & $  11.49840 $ & $ r$\\
$ 55666.90910 $ & $  -0.00015 $ & $   0.00133 $ & $  11.49520 $ & $ r$\\
$ 55666.91061 $ & $   0.00082 $ & $   0.00134 $ & $  11.49580 $ & $ r$\\
$ 55666.91214 $ & $   0.00157 $ & $   0.00142 $ & $  11.49680 $ & $ r$\\
$ 55666.91364 $ & $  -0.00037 $ & $   0.00139 $ & $  11.49480 $ & $ r$\\
$ 55666.91671 $ & $  -0.00610 $ & $   0.00139 $ & $  11.48860 $ & $ r$\\
$ 55666.91824 $ & $   0.00078 $ & $   0.00139 $ & $  11.49580 $ & $ r$\\
$ 55666.91978 $ & $  -0.00156 $ & $   0.00146 $ & $  11.49630 $ & $ r$\\
$ 55666.92130 $ & $   0.00076 $ & $   0.00136 $ & $  11.49700 $ & $ r$\\
$ 55666.92282 $ & $  -0.00023 $ & $   0.00148 $ & $  11.49480 $ & $ r$\\
$ 55666.92437 $ & $   0.00386 $ & $   0.00137 $ & $  11.49920 $ & $ r$\\
$ 55666.92590 $ & $  -0.00085 $ & $   0.00150 $ & $  11.49590 $ & $ r$\\
$ 55666.92742 $ & $  -0.00182 $ & $   0.00148 $ & $  11.49340 $ & $ r$\\
$ 55666.92893 $ & $  -0.00304 $ & $   0.00139 $ & $  11.49200 $ & $ r$\\
$ 55666.93044 $ & $  -0.00147 $ & $   0.00150 $ & $  11.49660 $ & $ r$\\
$ 55666.93194 $ & $   0.00287 $ & $   0.00142 $ & $  11.50280 $ & $ r$\\
$ 55666.93347 $ & $   0.00054 $ & $   0.00140 $ & $  11.49580 $ & $ r$\\
$ 55666.93500 $ & $   0.00063 $ & $   0.00146 $ & $  11.49740 $ & $ r$\\
$ 55666.93655 $ & $   0.00183 $ & $   0.00143 $ & $  11.49630 $ & $ r$\\
$ 55666.93809 $ & $  -0.00176 $ & $   0.00152 $ & $  11.49370 $ & $ r$\\
$ 55666.93961 $ & $  -0.00010 $ & $   0.00155 $ & $  11.49570 $ & $ r$\\
$ 55666.94115 $ & $   0.00089 $ & $   0.00152 $ & $  11.49540 $ & $ r$\\
$ 55666.94268 $ & $   0.00308 $ & $   0.00154 $ & $  11.49690 $ & $ r$\\
$ 55666.94418 $ & $  -0.00184 $ & $   0.00150 $ & $  11.49350 $ & $ r$\\
$ 55666.94571 $ & $  -0.00282 $ & $   0.00154 $ & $  11.49010 $ & $ r$\\
$ 55666.94721 $ & $  -0.00498 $ & $   0.00156 $ & $  11.48890 $ & $ r$\\
$ 55666.94875 $ & $  -0.00154 $ & $   0.00158 $ & $  11.49220 $ & $ r$\\
$ 55666.95025 $ & $  -0.00310 $ & $   0.00157 $ & $  11.49220 $ & $ r$\\
$ 55666.95177 $ & $  -0.00065 $ & $   0.00167 $ & $  11.49470 $ & $ r$\\
$ 55666.95330 $ & $   0.00183 $ & $   0.00145 $ & $  11.49710 $ & $ r$\\
$ 55666.95481 $ & $   0.00304 $ & $   0.00147 $ & $  11.49980 $ & $ r$\\
$ 55666.95632 $ & $  -0.00132 $ & $   0.00166 $ & $  11.49250 $ & $ r$\\
$ 55666.95784 $ & $   0.00007 $ & $   0.00163 $ & $  11.49490 $ & $ r$\\
$ 55666.95937 $ & $   0.00006 $ & $   0.00161 $ & $  11.49470 $ & $ r$\\
$ 55666.96091 $ & $  -0.00191 $ & $   0.00168 $ & $  11.49320 $ & $ r$\\
$ 55666.96242 $ & $   0.00064 $ & $   0.00163 $ & $  11.49730 $ & $ r$\\
$ 55666.96391 $ & $  -0.00046 $ & $   0.00165 $ & $  11.49430 $ & $ r$\\
$ 55666.96695 $ & $  -0.00317 $ & $   0.00150 $ & $  11.49130 $ & $ r$\\
$ 55666.96847 $ & $  -0.00350 $ & $   0.00147 $ & $  11.49240 $ & $ r$\\
$ 55666.96997 $ & $   0.00241 $ & $   0.00149 $ & $  11.49870 $ & $ r$\\
$ 55666.97152 $ & $  -0.00169 $ & $   0.00153 $ & $  11.49360 $ & $ r$\\
$ 55666.97305 $ & $  -0.00360 $ & $   0.00167 $ & $  11.49090 $ & $ r$\\
$ 55666.97457 $ & $   0.00399 $ & $   0.00192 $ & $  11.49740 $ & $ r$\\
$ 55666.97910 $ & $  -0.00198 $ & $   0.00176 $ & $  11.49320 $ & $ r$\\
$ 55666.98364 $ & $  -0.00098 $ & $   0.00167 $ & $  11.49310 $ & $ r$\\
$ 55666.98517 $ & $   0.00122 $ & $   0.00178 $ & $  11.49470 $ & $ r$\\
$ 55666.98667 $ & $   0.00088 $ & $   0.00185 $ & $  11.49600 $ & $ r$\\
$ 55666.98820 $ & $   0.00416 $ & $   0.00151 $ & $  11.49830 $ & $ r$\\
$ 55666.98970 $ & $   0.00007 $ & $   0.00164 $ & $  11.49540 $ & $ r$\\
$ 55666.99122 $ & $   0.00458 $ & $   0.00180 $ & $  11.49970 $ & $ r$\\
$ 55666.99428 $ & $   0.00046 $ & $   0.00216 $ & $  11.49810 $ & $ r$\\
$ 55666.99581 $ & $  -0.00399 $ & $   0.00190 $ & $  11.48970 $ & $ r$\\
$ 55667.00189 $ & $   0.00072 $ & $   0.00206 $ & $  11.49580 $ & $ r$\\
$ 55667.00339 $ & $   0.00261 $ & $   0.00181 $ & $  11.49720 $ & $ r$\\
$ 55667.00489 $ & $   0.00184 $ & $   0.00212 $ & $  11.49640 $ & $ r$\\
$ 55667.00641 $ & $  -0.00314 $ & $   0.00202 $ & $  11.48930 $ & $ r$\\
$ 55666.82114 $ & $   0.02224 $ & $   0.00104 $ & $  11.77570 $ & $ i$\\
$ 55666.82270 $ & $   0.02518 $ & $   0.00105 $ & $  11.77820 $ & $ i$\\
$ 55666.82425 $ & $   0.02385 $ & $   0.00105 $ & $  11.77710 $ & $ i$\\
$ 55666.82579 $ & $   0.02342 $ & $   0.00104 $ & $  11.77690 $ & $ i$\\
$ 55666.82735 $ & $   0.02442 $ & $   0.00104 $ & $  11.77700 $ & $ i$\\
$ 55666.82888 $ & $   0.02122 $ & $   0.00106 $ & $  11.77410 $ & $ i$\\
$ 55666.83043 $ & $   0.02442 $ & $   0.00105 $ & $  11.77630 $ & $ i$\\
$ 55666.83199 $ & $   0.02535 $ & $   0.00105 $ & $  11.77750 $ & $ i$\\
$ 55666.83356 $ & $   0.02537 $ & $   0.00104 $ & $  11.77680 $ & $ i$\\
$ 55666.83511 $ & $   0.02133 $ & $   0.00104 $ & $  11.77350 $ & $ i$\\
$ 55666.83667 $ & $   0.02253 $ & $   0.00104 $ & $  11.77550 $ & $ i$\\
$ 55666.83820 $ & $   0.02418 $ & $   0.00105 $ & $  11.77650 $ & $ i$\\
$ 55666.83977 $ & $   0.02417 $ & $   0.00105 $ & $  11.77650 $ & $ i$\\
$ 55666.84133 $ & $   0.02576 $ & $   0.00106 $ & $  11.77700 $ & $ i$\\
$ 55666.84287 $ & $   0.02370 $ & $   0.00106 $ & $  11.77590 $ & $ i$\\
$ 55666.84443 $ & $   0.02072 $ & $   0.00105 $ & $  11.77280 $ & $ i$\\
$ 55666.84598 $ & $   0.02208 $ & $   0.00107 $ & $  11.77450 $ & $ i$\\
$ 55666.84753 $ & $   0.02163 $ & $   0.00106 $ & $  11.77340 $ & $ i$\\
$ 55666.84906 $ & $   0.02066 $ & $   0.00106 $ & $  11.77290 $ & $ i$\\
$ 55666.85061 $ & $   0.02257 $ & $   0.00106 $ & $  11.77430 $ & $ i$\\
$ 55666.85235 $ & $   0.02319 $ & $   0.00106 $ & $  11.77510 $ & $ i$\\
$ 55666.85389 $ & $   0.02215 $ & $   0.00105 $ & $  11.77460 $ & $ i$\\
$ 55666.85545 $ & $   0.02294 $ & $   0.00106 $ & $  11.77520 $ & $ i$\\
$ 55666.85698 $ & $   0.02496 $ & $   0.00106 $ & $  11.77720 $ & $ i$\\
$ 55666.85855 $ & $   0.02363 $ & $   0.00105 $ & $  11.77530 $ & $ i$\\
$ 55666.86011 $ & $   0.02148 $ & $   0.00106 $ & $  11.77400 $ & $ i$\\
$ 55666.86165 $ & $   0.02374 $ & $   0.00105 $ & $  11.77570 $ & $ i$\\
$ 55666.86320 $ & $   0.02304 $ & $   0.00106 $ & $  11.77550 $ & $ i$\\
$ 55666.86474 $ & $   0.02153 $ & $   0.00105 $ & $  11.77410 $ & $ i$\\
$ 55666.86631 $ & $   0.01931 $ & $   0.00105 $ & $  11.77140 $ & $ i$\\
$ 55666.86786 $ & $   0.01935 $ & $   0.00105 $ & $  11.77220 $ & $ i$\\
$ 55666.86940 $ & $   0.01879 $ & $   0.00105 $ & $  11.77080 $ & $ i$\\
$ 55666.87095 $ & $   0.01804 $ & $   0.00105 $ & $  11.77040 $ & $ i$\\
$ 55666.87250 $ & $   0.01947 $ & $   0.00105 $ & $  11.77150 $ & $ i$\\
$ 55666.87405 $ & $   0.01973 $ & $   0.00106 $ & $  11.77270 $ & $ i$\\
$ 55666.87561 $ & $   0.01667 $ & $   0.00105 $ & $  11.76980 $ & $ i$\\
$ 55666.87715 $ & $   0.01815 $ & $   0.00109 $ & $  11.77080 $ & $ i$\\
$ 55666.87870 $ & $   0.01774 $ & $   0.00107 $ & $  11.77030 $ & $ i$\\
$ 55666.88025 $ & $   0.01483 $ & $   0.00105 $ & $  11.76710 $ & $ i$\\
$ 55666.88180 $ & $   0.01024 $ & $   0.00105 $ & $  11.76330 $ & $ i$\\
$ 55666.88456 $ & $   0.00814 $ & $   0.00105 $ & $  11.76100 $ & $ i$\\
$ 55666.88610 $ & $   0.00656 $ & $   0.00105 $ & $  11.75830 $ & $ i$\\
$ 55666.88766 $ & $   0.00581 $ & $   0.00105 $ & $  11.75830 $ & $ i$\\
$ 55666.88921 $ & $   0.00341 $ & $   0.00105 $ & $  11.75580 $ & $ i$\\
$ 55666.89075 $ & $  -0.00094 $ & $   0.00104 $ & $  11.75060 $ & $ i$\\
$ 55666.89231 $ & $   0.00128 $ & $   0.00105 $ & $  11.75290 $ & $ i$\\
$ 55666.89385 $ & $   0.00079 $ & $   0.00105 $ & $  11.75250 $ & $ i$\\
$ 55666.89555 $ & $   0.00052 $ & $   0.00104 $ & $  11.75230 $ & $ i$\\
$ 55666.89709 $ & $   0.00122 $ & $   0.00104 $ & $  11.75300 $ & $ i$\\
$ 55666.89885 $ & $   0.00081 $ & $   0.00105 $ & $  11.75310 $ & $ i$\\
$ 55666.90038 $ & $  -0.00060 $ & $   0.00105 $ & $  11.75190 $ & $ i$\\
$ 55666.90194 $ & $   0.00175 $ & $   0.00105 $ & $  11.75290 $ & $ i$\\
$ 55666.90348 $ & $   0.00061 $ & $   0.00104 $ & $  11.75300 $ & $ i$\\
$ 55666.90502 $ & $  -0.00009 $ & $   0.00106 $ & $  11.75160 $ & $ i$\\
$ 55666.90657 $ & $  -0.00177 $ & $   0.00107 $ & $  11.74970 $ & $ i$\\
$ 55666.90812 $ & $   0.00178 $ & $   0.00110 $ & $  11.75370 $ & $ i$\\
$ 55666.90966 $ & $   0.00014 $ & $   0.00107 $ & $  11.75230 $ & $ i$\\
$ 55666.91120 $ & $  -0.00072 $ & $   0.00109 $ & $  11.75110 $ & $ i$\\
$ 55666.91274 $ & $   0.00075 $ & $   0.00110 $ & $  11.75280 $ & $ i$\\
$ 55666.91428 $ & $  -0.00394 $ & $   0.00108 $ & $  11.74920 $ & $ i$\\
$ 55666.91610 $ & $   0.00043 $ & $   0.00107 $ & $  11.75220 $ & $ i$\\
$ 55666.91766 $ & $   0.00156 $ & $   0.00107 $ & $  11.75500 $ & $ i$\\
$ 55666.91921 $ & $  -0.00006 $ & $   0.00108 $ & $  11.75170 $ & $ i$\\
$ 55666.92076 $ & $   0.00073 $ & $   0.00106 $ & $  11.75260 $ & $ i$\\
$ 55666.92229 $ & $  -0.00081 $ & $   0.00106 $ & $  11.75110 $ & $ i$\\
$ 55666.92384 $ & $   0.00009 $ & $   0.00106 $ & $  11.75220 $ & $ i$\\
$ 55666.92538 $ & $   0.00112 $ & $   0.00107 $ & $  11.75480 $ & $ i$\\
$ 55666.92692 $ & $  -0.00032 $ & $   0.00106 $ & $  11.75400 $ & $ i$\\
$ 55666.92843 $ & $  -0.00042 $ & $   0.00107 $ & $  11.75280 $ & $ i$\\
$ 55666.92997 $ & $  -0.00039 $ & $   0.00107 $ & $  11.75280 $ & $ i$\\
$ 55666.93154 $ & $  -0.00077 $ & $   0.00107 $ & $  11.75230 $ & $ i$\\
$ 55666.93309 $ & $   0.00059 $ & $   0.00108 $ & $  11.75340 $ & $ i$\\
$ 55666.93463 $ & $   0.00028 $ & $   0.00106 $ & $  11.75440 $ & $ i$\\
$ 55666.93618 $ & $  -0.00315 $ & $   0.00105 $ & $  11.75190 $ & $ i$\\
$ 55666.93770 $ & $   0.00288 $ & $   0.00106 $ & $  11.75750 $ & $ i$\\
$ 55666.93927 $ & $   0.00013 $ & $   0.00106 $ & $  11.75390 $ & $ i$\\
$ 55666.94084 $ & $   0.00079 $ & $   0.00106 $ & $  11.75450 $ & $ i$\\
$ 55666.94251 $ & $  -0.00084 $ & $   0.00105 $ & $  11.75310 $ & $ i$\\
$ 55666.94407 $ & $  -0.00114 $ & $   0.00105 $ & $  11.75200 $ & $ i$\\
$ 55666.94562 $ & $  -0.00242 $ & $   0.00105 $ & $  11.75200 $ & $ i$\\
$ 55666.94759 $ & $  -0.00008 $ & $   0.00104 $ & $  11.75520 $ & $ i$\\
$ 55666.94915 $ & $  -0.00065 $ & $   0.00105 $ & $  11.75420 $ & $ i$\\
$ 55666.95070 $ & $   0.00242 $ & $   0.00105 $ & $  11.75770 $ & $ i$\\
$ 55666.95225 $ & $   0.00063 $ & $   0.00104 $ & $  11.75630 $ & $ i$\\
$ 55666.95382 $ & $   0.00049 $ & $   0.00103 $ & $  11.75670 $ & $ i$\\
$ 55709.65702 $ & $  -0.00018 $ & $   0.00095 $ & $  11.69810 $ & $ i$\\
$ 55709.65860 $ & $  -0.00254 $ & $   0.00095 $ & $  11.69640 $ & $ i$\\
$ 55709.66015 $ & $   0.00183 $ & $   0.00094 $ & $  11.70000 $ & $ i$\\
$ 55709.66169 $ & $   0.00088 $ & $   0.00095 $ & $  11.69830 $ & $ i$\\
$ 55709.66325 $ & $   0.00066 $ & $   0.00095 $ & $  11.69830 $ & $ i$\\
$ 55709.66480 $ & $   0.00048 $ & $   0.00094 $ & $  11.69780 $ & $ i$\\
$ 55709.66635 $ & $  -0.00048 $ & $   0.00094 $ & $  11.69590 $ & $ i$\\
$ 55709.66790 $ & $   0.00027 $ & $   0.00095 $ & $  11.69680 $ & $ i$\\
$ 55709.66947 $ & $   0.00359 $ & $   0.00095 $ & $  11.69970 $ & $ i$\\
$ 55709.67103 $ & $  -0.00051 $ & $   0.00095 $ & $  11.69550 $ & $ i$\\
$ 55709.67257 $ & $   0.00276 $ & $   0.00095 $ & $  11.69930 $ & $ i$\\
$ 55709.67411 $ & $  -0.00206 $ & $   0.00094 $ & $  11.69400 $ & $ i$\\
$ 55709.67567 $ & $  -0.00218 $ & $   0.00095 $ & $  11.69500 $ & $ i$\\
$ 55709.67723 $ & $  -0.00051 $ & $   0.00095 $ & $  11.69500 $ & $ i$\\
$ 55709.67879 $ & $   0.00085 $ & $   0.00094 $ & $  11.69550 $ & $ i$\\
$ 55709.68034 $ & $   0.00111 $ & $   0.00095 $ & $  11.69600 $ & $ i$\\
$ 55709.68190 $ & $  -0.00075 $ & $   0.00094 $ & $  11.69460 $ & $ i$\\
$ 55709.68346 $ & $  -0.00084 $ & $   0.00095 $ & $  11.69480 $ & $ i$\\
$ 55709.68502 $ & $   0.00081 $ & $   0.00094 $ & $  11.69560 $ & $ i$\\
$ 55709.68657 $ & $   0.00019 $ & $   0.00095 $ & $  11.69540 $ & $ i$\\
$ 55709.68812 $ & $  -0.00036 $ & $   0.00095 $ & $  11.69450 $ & $ i$\\
$ 55709.68971 $ & $   0.00160 $ & $   0.00095 $ & $  11.69670 $ & $ i$\\
$ 55709.69125 $ & $   0.00209 $ & $   0.00095 $ & $  11.69740 $ & $ i$\\
$ 55709.69280 $ & $   0.00045 $ & $   0.00095 $ & $  11.69650 $ & $ i$\\
$ 55709.69435 $ & $   0.00122 $ & $   0.00096 $ & $  11.69690 $ & $ i$\\
$ 55709.69590 $ & $  -0.00159 $ & $   0.00094 $ & $  11.69480 $ & $ i$\\
$ 55709.69743 $ & $  -0.00147 $ & $   0.00095 $ & $  11.69480 $ & $ i$\\
$ 55709.69894 $ & $  -0.00118 $ & $   0.00095 $ & $  11.69460 $ & $ i$\\
$ 55709.70049 $ & $  -0.00112 $ & $   0.00095 $ & $  11.69500 $ & $ i$\\
$ 55709.70205 $ & $   0.00196 $ & $   0.00095 $ & $  11.69770 $ & $ i$\\
$ 55709.70357 $ & $  -0.00028 $ & $   0.00095 $ & $  11.69640 $ & $ i$\\
$ 55709.70512 $ & $  -0.00192 $ & $   0.00095 $ & $  11.69310 $ & $ i$\\
$ 55709.70666 $ & $  -0.00120 $ & $   0.00095 $ & $  11.69330 $ & $ i$\\
$ 55709.70975 $ & $   0.00064 $ & $   0.00095 $ & $  11.69670 $ & $ i$\\
$ 55709.71132 $ & $   0.00095 $ & $   0.00095 $ & $  11.69620 $ & $ i$\\
$ 55709.71284 $ & $  -0.00044 $ & $   0.00095 $ & $  11.69420 $ & $ i$\\
$ 55709.71441 $ & $  -0.00117 $ & $   0.00095 $ & $  11.69430 $ & $ i$\\
$ 55709.71597 $ & $  -0.00105 $ & $   0.00095 $ & $  11.69430 $ & $ i$\\
$ 55709.71752 $ & $  -0.00050 $ & $   0.00095 $ & $  11.69430 $ & $ i$\\
$ 55709.71908 $ & $   0.00117 $ & $   0.00095 $ & $  11.69630 $ & $ i$\\
$ 55709.72070 $ & $  -0.00174 $ & $   0.00095 $ & $  11.69450 $ & $ i$\\
$ 55709.72224 $ & $  -0.00111 $ & $   0.00095 $ & $  11.69480 $ & $ i$\\
$ 55709.72378 $ & $   0.00051 $ & $   0.00095 $ & $  11.69660 $ & $ i$\\
$ 55709.72533 $ & $  -0.00131 $ & $   0.00095 $ & $  11.69420 $ & $ i$\\
$ 55709.72688 $ & $   0.00104 $ & $   0.00095 $ & $  11.69720 $ & $ i$\\
$ 55709.72842 $ & $   0.00010 $ & $   0.00095 $ & $  11.69630 $ & $ i$\\
$ 55709.72997 $ & $   0.00203 $ & $   0.00094 $ & $  11.69810 $ & $ i$\\
$ 55709.73152 $ & $  -0.00314 $ & $   0.00095 $ & $  11.69350 $ & $ i$\\
$ 55709.73307 $ & $   0.00094 $ & $   0.00096 $ & $  11.69680 $ & $ i$\\
$ 55709.73461 $ & $  -0.00116 $ & $   0.00096 $ & $  11.69530 $ & $ i$\\
$ 55709.73616 $ & $  -0.00059 $ & $   0.00095 $ & $  11.69540 $ & $ i$\\
$ 55709.73771 $ & $   0.00137 $ & $   0.00095 $ & $  11.69720 $ & $ i$\\
$ 55709.73927 $ & $  -0.00057 $ & $   0.00096 $ & $  11.69590 $ & $ i$\\
$ 55709.74080 $ & $   0.00008 $ & $   0.00095 $ & $  11.69680 $ & $ i$\\
$ 55709.74237 $ & $   0.00186 $ & $   0.00095 $ & $  11.69810 $ & $ i$\\
$ 55709.74391 $ & $  -0.00123 $ & $   0.00095 $ & $  11.69560 $ & $ i$\\
$ 55709.74545 $ & $   0.00180 $ & $   0.00095 $ & $  11.69780 $ & $ i$\\
$ 55709.74700 $ & $  -0.00010 $ & $   0.00095 $ & $  11.69610 $ & $ i$\\
$ 55709.74854 $ & $  -0.00088 $ & $   0.00095 $ & $  11.69580 $ & $ i$\\
$ 55709.75016 $ & $  -0.00151 $ & $   0.00095 $ & $  11.69560 $ & $ i$\\
$ 55709.75172 $ & $   0.00131 $ & $   0.00095 $ & $  11.69780 $ & $ i$\\
$ 55709.75326 $ & $   0.00194 $ & $   0.00095 $ & $  11.69840 $ & $ i$\\
$ 55709.75481 $ & $  -0.00072 $ & $   0.00094 $ & $  11.69570 $ & $ i$\\
$ 55709.75634 $ & $   0.00044 $ & $   0.00095 $ & $  11.69620 $ & $ i$\\
$ 55709.75790 $ & $  -0.00029 $ & $   0.00095 $ & $  11.69630 $ & $ i$\\
$ 55709.75945 $ & $   0.00095 $ & $   0.00095 $ & $  11.69710 $ & $ i$\\
$ 55709.76099 $ & $   0.00043 $ & $   0.00096 $ & $  11.69750 $ & $ i$\\
$ 55709.76253 $ & $  -0.00158 $ & $   0.00095 $ & $  11.69400 $ & $ i$\\
$ 55709.76408 $ & $  -0.00046 $ & $   0.00096 $ & $  11.69510 $ & $ i$\\
$ 55709.76562 $ & $  -0.00096 $ & $   0.00096 $ & $  11.69560 $ & $ i$\\
$ 55709.76718 $ & $   0.00133 $ & $   0.00096 $ & $  11.69780 $ & $ i$\\
$ 55709.76872 $ & $  -0.00133 $ & $   0.00096 $ & $  11.69450 $ & $ i$\\
$ 55709.77028 $ & $  -0.00138 $ & $   0.00095 $ & $  11.69490 $ & $ i$\\
$ 55709.77182 $ & $   0.00182 $ & $   0.00096 $ & $  11.69810 $ & $ i$\\
$ 55709.77338 $ & $  -0.00139 $ & $   0.00095 $ & $  11.69460 $ & $ i$\\
$ 55709.77492 $ & $   0.00041 $ & $   0.00095 $ & $  11.69680 $ & $ i$\\
$ 55709.77647 $ & $  -0.00003 $ & $   0.00096 $ & $  11.69630 $ & $ i$\\
$ 55709.77803 $ & $   0.00247 $ & $   0.00096 $ & $  11.69900 $ & $ i$\\
$ 55709.77958 $ & $  -0.00030 $ & $   0.00096 $ & $  11.69620 $ & $ i$\\
$ 55709.78116 $ & $   0.00478 $ & $   0.00096 $ & $  11.70170 $ & $ i$\\
$ 55709.78271 $ & $   0.00647 $ & $   0.00096 $ & $  11.70340 $ & $ i$\\
$ 55709.78425 $ & $   0.00721 $ & $   0.00096 $ & $  11.70370 $ & $ i$\\
$ 55709.78580 $ & $   0.00732 $ & $   0.00097 $ & $  11.70420 $ & $ i$\\
$ 55709.78734 $ & $   0.01441 $ & $   0.00096 $ & $  11.71120 $ & $ i$\\
$ 55709.78890 $ & $   0.01582 $ & $   0.00096 $ & $  11.71290 $ & $ i$\\
$ 55709.79047 $ & $   0.01626 $ & $   0.00097 $ & $  11.71290 $ & $ i$\\
$ 55709.79204 $ & $   0.01797 $ & $   0.00097 $ & $  11.71480 $ & $ i$\\
$ 55709.79360 $ & $   0.01729 $ & $   0.00097 $ & $  11.71380 $ & $ i$\\
$ 55709.79518 $ & $   0.01771 $ & $   0.00097 $ & $  11.71400 $ & $ i$\\
$ 55709.79673 $ & $   0.01935 $ & $   0.00097 $ & $  11.71600 $ & $ i$\\
$ 55709.79827 $ & $   0.02129 $ & $   0.00097 $ & $  11.71730 $ & $ i$\\
$ 55709.79983 $ & $   0.02109 $ & $   0.00098 $ & $  11.71750 $ & $ i$\\
$ 55709.80138 $ & $   0.02090 $ & $   0.00097 $ & $  11.71670 $ & $ i$\\
$ 55709.80293 $ & $   0.02194 $ & $   0.00098 $ & $  11.71820 $ & $ i$\\
$ 55709.80449 $ & $   0.01924 $ & $   0.00098 $ & $  11.71530 $ & $ i$\\
$ 55709.80611 $ & $   0.02093 $ & $   0.00098 $ & $  11.71710 $ & $ i$\\
$ 55709.80765 $ & $   0.02125 $ & $   0.00098 $ & $  11.71720 $ & $ i$\\
$ 55709.80920 $ & $   0.02266 $ & $   0.00098 $ & $  11.71890 $ & $ i$\\
$ 55709.81075 $ & $   0.02194 $ & $   0.00097 $ & $  11.71810 $ & $ i$\\
$ 55709.81234 $ & $   0.02373 $ & $   0.00098 $ & $  11.72100 $ & $ i$\\
$ 55709.81389 $ & $   0.02282 $ & $   0.00098 $ & $  11.71830 $ & $ i$\\
$ 55709.81543 $ & $   0.02472 $ & $   0.00098 $ & $  11.72180 $ & $ i$\\
$ 55709.81698 $ & $   0.02224 $ & $   0.00098 $ & $  11.72010 $ & $ i$\\
$ 55709.81853 $ & $   0.02119 $ & $   0.00097 $ & $  11.71950 $ & $ i$\\
$ 55709.82006 $ & $   0.02315 $ & $   0.00097 $ & $  11.72140 $ & $ i$\\
$ 55709.82161 $ & $   0.02465 $ & $   0.00098 $ & $  11.72240 $ & $ i$\\
$ 55709.82320 $ & $   0.02549 $ & $   0.00097 $ & $  11.72290 $ & $ i$\\
$ 55709.82475 $ & $   0.02370 $ & $   0.00098 $ & $  11.72200 $ & $ i$\\
$ 55709.82630 $ & $   0.02353 $ & $   0.00098 $ & $  11.72120 $ & $ i$\\
$ 55709.82786 $ & $   0.02095 $ & $   0.00098 $ & $  11.71890 $ & $ i$\\
$ 55709.82943 $ & $   0.02293 $ & $   0.00098 $ & $  11.72090 $ & $ i$\\
$ 55709.83097 $ & $   0.02601 $ & $   0.00098 $ & $  11.72360 $ & $ i$\\
$ 55709.83251 $ & $   0.02549 $ & $   0.00099 $ & $  11.72360 $ & $ i$\\
$ 55709.83408 $ & $   0.02071 $ & $   0.00098 $ & $  11.71850 $ & $ i$\\
$ 55709.83564 $ & $   0.02487 $ & $   0.00098 $ & $  11.72210 $ & $ i$\\
$ 55709.83717 $ & $   0.02422 $ & $   0.00098 $ & $  11.72230 $ & $ i$\\
$ 55709.83873 $ & $   0.02198 $ & $   0.00098 $ & $  11.71970 $ & $ i$\\
$ 55709.84029 $ & $   0.02482 $ & $   0.00099 $ & $  11.72240 $ & $ i$\\
$ 55709.84183 $ & $   0.02198 $ & $   0.00098 $ & $  11.72010 $ & $ i$\\
$ 55709.84343 $ & $   0.02098 $ & $   0.00098 $ & $  11.71870 $ & $ i$\\
$ 55709.84497 $ & $   0.02370 $ & $   0.00098 $ & $  11.72160 $ & $ i$\\
$ 55709.84652 $ & $   0.02237 $ & $   0.00098 $ & $  11.72050 $ & $ i$\\
$ 55709.84806 $ & $   0.02480 $ & $   0.00099 $ & $  11.72330 $ & $ i$\\
$ 55709.84961 $ & $   0.02409 $ & $   0.00098 $ & $  11.72280 $ & $ i$\\
$ 55709.85116 $ & $   0.02500 $ & $   0.00099 $ & $  11.72320 $ & $ i$\\
$ 55709.85271 $ & $   0.02567 $ & $   0.00098 $ & $  11.72400 $ & $ i$\\
$ 55709.85425 $ & $   0.02502 $ & $   0.00098 $ & $  11.72340 $ & $ i$\\
$ 55709.85580 $ & $   0.02339 $ & $   0.00098 $ & $  11.72200 $ & $ i$\\
$ 55709.85734 $ & $   0.02310 $ & $   0.00099 $ & $  11.72140 $ & $ i$\\
$ 55709.85888 $ & $   0.02430 $ & $   0.00099 $ & $  11.72260 $ & $ i$\\
$ 55709.86043 $ & $   0.02429 $ & $   0.00099 $ & $  11.72310 $ & $ i$\\
$ 55709.86198 $ & $   0.02091 $ & $   0.00098 $ & $  11.71960 $ & $ i$\\
$ 55709.86351 $ & $   0.02258 $ & $   0.00099 $ & $  11.72130 $ & $ i$\\
$ 55709.86507 $ & $   0.02465 $ & $   0.00098 $ & $  11.72290 $ & $ i$\\
$ 55709.86660 $ & $   0.02472 $ & $   0.00099 $ & $  11.72350 $ & $ i$\\
$ 55709.86816 $ & $   0.02242 $ & $   0.00098 $ & $  11.72210 $ & $ i$\\
$ 55709.86971 $ & $   0.02091 $ & $   0.00098 $ & $  11.71960 $ & $ i$\\
$ 55709.87139 $ & $   0.02293 $ & $   0.00097 $ & $  11.72180 $ & $ i$\\
$ 55709.87294 $ & $   0.02238 $ & $   0.00099 $ & $  11.72180 $ & $ i$\\
$ 55709.87448 $ & $   0.02089 $ & $   0.00099 $ & $  11.72040 $ & $ i$\\
$ 55709.87604 $ & $   0.01975 $ & $   0.00098 $ & $  11.71920 $ & $ i$\\
$ 55709.87757 $ & $   0.01955 $ & $   0.00098 $ & $  11.71970 $ & $ i$\\
$ 55709.87911 $ & $   0.02187 $ & $   0.00099 $ & $  11.72150 $ & $ i$\\
$ 55709.88067 $ & $   0.02195 $ & $   0.00098 $ & $  11.72130 $ & $ i$\\
$ 55709.88221 $ & $   0.02136 $ & $   0.00099 $ & $  11.72040 $ & $ i$\\
$ 55709.88375 $ & $   0.01976 $ & $   0.00099 $ & $  11.71960 $ & $ i$\\
$ 55709.88529 $ & $   0.02112 $ & $   0.00099 $ & $  11.71990 $ & $ i$\\
$ 55709.88686 $ & $   0.01901 $ & $   0.00099 $ & $  11.71780 $ & $ i$\\
$ 55709.88839 $ & $   0.01648 $ & $   0.00098 $ & $  11.71600 $ & $ i$\\
$ 55709.88995 $ & $   0.01640 $ & $   0.00098 $ & $  11.71610 $ & $ i$\\
$ 55709.89151 $ & $   0.01539 $ & $   0.00098 $ & $  11.71540 $ & $ i$\\
$ 55709.89307 $ & $   0.01499 $ & $   0.00099 $ & $  11.71580 $ & $ i$\\
$ 55709.89460 $ & $   0.01169 $ & $   0.00098 $ & $  11.71230 $ & $ i$\\
$ 55709.89616 $ & $   0.01028 $ & $   0.00097 $ & $  11.71000 $ & $ i$\\
$ 55709.89771 $ & $   0.00576 $ & $   0.00098 $ & $  11.70680 $ & $ i$\\
$ 55709.89925 $ & $   0.00376 $ & $   0.00097 $ & $  11.70450 $ & $ i$\\
$ 55709.90083 $ & $   0.00436 $ & $   0.00098 $ & $  11.70480 $ & $ i$\\
$ 55709.90245 $ & $   0.00105 $ & $   0.00098 $ & $  11.70240 $ & $ i$\\
$ 55709.90401 $ & $   0.00061 $ & $   0.00097 $ & $  11.70120 $ & $ i$\\
$ 55709.90555 $ & $   0.00109 $ & $   0.00097 $ & $  11.70250 $ & $ i$\\
$ 55709.90710 $ & $  -0.00095 $ & $   0.00097 $ & $  11.69910 $ & $ i$\\
$ 55709.90865 $ & $  -0.00303 $ & $   0.00098 $ & $  11.69760 $ & $ i$\\
$ 55709.91022 $ & $   0.00029 $ & $   0.00098 $ & $  11.70160 $ & $ i$\\
$ 55709.91176 $ & $   0.00199 $ & $   0.00098 $ & $  11.70300 $ & $ i$\\
$ 55709.91331 $ & $  -0.00175 $ & $   0.00098 $ & $  11.69890 $ & $ i$\\
$ 55709.91484 $ & $  -0.00126 $ & $   0.00098 $ & $  11.69960 $ & $ i$\\
$ 55709.91640 $ & $  -0.00265 $ & $   0.00099 $ & $  11.69730 $ & $ i$\\
$ 55709.91795 $ & $   0.00401 $ & $   0.00098 $ & $  11.70460 $ & $ i$\\
$ 55709.91950 $ & $  -0.00095 $ & $   0.00098 $ & $  11.70010 $ & $ i$\\
$ 55709.92105 $ & $  -0.00355 $ & $   0.00098 $ & $  11.69720 $ & $ i$\\
$ 55709.92261 $ & $   0.00434 $ & $   0.00099 $ & $  11.70450 $ & $ i$\\
$ 55709.92418 $ & $  -0.00153 $ & $   0.00098 $ & $  11.69970 $ & $ i$\\
$ 55709.92574 $ & $  -0.00265 $ & $   0.00099 $ & $  11.69800 $ & $ i$\\
$ 55709.92729 $ & $  -0.00005 $ & $   0.00099 $ & $  11.70040 $ & $ i$\\
$ 55709.92884 $ & $   0.00225 $ & $   0.00099 $ & $  11.70390 $ & $ i$\\


==> data/HTR146-002_phfu_tab_short.tex <==
$ 55640.84396 $ & $  -0.00143 $ & $   0.00122 $ & $  12.01460 $ & $ i$\\
$ 55640.84597 $ & $   0.00034 $ & $   0.00119 $ & $  12.01570 $ & $ i$\\
$ 55640.84767 $ & $  -0.00081 $ & $   0.00119 $ & $  12.01670 $ & $ i$\\
$ 55640.84922 $ & $   0.00007 $ & $   0.00122 $ & $  12.01650 $ & $ i$\\
$ 55640.85109 $ & $  -0.00137 $ & $   0.00119 $ & $  12.01450 $ & $ i$\\
$ 55640.85271 $ & $   0.00200 $ & $   0.00122 $ & $  12.01870 $ & $ i$\\
$ 55640.85427 $ & $  -0.00050 $ & $   0.00121 $ & $  12.01580 $ & $ i$\\
$ 55640.85593 $ & $  -0.00410 $ & $   0.00122 $ & $  12.01310 $ & $ i$\\
$ 55640.85747 $ & $  -0.00288 $ & $   0.00122 $ & $  12.01370 $ & $ i$\\
$ 55640.85902 $ & $  -0.00104 $ & $   0.00119 $ & $  12.01550 $ & $ i$\\


==> data/HTR146-002_rvtable.tex <==
$ 1606.11852 $ & $   103.86 $ & $     4.35 $ & $     4.86 $ & $     6.27 $ & $    0.1310 $ & $   0.885 $\\
$ 1612.12701 $ & $    -5.37 $ & $     3.65 $ & $    -6.08 $ & $     4.51 $ & $    0.1220 $ & $   0.282 $\\
$ 1612.14300 $ & \nodata      & \nodata      & $    19.68 $ & $     8.23 $ & $    0.1340 $ & $   0.286 $\\
$ 1613.03742 $ & $    67.53 $ & $    12.22 $ & \nodata      & \nodata      & $    0.2320 $ & $   0.494 $\\
$ 1614.11905 $ & $    99.23 $ & $     4.03 $ & $    -0.94 $ & $     5.65 $ & $    0.1060 $ & $   0.745 $\\
$ 1634.02686 $ & $     4.99 $ & $     3.88 $ & $     0.70 $ & $     5.06 $ & $    0.1460 $ & $   0.374 $\\
$ 1663.99061 $ & $   -13.54 $ & $     3.76 $ & $    -1.47 $ & $     8.11 $ & $    0.1270 $ & $   0.340 $\\
$ 1671.88450 $ & $   -25.58 $ & $     4.06 $ & $    -6.52 $ & $     5.82 $ & $    0.1150 $ & $   0.176 $\\
$ 1672.95630 $ & $     2.88 $ & $     4.01 $ & $    -8.64 $ & $     6.49 $ & $    0.1340 $ & $   0.425 $\\
$ 1673.87329 $ & $    57.51 $ & $     3.84 $ & $    13.66 $ & $     6.67 $ & $    0.1230 $ & $   0.638 $\\
$ 1696.81647 $ & $     7.20 $ & $     4.38 $ & $    28.16 $ & $    19.64 $ & $    0.0878 $ & $   0.972 $\\
$ 1697.81428 $ & $   -47.86 $ & $     3.61 $ & $    16.33 $ & $    16.80 $ & $    0.1130 $ & $   0.204 $\\
$ 1698.88909 $ & \nodata      & \nodata      & \nodata      & \nodata      & $    0.2110 $ & $   0.454 $\\
$ 1699.79550 $ & $    17.57 $ & $     3.65 $ & $    23.87 $ & $    12.27 $ & $    0.1410 $ & $   0.665 $\\
$ 1700.84720 $ & $    -1.91 $ & $     3.34 $ & $     4.25 $ & $     4.48 $ & $    0.1180 $ & $   0.909 $\\
$ 1703.83608 $ & $   -14.10 $ & $     3.34 $ & $     6.33 $ & $     6.88 $ & $    0.1230 $ & $   0.604 $\\
$ 1704.77501 $ & $    11.45 $ & $     3.83 $ & $   -12.18 $ & $    10.70 $ & $    0.1230 $ & $   0.822 $\\
$ 1705.79848 $ & $   -57.55 $ & $     3.40 $ & $    -1.17 $ & $     5.64 $ & $    0.0890 $ & $   0.060 $\\
$ 1707.82993 $ & $   -27.03 $ & $     3.90 $ & $     0.26 $ & $     5.30 $ & $    0.1370 $ & $   0.533 $\\
$ 1723.83103 $ & $  -105.67 $ & $     4.37 $ & $    -9.10 $ & $     4.26 $ & $    0.1330 $ & $   0.253 $\\
$ 1945.04563 $ & $   -11.27 $ & $     4.68 $ & \nodata      & \nodata      & \nodata      & $   0.683 $\\
$ 2019.98862 $ & $   -38.87 $ & $     4.18 $ & \nodata      & \nodata      & \nodata      & $   0.107 $\\
$ 2115.75933 $ & $   -27.58 $ & $     3.90 $ & \nodata      & \nodata      & \nodata      & $   0.373 $\\


==> data/HTR432-011_phfu_tab.tex <==
$ 55687.79447 $ & $  -0.00440 $ & $   0.00112 $ & $  10.45700 $ & $ i$\\
$ 55687.79497 $ & $   0.00288 $ & $   0.00113 $ & $  10.46460 $ & $ i$\\
$ 55687.79596 $ & $  -0.00087 $ & $   0.00113 $ & $  10.46190 $ & $ i$\\
$ 55687.79647 $ & $  -0.00065 $ & $   0.00113 $ & $  10.46210 $ & $ i$\\
$ 55687.79699 $ & $  -0.00327 $ & $   0.00112 $ & $  10.45850 $ & $ i$\\
$ 55687.79749 $ & $   0.00222 $ & $   0.00112 $ & $  10.46330 $ & $ i$\\
$ 55687.79798 $ & $   0.00089 $ & $   0.00113 $ & $  10.46300 $ & $ i$\\
$ 55687.79850 $ & $  -0.00339 $ & $   0.00112 $ & $  10.45840 $ & $ i$\\
$ 55687.79901 $ & $   0.00378 $ & $   0.00112 $ & $  10.46610 $ & $ i$\\
$ 55687.79952 $ & $   0.00308 $ & $   0.00113 $ & $  10.46470 $ & $ i$\\
$ 55687.80003 $ & $  -0.00217 $ & $   0.00113 $ & $  10.46010 $ & $ i$\\
$ 55687.80054 $ & $  -0.00289 $ & $   0.00112 $ & $  10.45820 $ & $ i$\\
$ 55687.80208 $ & $   0.00497 $ & $   0.00112 $ & $  10.46650 $ & $ i$\\
$ 55687.80258 $ & $  -0.00327 $ & $   0.00112 $ & $  10.45760 $ & $ i$\\
$ 55687.80309 $ & $   0.00292 $ & $   0.00112 $ & $  10.46480 $ & $ i$\\
$ 55687.80357 $ & $   0.00154 $ & $   0.00112 $ & $  10.46390 $ & $ i$\\
$ 55687.80408 $ & $  -0.00112 $ & $   0.00112 $ & $  10.46070 $ & $ i$\\
$ 55687.80460 $ & $   0.00358 $ & $   0.00112 $ & $  10.46530 $ & $ i$\\
$ 55687.80513 $ & $   0.00141 $ & $   0.00112 $ & $  10.46310 $ & $ i$\\
$ 55687.80564 $ & $   0.00023 $ & $   0.00112 $ & $  10.46270 $ & $ i$\\
$ 55687.80616 $ & $  -0.00283 $ & $   0.00112 $ & $  10.45960 $ & $ i$\\
$ 55687.80667 $ & $   0.00023 $ & $   0.00112 $ & $  10.46250 $ & $ i$\\
$ 55687.80716 $ & $   0.00279 $ & $   0.00112 $ & $  10.46400 $ & $ i$\\
$ 55687.80767 $ & $  -0.00195 $ & $   0.00111 $ & $  10.45930 $ & $ i$\\
$ 55687.80819 $ & $   0.00132 $ & $   0.00112 $ & $  10.46270 $ & $ i$\\
$ 55687.80871 $ & $  -0.00001 $ & $   0.00111 $ & $  10.46180 $ & $ i$\\
$ 55687.80921 $ & $   0.00175 $ & $   0.00112 $ & $  10.46300 $ & $ i$\\
$ 55687.80970 $ & $  -0.00355 $ & $   0.00111 $ & $  10.45910 $ & $ i$\\
$ 55687.81020 $ & $   0.00161 $ & $   0.00111 $ & $  10.46350 $ & $ i$\\
$ 55687.81070 $ & $   0.00267 $ & $   0.00111 $ & $  10.46350 $ & $ i$\\
$ 55687.81121 $ & $  -0.00177 $ & $   0.00110 $ & $  10.46090 $ & $ i$\\
$ 55687.81172 $ & $  -0.00047 $ & $   0.00111 $ & $  10.46160 $ & $ i$\\
$ 55687.81223 $ & $  -0.00197 $ & $   0.00111 $ & $  10.45940 $ & $ i$\\
$ 55687.81272 $ & $   0.00026 $ & $   0.00111 $ & $  10.46210 $ & $ i$\\
$ 55687.81322 $ & $   0.00010 $ & $   0.00111 $ & $  10.46110 $ & $ i$\\
$ 55687.81373 $ & $  -0.00064 $ & $   0.00111 $ & $  10.45940 $ & $ i$\\
$ 55687.81424 $ & $   0.00010 $ & $   0.00111 $ & $  10.46230 $ & $ i$\\
$ 55687.81475 $ & $  -0.00397 $ & $   0.00110 $ & $  10.45840 $ & $ i$\\
$ 55687.81526 $ & $  -0.00070 $ & $   0.00110 $ & $  10.46110 $ & $ i$\\
$ 55687.81577 $ & $  -0.00203 $ & $   0.00111 $ & $  10.45900 $ & $ i$\\
$ 55687.81625 $ & $   0.00075 $ & $   0.00110 $ & $  10.46220 $ & $ i$\\
$ 55687.81676 $ & $   0.00206 $ & $   0.00110 $ & $  10.46380 $ & $ i$\\
$ 55687.81728 $ & $  -0.00112 $ & $   0.00111 $ & $  10.46070 $ & $ i$\\
$ 55687.81778 $ & $   0.00247 $ & $   0.00111 $ & $  10.46470 $ & $ i$\\
$ 55687.81830 $ & $   0.00145 $ & $   0.00110 $ & $  10.46320 $ & $ i$\\
$ 55687.81882 $ & $  -0.00008 $ & $   0.00111 $ & $  10.46070 $ & $ i$\\
$ 55687.81935 $ & $  -0.00018 $ & $   0.00110 $ & $  10.46090 $ & $ i$\\
$ 55687.81985 $ & $   0.00332 $ & $   0.00111 $ & $  10.46540 $ & $ i$\\
$ 55687.82038 $ & $  -0.00167 $ & $   0.00110 $ & $  10.45940 $ & $ i$\\
$ 55687.82090 $ & $   0.00093 $ & $   0.00110 $ & $  10.46310 $ & $ i$\\
$ 55687.82141 $ & $  -0.00184 $ & $   0.00110 $ & $  10.46050 $ & $ i$\\
$ 55687.82191 $ & $   0.00103 $ & $   0.00110 $ & $  10.46350 $ & $ i$\\
$ 55687.82244 $ & $  -0.00157 $ & $   0.00110 $ & $  10.46020 $ & $ i$\\
$ 55687.82293 $ & $   0.00037 $ & $   0.00110 $ & $  10.46170 $ & $ i$\\
$ 55687.82340 $ & $  -0.00140 $ & $   0.00110 $ & $  10.45980 $ & $ i$\\
$ 55687.82389 $ & $   0.00178 $ & $   0.00110 $ & $  10.46280 $ & $ i$\\
$ 55687.82440 $ & $   0.00099 $ & $   0.00110 $ & $  10.46300 $ & $ i$\\
$ 55687.82490 $ & $   0.00026 $ & $   0.00110 $ & $  10.46230 $ & $ i$\\
$ 55687.82540 $ & $  -0.00297 $ & $   0.00109 $ & $  10.45800 $ & $ i$\\
$ 55687.82591 $ & $   0.00079 $ & $   0.00109 $ & $  10.46200 $ & $ i$\\
$ 55687.82644 $ & $  -0.00049 $ & $   0.00109 $ & $  10.46140 $ & $ i$\\
$ 55687.82695 $ & $   0.00291 $ & $   0.00109 $ & $  10.46450 $ & $ i$\\
$ 55687.82747 $ & $   0.00334 $ & $   0.00109 $ & $  10.46560 $ & $ i$\\
$ 55687.82796 $ & $  -0.00189 $ & $   0.00108 $ & $  10.45920 $ & $ i$\\
$ 55687.82847 $ & $  -0.00322 $ & $   0.00109 $ & $  10.45770 $ & $ i$\\
$ 55687.82900 $ & $   0.00148 $ & $   0.00110 $ & $  10.46220 $ & $ i$\\
$ 55687.82951 $ & $  -0.00206 $ & $   0.00110 $ & $  10.45910 $ & $ i$\\
$ 55687.83003 $ & $  -0.00292 $ & $   0.00109 $ & $  10.45920 $ & $ i$\\
$ 55687.83054 $ & $  -0.00121 $ & $   0.00109 $ & $  10.46050 $ & $ i$\\
$ 55687.83105 $ & $  -0.00281 $ & $   0.00109 $ & $  10.45900 $ & $ i$\\
$ 55687.83154 $ & $   0.00047 $ & $   0.00109 $ & $  10.46090 $ & $ i$\\
$ 55687.83204 $ & $  -0.00311 $ & $   0.00108 $ & $  10.45890 $ & $ i$\\
$ 55687.83255 $ & $   0.00194 $ & $   0.00109 $ & $  10.46400 $ & $ i$\\
$ 55687.83307 $ & $  -0.00026 $ & $   0.00108 $ & $  10.46120 $ & $ i$\\
$ 55687.83359 $ & $   0.00286 $ & $   0.00109 $ & $  10.46510 $ & $ i$\\
$ 55687.83411 $ & $  -0.00166 $ & $   0.00109 $ & $  10.46000 $ & $ i$\\
$ 55687.83462 $ & $   0.00226 $ & $   0.00108 $ & $  10.46410 $ & $ i$\\
$ 55687.83513 $ & $  -0.00109 $ & $   0.00108 $ & $  10.46090 $ & $ i$\\
$ 55687.83565 $ & $   0.00158 $ & $   0.00108 $ & $  10.46280 $ & $ i$\\
$ 55687.83615 $ & $  -0.00347 $ & $   0.00108 $ & $  10.45750 $ & $ i$\\
$ 55687.83666 $ & $  -0.00251 $ & $   0.00108 $ & $  10.45880 $ & $ i$\\
$ 55687.83715 $ & $  -0.00073 $ & $   0.00109 $ & $  10.46130 $ & $ i$\\
$ 55687.83766 $ & $   0.00285 $ & $   0.00109 $ & $  10.46500 $ & $ i$\\
$ 55687.83814 $ & $  -0.00181 $ & $   0.00108 $ & $  10.46030 $ & $ i$\\
$ 55687.83863 $ & $  -0.00248 $ & $   0.00108 $ & $  10.45880 $ & $ i$\\
$ 55687.83913 $ & $   0.00310 $ & $   0.00108 $ & $  10.46450 $ & $ i$\\
$ 55687.83962 $ & $  -0.00232 $ & $   0.00108 $ & $  10.45980 $ & $ i$\\
$ 55687.84012 $ & $   0.00070 $ & $   0.00107 $ & $  10.46270 $ & $ i$\\
$ 55687.84063 $ & $  -0.00169 $ & $   0.00108 $ & $  10.46050 $ & $ i$\\
$ 55687.84123 $ & $  -0.00117 $ & $   0.00107 $ & $  10.45990 $ & $ i$\\
$ 55687.84182 $ & $   0.00078 $ & $   0.00108 $ & $  10.46300 $ & $ i$\\
$ 55687.84231 $ & $  -0.00045 $ & $   0.00108 $ & $  10.46050 $ & $ i$\\
$ 55687.84283 $ & $   0.00516 $ & $   0.00107 $ & $  10.46630 $ & $ i$\\
$ 55687.84335 $ & $  -0.00126 $ & $   0.00107 $ & $  10.46070 $ & $ i$\\
$ 55687.84386 $ & $  -0.00146 $ & $   0.00107 $ & $  10.45920 $ & $ i$\\
$ 55687.84436 $ & $   0.00160 $ & $   0.00107 $ & $  10.46300 $ & $ i$\\
$ 55687.84488 $ & $  -0.00229 $ & $   0.00107 $ & $  10.45850 $ & $ i$\\
$ 55687.84538 $ & $   0.00397 $ & $   0.00107 $ & $  10.46600 $ & $ i$\\
$ 55687.84590 $ & $  -0.00322 $ & $   0.00107 $ & $  10.45810 $ & $ i$\\
$ 55687.84641 $ & $  -0.00100 $ & $   0.00107 $ & $  10.46020 $ & $ i$\\
$ 55687.84693 $ & $  -0.00010 $ & $   0.00107 $ & $  10.46170 $ & $ i$\\
$ 55687.84745 $ & $  -0.00139 $ & $   0.00107 $ & $  10.45980 $ & $ i$\\
$ 55687.84796 $ & $   0.00053 $ & $   0.00107 $ & $  10.46170 $ & $ i$\\
$ 55687.84844 $ & $  -0.00103 $ & $   0.00106 $ & $  10.46070 $ & $ i$\\
$ 55687.84894 $ & $   0.00268 $ & $   0.00107 $ & $  10.46380 $ & $ i$\\
$ 55687.84945 $ & $  -0.00139 $ & $   0.00106 $ & $  10.45990 $ & $ i$\\
$ 55687.84994 $ & $  -0.00030 $ & $   0.00106 $ & $  10.46120 $ & $ i$\\
$ 55687.85043 $ & $  -0.00063 $ & $   0.00106 $ & $  10.46000 $ & $ i$\\
$ 55687.85096 $ & $  -0.00158 $ & $   0.00106 $ & $  10.45930 $ & $ i$\\
$ 55687.85148 $ & $  -0.00062 $ & $   0.00106 $ & $  10.46050 $ & $ i$\\
$ 55687.85200 $ & $  -0.00040 $ & $   0.00106 $ & $  10.46060 $ & $ i$\\
$ 55687.85251 $ & $  -0.00223 $ & $   0.00106 $ & $  10.45840 $ & $ i$\\
$ 55687.85300 $ & $   0.00301 $ & $   0.00106 $ & $  10.46420 $ & $ i$\\
$ 55687.85351 $ & $  -0.00123 $ & $   0.00107 $ & $  10.46150 $ & $ i$\\
$ 55687.85401 $ & $  -0.00099 $ & $   0.00106 $ & $  10.45970 $ & $ i$\\
$ 55687.85451 $ & $  -0.00208 $ & $   0.00106 $ & $  10.45900 $ & $ i$\\
$ 55687.85502 $ & $   0.00072 $ & $   0.00106 $ & $  10.46190 $ & $ i$\\
$ 55687.85552 $ & $   0.00088 $ & $   0.00107 $ & $  10.46260 $ & $ i$\\
$ 55687.85601 $ & $   0.00137 $ & $   0.00107 $ & $  10.46350 $ & $ i$\\
$ 55687.85650 $ & $   0.00346 $ & $   0.00107 $ & $  10.46410 $ & $ i$\\
$ 55687.85701 $ & $  -0.00010 $ & $   0.00107 $ & $  10.46140 $ & $ i$\\
$ 55687.85753 $ & $  -0.00159 $ & $   0.00107 $ & $  10.46000 $ & $ i$\\
$ 55687.85803 $ & $   0.00069 $ & $   0.00107 $ & $  10.46170 $ & $ i$\\
$ 55687.85854 $ & $  -0.00138 $ & $   0.00106 $ & $  10.45970 $ & $ i$\\
$ 55687.85902 $ & $  -0.00108 $ & $   0.00106 $ & $  10.46020 $ & $ i$\\
$ 55687.85950 $ & $   0.00132 $ & $   0.00106 $ & $  10.46260 $ & $ i$\\
$ 55687.86002 $ & $   0.00250 $ & $   0.00106 $ & $  10.46350 $ & $ i$\\
$ 55687.86054 $ & $   0.00032 $ & $   0.00106 $ & $  10.46100 $ & $ i$\\
$ 55687.86105 $ & $  -0.00100 $ & $   0.00106 $ & $  10.46040 $ & $ i$\\
$ 55687.86155 $ & $   0.00473 $ & $   0.00107 $ & $  10.46540 $ & $ i$\\
$ 55687.86204 $ & $   0.00007 $ & $   0.00107 $ & $  10.46180 $ & $ i$\\
$ 55687.86254 $ & $   0.00016 $ & $   0.00107 $ & $  10.46120 $ & $ i$\\
$ 55687.86306 $ & $  -0.00253 $ & $   0.00106 $ & $  10.45810 $ & $ i$\\
$ 55687.86358 $ & $  -0.00137 $ & $   0.00106 $ & $  10.45940 $ & $ i$\\
$ 55687.86408 $ & $   0.00235 $ & $   0.00106 $ & $  10.46340 $ & $ i$\\
$ 55687.86459 $ & $   0.00246 $ & $   0.00106 $ & $  10.46340 $ & $ i$\\
$ 55687.86517 $ & $   0.00267 $ & $   0.00106 $ & $  10.46370 $ & $ i$\\
$ 55687.86578 $ & $   0.00016 $ & $   0.00106 $ & $  10.46200 $ & $ i$\\
$ 55687.86639 $ & $   0.00130 $ & $   0.00106 $ & $  10.46300 $ & $ i$\\
$ 55687.86694 $ & $   0.00092 $ & $   0.00106 $ & $  10.46270 $ & $ i$\\
$ 55687.86745 $ & $   0.00322 $ & $   0.00106 $ & $  10.46360 $ & $ i$\\
$ 55687.86795 $ & $  -0.00007 $ & $   0.00106 $ & $  10.46140 $ & $ i$\\
$ 55687.86845 $ & $  -0.00023 $ & $   0.00106 $ & $  10.46040 $ & $ i$\\
$ 55687.86893 $ & $   0.00134 $ & $   0.00106 $ & $  10.46200 $ & $ i$\\
$ 55687.86943 $ & $   0.00078 $ & $   0.00106 $ & $  10.46140 $ & $ i$\\
$ 55687.86994 $ & $  -0.00199 $ & $   0.00105 $ & $  10.45870 $ & $ i$\\
$ 55687.87046 $ & $  -0.00235 $ & $   0.00106 $ & $  10.45880 $ & $ i$\\
$ 55687.87097 $ & $   0.00108 $ & $   0.00106 $ & $  10.46150 $ & $ i$\\
$ 55687.87149 $ & $   0.00013 $ & $   0.00106 $ & $  10.46140 $ & $ i$\\
$ 55687.87200 $ & $  -0.00274 $ & $   0.00106 $ & $  10.45870 $ & $ i$\\
$ 55687.87251 $ & $   0.00070 $ & $   0.00106 $ & $  10.46190 $ & $ i$\\
$ 55687.87301 $ & $   0.00199 $ & $   0.00106 $ & $  10.46300 $ & $ i$\\
$ 55687.87351 $ & $   0.00325 $ & $   0.00105 $ & $  10.46370 $ & $ i$\\
$ 55687.87401 $ & $  -0.00207 $ & $   0.00105 $ & $  10.45840 $ & $ i$\\
$ 55687.87452 $ & $  -0.00018 $ & $   0.00105 $ & $  10.46020 $ & $ i$\\
$ 55687.87504 $ & $   0.00280 $ & $   0.00106 $ & $  10.46340 $ & $ i$\\
$ 55687.87554 $ & $  -0.00026 $ & $   0.00105 $ & $  10.46050 $ & $ i$\\
$ 55687.87607 $ & $  -0.00137 $ & $   0.00105 $ & $  10.45960 $ & $ i$\\
$ 55687.87666 $ & $   0.00072 $ & $   0.00105 $ & $  10.46140 $ & $ i$\\
$ 55687.87725 $ & $  -0.00109 $ & $   0.00105 $ & $  10.45920 $ & $ i$\\
$ 55687.87783 $ & $  -0.00169 $ & $   0.00105 $ & $  10.45980 $ & $ i$\\
$ 55687.87842 $ & $   0.00157 $ & $   0.00106 $ & $  10.46190 $ & $ i$\\
$ 55687.87902 $ & $   0.00037 $ & $   0.00106 $ & $  10.46120 $ & $ i$\\
$ 55687.87962 $ & $   0.00250 $ & $   0.00105 $ & $  10.46340 $ & $ i$\\
$ 55687.88022 $ & $  -0.00237 $ & $   0.00105 $ & $  10.45830 $ & $ i$\\
$ 55687.88078 $ & $   0.00079 $ & $   0.00105 $ & $  10.46140 $ & $ i$\\
$ 55687.88133 $ & $   0.00221 $ & $   0.00106 $ & $  10.46300 $ & $ i$\\
$ 55687.88185 $ & $   0.00077 $ & $   0.00105 $ & $  10.46100 $ & $ i$\\
$ 55687.88239 $ & $  -0.00173 $ & $   0.00105 $ & $  10.45940 $ & $ i$\\
$ 55687.88289 $ & $   0.00003 $ & $   0.00105 $ & $  10.46000 $ & $ i$\\
$ 55687.88339 $ & $   0.00070 $ & $   0.00105 $ & $  10.46180 $ & $ i$\\
$ 55687.88389 $ & $  -0.00028 $ & $   0.00105 $ & $  10.46050 $ & $ i$\\
$ 55687.88438 $ & $   0.00028 $ & $   0.00106 $ & $  10.46160 $ & $ i$\\
$ 55687.88488 $ & $  -0.00198 $ & $   0.00105 $ & $  10.45890 $ & $ i$\\
$ 55687.88540 $ & $   0.00191 $ & $   0.00105 $ & $  10.46290 $ & $ i$\\
$ 55687.88591 $ & $  -0.00003 $ & $   0.00105 $ & $  10.46060 $ & $ i$\\
$ 55687.88642 $ & $   0.00100 $ & $   0.00105 $ & $  10.46090 $ & $ i$\\
$ 55687.88694 $ & $  -0.00017 $ & $   0.00105 $ & $  10.46010 $ & $ i$\\
$ 55687.88745 $ & $   0.00400 $ & $   0.00105 $ & $  10.46490 $ & $ i$\\
$ 55687.88795 $ & $   0.00218 $ & $   0.00105 $ & $  10.46330 $ & $ i$\\
$ 55687.88842 $ & $   0.00099 $ & $   0.00105 $ & $  10.46180 $ & $ i$\\
$ 55687.88893 $ & $   0.00064 $ & $   0.00106 $ & $  10.46180 $ & $ i$\\
$ 55687.88944 $ & $   0.00426 $ & $   0.00106 $ & $  10.46490 $ & $ i$\\
$ 55687.88996 $ & $   0.00348 $ & $   0.00105 $ & $  10.46350 $ & $ i$\\
$ 55687.89045 $ & $   0.00267 $ & $   0.00105 $ & $  10.46320 $ & $ i$\\
$ 55687.89097 $ & $   0.00577 $ & $   0.00106 $ & $  10.46720 $ & $ i$\\
$ 55687.89149 $ & $   0.00424 $ & $   0.00105 $ & $  10.46560 $ & $ i$\\
$ 55687.89200 $ & $   0.00560 $ & $   0.00105 $ & $  10.46640 $ & $ i$\\
$ 55687.89251 $ & $   0.00281 $ & $   0.00105 $ & $  10.46320 $ & $ i$\\
$ 55687.89303 $ & $   0.00592 $ & $   0.00105 $ & $  10.46620 $ & $ i$\\
$ 55687.89356 $ & $   0.00613 $ & $   0.00105 $ & $  10.46620 $ & $ i$\\
$ 55687.89406 $ & $   0.00539 $ & $   0.00105 $ & $  10.46550 $ & $ i$\\
$ 55687.89456 $ & $   0.00753 $ & $   0.00106 $ & $  10.46870 $ & $ i$\\
$ 55687.89508 $ & $   0.00671 $ & $   0.00106 $ & $  10.46780 $ & $ i$\\
$ 55687.89557 $ & $   0.00532 $ & $   0.00106 $ & $  10.46600 $ & $ i$\\
$ 55687.89605 $ & $   0.00773 $ & $   0.00106 $ & $  10.46870 $ & $ i$\\
$ 55687.89658 $ & $   0.00637 $ & $   0.00105 $ & $  10.46670 $ & $ i$\\
$ 55687.89709 $ & $   0.00593 $ & $   0.00105 $ & $  10.46720 $ & $ i$\\
$ 55687.89759 $ & $   0.00874 $ & $   0.00106 $ & $  10.46910 $ & $ i$\\
$ 55687.89810 $ & $   0.00888 $ & $   0.00106 $ & $  10.46940 $ & $ i$\\
$ 55687.89861 $ & $   0.00820 $ & $   0.00106 $ & $  10.46870 $ & $ i$\\
$ 55687.89912 $ & $   0.00802 $ & $   0.00106 $ & $  10.46880 $ & $ i$\\
$ 55687.89963 $ & $   0.00846 $ & $   0.00106 $ & $  10.46850 $ & $ i$\\
$ 55687.90014 $ & $   0.00857 $ & $   0.00106 $ & $  10.46970 $ & $ i$\\
$ 55687.90066 $ & $   0.00654 $ & $   0.00106 $ & $  10.46740 $ & $ i$\\
$ 55687.90118 $ & $   0.00612 $ & $   0.00105 $ & $  10.46690 $ & $ i$\\
$ 55687.90168 $ & $   0.01180 $ & $   0.00106 $ & $  10.47190 $ & $ i$\\
$ 55687.90219 $ & $   0.00851 $ & $   0.00106 $ & $  10.46880 $ & $ i$\\
$ 55687.90269 $ & $   0.00997 $ & $   0.00106 $ & $  10.47070 $ & $ i$\\
$ 55687.90320 $ & $   0.00977 $ & $   0.00106 $ & $  10.47070 $ & $ i$\\
$ 55687.90371 $ & $   0.01004 $ & $   0.00106 $ & $  10.47050 $ & $ i$\\
$ 55687.90422 $ & $   0.00944 $ & $   0.00106 $ & $  10.46990 $ & $ i$\\
$ 55687.90472 $ & $   0.01079 $ & $   0.00105 $ & $  10.47110 $ & $ i$\\
$ 55687.90521 $ & $   0.01177 $ & $   0.00106 $ & $  10.47210 $ & $ i$\\
$ 55687.90573 $ & $   0.00945 $ & $   0.00106 $ & $  10.46980 $ & $ i$\\
$ 55687.90625 $ & $   0.00716 $ & $   0.00106 $ & $  10.46750 $ & $ i$\\
$ 55687.90677 $ & $   0.00854 $ & $   0.00106 $ & $  10.46960 $ & $ i$\\
$ 55687.90729 $ & $   0.01037 $ & $   0.00106 $ & $  10.47100 $ & $ i$\\
$ 55687.90781 $ & $   0.00847 $ & $   0.00106 $ & $  10.46980 $ & $ i$\\
$ 55687.90830 $ & $   0.00980 $ & $   0.00106 $ & $  10.47040 $ & $ i$\\
$ 55687.90881 $ & $   0.01050 $ & $   0.00106 $ & $  10.47110 $ & $ i$\\
$ 55687.90934 $ & $   0.00990 $ & $   0.00105 $ & $  10.47030 $ & $ i$\\
$ 55687.90985 $ & $   0.01011 $ & $   0.00105 $ & $  10.47040 $ & $ i$\\
$ 55687.91036 $ & $   0.01248 $ & $   0.00106 $ & $  10.47280 $ & $ i$\\
$ 55687.91087 $ & $   0.00988 $ & $   0.00106 $ & $  10.47010 $ & $ i$\\
$ 55687.91136 $ & $   0.01042 $ & $   0.00105 $ & $  10.47030 $ & $ i$\\
$ 55687.91187 $ & $   0.01029 $ & $   0.00106 $ & $  10.47040 $ & $ i$\\
$ 55687.91238 $ & $   0.00910 $ & $   0.00106 $ & $  10.46880 $ & $ i$\\
$ 55687.91288 $ & $   0.01051 $ & $   0.00106 $ & $  10.47060 $ & $ i$\\
$ 55687.91339 $ & $   0.00806 $ & $   0.00105 $ & $  10.46770 $ & $ i$\\
$ 55687.91389 $ & $   0.01212 $ & $   0.00106 $ & $  10.47210 $ & $ i$\\
$ 55687.91440 $ & $   0.00871 $ & $   0.00106 $ & $  10.46940 $ & $ i$\\
$ 55687.91489 $ & $   0.01003 $ & $   0.00105 $ & $  10.47120 $ & $ i$\\
$ 55687.91540 $ & $   0.01119 $ & $   0.00106 $ & $  10.47150 $ & $ i$\\
$ 55687.91593 $ & $   0.00686 $ & $   0.00105 $ & $  10.46760 $ & $ i$\\
$ 55687.91646 $ & $   0.01032 $ & $   0.00106 $ & $  10.47010 $ & $ i$\\
$ 55687.91707 $ & $   0.01141 $ & $   0.00106 $ & $  10.47160 $ & $ i$\\
$ 55687.91767 $ & $   0.00886 $ & $   0.00105 $ & $  10.46910 $ & $ i$\\
$ 55687.91825 $ & $   0.00999 $ & $   0.00106 $ & $  10.47090 $ & $ i$\\
$ 55687.91875 $ & $   0.00984 $ & $   0.00106 $ & $  10.46940 $ & $ i$\\
$ 55687.91927 $ & $   0.01163 $ & $   0.00106 $ & $  10.47200 $ & $ i$\\
$ 55687.91978 $ & $   0.01226 $ & $   0.00106 $ & $  10.47250 $ & $ i$\\
$ 55687.92029 $ & $   0.01088 $ & $   0.00105 $ & $  10.47180 $ & $ i$\\
$ 55687.92081 $ & $   0.00777 $ & $   0.00105 $ & $  10.46810 $ & $ i$\\
$ 55687.92133 $ & $   0.01116 $ & $   0.00105 $ & $  10.47020 $ & $ i$\\
$ 55687.92184 $ & $   0.00874 $ & $   0.00105 $ & $  10.46840 $ & $ i$\\
$ 55687.92237 $ & $   0.01116 $ & $   0.00106 $ & $  10.47050 $ & $ i$\\
$ 55687.92287 $ & $   0.01184 $ & $   0.00105 $ & $  10.47240 $ & $ i$\\
$ 55687.92339 $ & $   0.00925 $ & $   0.00105 $ & $  10.46920 $ & $ i$\\
$ 55687.92391 $ & $   0.00964 $ & $   0.00106 $ & $  10.46990 $ & $ i$\\
$ 55687.92441 $ & $   0.00993 $ & $   0.00106 $ & $  10.47040 $ & $ i$\\
$ 55687.92492 $ & $   0.01068 $ & $   0.00106 $ & $  10.47140 $ & $ i$\\
$ 55687.92543 $ & $   0.01214 $ & $   0.00106 $ & $  10.47240 $ & $ i$\\
$ 55687.92603 $ & $   0.00803 $ & $   0.00105 $ & $  10.46850 $ & $ i$\\
$ 55687.92662 $ & $   0.01059 $ & $   0.00106 $ & $  10.47080 $ & $ i$\\
$ 55687.92720 $ & $   0.01117 $ & $   0.00105 $ & $  10.47160 $ & $ i$\\
$ 55687.92779 $ & $   0.00909 $ & $   0.00105 $ & $  10.46850 $ & $ i$\\
$ 55687.92838 $ & $   0.00772 $ & $   0.00105 $ & $  10.46850 $ & $ i$\\
$ 55687.92890 $ & $   0.00808 $ & $   0.00105 $ & $  10.46790 $ & $ i$\\
$ 55687.92939 $ & $   0.01162 $ & $   0.00106 $ & $  10.47210 $ & $ i$\\
$ 55687.92988 $ & $   0.00743 $ & $   0.00105 $ & $  10.46730 $ & $ i$\\
$ 55687.93045 $ & $   0.00910 $ & $   0.00105 $ & $  10.46820 $ & $ i$\\
$ 55687.93097 $ & $   0.00981 $ & $   0.00105 $ & $  10.46960 $ & $ i$\\
$ 55687.93149 $ & $   0.00939 $ & $   0.00106 $ & $  10.46970 $ & $ i$\\
$ 55687.93200 $ & $   0.01004 $ & $   0.00106 $ & $  10.47020 $ & $ i$\\
$ 55687.93251 $ & $   0.00784 $ & $   0.00105 $ & $  10.46800 $ & $ i$\\
$ 55687.93302 $ & $   0.00942 $ & $   0.00105 $ & $  10.47020 $ & $ i$\\
$ 55687.93352 $ & $   0.00989 $ & $   0.00105 $ & $  10.47040 $ & $ i$\\
$ 55687.93402 $ & $   0.01033 $ & $   0.00106 $ & $  10.47070 $ & $ i$\\
$ 55687.93451 $ & $   0.00777 $ & $   0.00106 $ & $  10.46820 $ & $ i$\\
$ 55687.93502 $ & $   0.00846 $ & $   0.00105 $ & $  10.46860 $ & $ i$\\
$ 55687.93554 $ & $   0.00945 $ & $   0.00105 $ & $  10.46930 $ & $ i$\\
$ 55687.93604 $ & $   0.01335 $ & $   0.00105 $ & $  10.47370 $ & $ i$\\
$ 55687.93654 $ & $   0.01036 $ & $   0.00105 $ & $  10.47030 $ & $ i$\\
$ 55687.93705 $ & $   0.00866 $ & $   0.00106 $ & $  10.46860 $ & $ i$\\
$ 55687.93753 $ & $   0.00996 $ & $   0.00105 $ & $  10.47020 $ & $ i$\\
$ 55687.93806 $ & $   0.01198 $ & $   0.00106 $ & $  10.47210 $ & $ i$\\
$ 55687.93855 $ & $   0.01100 $ & $   0.00105 $ & $  10.47120 $ & $ i$\\
$ 55687.93908 $ & $   0.00648 $ & $   0.00106 $ & $  10.46640 $ & $ i$\\
$ 55687.93958 $ & $   0.01051 $ & $   0.00105 $ & $  10.47010 $ & $ i$\\
$ 55687.94008 $ & $   0.01247 $ & $   0.00106 $ & $  10.47300 $ & $ i$\\
$ 55687.94057 $ & $   0.00681 $ & $   0.00105 $ & $  10.46660 $ & $ i$\\
$ 55687.94108 $ & $   0.01051 $ & $   0.00106 $ & $  10.46980 $ & $ i$\\
$ 55687.94159 $ & $   0.00866 $ & $   0.00105 $ & $  10.46910 $ & $ i$\\
$ 55687.94212 $ & $   0.01016 $ & $   0.00105 $ & $  10.47060 $ & $ i$\\
$ 55687.94263 $ & $   0.01052 $ & $   0.00106 $ & $  10.47100 $ & $ i$\\
$ 55687.94313 $ & $   0.00855 $ & $   0.00106 $ & $  10.46920 $ & $ i$\\
$ 55687.94364 $ & $   0.01038 $ & $   0.00105 $ & $  10.47080 $ & $ i$\\
$ 55687.94413 $ & $   0.00902 $ & $   0.00105 $ & $  10.46930 $ & $ i$\\
$ 55687.94464 $ & $   0.01114 $ & $   0.00105 $ & $  10.47140 $ & $ i$\\
$ 55687.94516 $ & $   0.01087 $ & $   0.00105 $ & $  10.47080 $ & $ i$\\
$ 55687.94568 $ & $   0.00911 $ & $   0.00105 $ & $  10.46900 $ & $ i$\\
$ 55687.94620 $ & $   0.01090 $ & $   0.00105 $ & $  10.47100 $ & $ i$\\
$ 55687.94673 $ & $   0.00988 $ & $   0.00105 $ & $  10.47010 $ & $ i$\\
$ 55687.94725 $ & $   0.00911 $ & $   0.00106 $ & $  10.47010 $ & $ i$\\
$ 55687.94776 $ & $   0.01143 $ & $   0.00106 $ & $  10.47220 $ & $ i$\\
$ 55687.94828 $ & $   0.00862 $ & $   0.00105 $ & $  10.46850 $ & $ i$\\
$ 55687.94879 $ & $   0.01120 $ & $   0.00105 $ & $  10.47100 $ & $ i$\\
$ 55687.94927 $ & $   0.00897 $ & $   0.00105 $ & $  10.46870 $ & $ i$\\
$ 55687.94979 $ & $   0.00952 $ & $   0.00105 $ & $  10.46920 $ & $ i$\\
$ 55687.95030 $ & $   0.00964 $ & $   0.00105 $ & $  10.46860 $ & $ i$\\
$ 55687.95082 $ & $   0.00878 $ & $   0.00105 $ & $  10.46870 $ & $ i$\\
$ 55687.95132 $ & $   0.00974 $ & $   0.00105 $ & $  10.46940 $ & $ i$\\
$ 55687.95184 $ & $   0.01277 $ & $   0.00105 $ & $  10.47310 $ & $ i$\\
$ 55687.95235 $ & $   0.01205 $ & $   0.00106 $ & $  10.47200 $ & $ i$\\
$ 55687.95286 $ & $   0.00726 $ & $   0.00106 $ & $  10.46760 $ & $ i$\\
$ 55687.95335 $ & $   0.00958 $ & $   0.00105 $ & $  10.46930 $ & $ i$\\
$ 55687.95387 $ & $   0.01136 $ & $   0.00105 $ & $  10.47180 $ & $ i$\\
$ 55687.95438 $ & $   0.01219 $ & $   0.00105 $ & $  10.47200 $ & $ i$\\
$ 55687.95489 $ & $   0.00900 $ & $   0.00106 $ & $  10.46960 $ & $ i$\\
$ 55687.95541 $ & $   0.00964 $ & $   0.00106 $ & $  10.47060 $ & $ i$\\
$ 55687.95589 $ & $   0.00971 $ & $   0.00105 $ & $  10.46980 $ & $ i$\\
$ 55687.95639 $ & $   0.00778 $ & $   0.00105 $ & $  10.46890 $ & $ i$\\
$ 55687.95689 $ & $   0.01267 $ & $   0.00105 $ & $  10.47290 $ & $ i$\\
$ 55687.95739 $ & $   0.01063 $ & $   0.00105 $ & $  10.47030 $ & $ i$\\
$ 55687.95790 $ & $   0.00734 $ & $   0.00106 $ & $  10.46720 $ & $ i$\\
$ 55687.95840 $ & $   0.00963 $ & $   0.00105 $ & $  10.46980 $ & $ i$\\
$ 55687.95891 $ & $   0.00931 $ & $   0.00105 $ & $  10.46880 $ & $ i$\\
$ 55687.95944 $ & $   0.00866 $ & $   0.00105 $ & $  10.46920 $ & $ i$\\
$ 55687.95993 $ & $   0.01154 $ & $   0.00105 $ & $  10.47160 $ & $ i$\\
$ 55687.96043 $ & $   0.01076 $ & $   0.00105 $ & $  10.47090 $ & $ i$\\
$ 55687.96095 $ & $   0.00857 $ & $   0.00105 $ & $  10.46890 $ & $ i$\\
$ 55687.96146 $ & $   0.00891 $ & $   0.00105 $ & $  10.46950 $ & $ i$\\
$ 55687.96196 $ & $   0.01032 $ & $   0.00105 $ & $  10.47000 $ & $ i$\\
$ 55687.96246 $ & $   0.01064 $ & $   0.00105 $ & $  10.47050 $ & $ i$\\
$ 55687.96295 $ & $   0.01009 $ & $   0.00106 $ & $  10.47090 $ & $ i$\\
$ 55687.96346 $ & $   0.01035 $ & $   0.00106 $ & $  10.47060 $ & $ i$\\
$ 55687.96397 $ & $   0.01087 $ & $   0.00105 $ & $  10.47080 $ & $ i$\\
$ 55687.96448 $ & $   0.01051 $ & $   0.00105 $ & $  10.47060 $ & $ i$\\
$ 55687.96498 $ & $   0.01286 $ & $   0.00106 $ & $  10.47280 $ & $ i$\\
$ 55687.96548 $ & $   0.01038 $ & $   0.00106 $ & $  10.47080 $ & $ i$\\
$ 55687.96597 $ & $   0.01007 $ & $   0.00105 $ & $  10.46990 $ & $ i$\\
$ 55687.96648 $ & $   0.00943 $ & $   0.00106 $ & $  10.46930 $ & $ i$\\
$ 55687.96698 $ & $   0.01214 $ & $   0.00106 $ & $  10.47240 $ & $ i$\\
$ 55687.96747 $ & $   0.01158 $ & $   0.00105 $ & $  10.47160 $ & $ i$\\
$ 55687.96808 $ & $   0.00987 $ & $   0.00105 $ & $  10.46990 $ & $ i$\\
$ 55687.96871 $ & $   0.01011 $ & $   0.00105 $ & $  10.47000 $ & $ i$\\
$ 55687.96931 $ & $   0.01093 $ & $   0.00105 $ & $  10.47130 $ & $ i$\\
$ 55687.96983 $ & $   0.01192 $ & $   0.00105 $ & $  10.47310 $ & $ i$\\
$ 55687.97034 $ & $   0.00900 $ & $   0.00106 $ & $  10.46860 $ & $ i$\\
$ 55687.97085 $ & $   0.01101 $ & $   0.00106 $ & $  10.47170 $ & $ i$\\
$ 55687.97135 $ & $   0.01254 $ & $   0.00105 $ & $  10.47260 $ & $ i$\\
$ 55687.97185 $ & $   0.01310 $ & $   0.00105 $ & $  10.47270 $ & $ i$\\
$ 55687.97246 $ & $   0.01014 $ & $   0.00105 $ & $  10.47060 $ & $ i$\\
$ 55687.97305 $ & $   0.01037 $ & $   0.00105 $ & $  10.47080 $ & $ i$\\
$ 55687.97365 $ & $   0.01048 $ & $   0.00106 $ & $  10.47030 $ & $ i$\\
$ 55687.97424 $ & $   0.00767 $ & $   0.00105 $ & $  10.46760 $ & $ i$\\
$ 55687.97483 $ & $   0.01285 $ & $   0.00105 $ & $  10.47320 $ & $ i$\\
$ 55687.97535 $ & $   0.00880 $ & $   0.00105 $ & $  10.46910 $ & $ i$\\
$ 55687.97587 $ & $   0.01108 $ & $   0.00105 $ & $  10.47080 $ & $ i$\\
$ 55687.97639 $ & $   0.00887 $ & $   0.00105 $ & $  10.46880 $ & $ i$\\
$ 55687.97692 $ & $   0.00875 $ & $   0.00105 $ & $  10.46870 $ & $ i$\\
$ 55687.97741 $ & $   0.00905 $ & $   0.00106 $ & $  10.46850 $ & $ i$\\
$ 55687.97791 $ & $   0.01069 $ & $   0.00106 $ & $  10.47100 $ & $ i$\\
$ 55687.97841 $ & $   0.00690 $ & $   0.00106 $ & $  10.46710 $ & $ i$\\
$ 55687.97890 $ & $   0.00848 $ & $   0.00106 $ & $  10.46840 $ & $ i$\\
$ 55687.97941 $ & $   0.00847 $ & $   0.00105 $ & $  10.46910 $ & $ i$\\
$ 55687.97993 $ & $   0.01100 $ & $   0.00105 $ & $  10.47110 $ & $ i$\\
$ 55687.98043 $ & $   0.00799 $ & $   0.00105 $ & $  10.46740 $ & $ i$\\
$ 55687.98093 $ & $   0.01041 $ & $   0.00105 $ & $  10.46980 $ & $ i$\\
$ 55687.98143 $ & $   0.00903 $ & $   0.00106 $ & $  10.46890 $ & $ i$\\
$ 55687.98194 $ & $   0.01211 $ & $   0.00106 $ & $  10.47210 $ & $ i$\\
$ 55687.98246 $ & $   0.01136 $ & $   0.00106 $ & $  10.47130 $ & $ i$\\
$ 55687.98299 $ & $   0.01099 $ & $   0.00106 $ & $  10.47090 $ & $ i$\\
$ 55687.98350 $ & $   0.00999 $ & $   0.00106 $ & $  10.46910 $ & $ i$\\
$ 55687.98400 $ & $   0.01008 $ & $   0.00106 $ & $  10.47010 $ & $ i$\\
$ 55687.98449 $ & $   0.01127 $ & $   0.00106 $ & $  10.47060 $ & $ i$\\
$ 55687.98500 $ & $   0.00968 $ & $   0.00106 $ & $  10.46950 $ & $ i$\\
$ 55687.98550 $ & $   0.00880 $ & $   0.00107 $ & $  10.46830 $ & $ i$\\
$ 55687.98601 $ & $   0.01146 $ & $   0.00107 $ & $  10.47080 $ & $ i$\\
$ 55687.98651 $ & $   0.01029 $ & $   0.00107 $ & $  10.46970 $ & $ i$\\
$ 55687.98702 $ & $   0.01054 $ & $   0.00107 $ & $  10.47030 $ & $ i$\\
$ 55687.98754 $ & $   0.01190 $ & $   0.00109 $ & $  10.47100 $ & $ i$\\
$ 55687.98805 $ & $   0.01098 $ & $   0.00108 $ & $  10.47080 $ & $ i$\\
$ 55687.98856 $ & $   0.00873 $ & $   0.00108 $ & $  10.46760 $ & $ i$\\
$ 55687.98907 $ & $   0.00864 $ & $   0.00108 $ & $  10.46820 $ & $ i$\\
$ 55687.98960 $ & $   0.00871 $ & $   0.00108 $ & $  10.46860 $ & $ i$\\
$ 55687.99010 $ & $   0.00995 $ & $   0.00110 $ & $  10.47000 $ & $ i$\\
$ 55687.99062 $ & $   0.00656 $ & $   0.00110 $ & $  10.46650 $ & $ i$\\
$ 55687.99110 $ & $   0.00860 $ & $   0.00110 $ & $  10.46850 $ & $ i$\\
$ 55687.99161 $ & $   0.00472 $ & $   0.00111 $ & $  10.46360 $ & $ i$\\
$ 55687.99212 $ & $   0.00919 $ & $   0.00112 $ & $  10.46930 $ & $ i$\\
$ 55687.99263 $ & $   0.00661 $ & $   0.00113 $ & $  10.46690 $ & $ i$\\
$ 55687.99313 $ & $   0.00839 $ & $   0.00114 $ & $  10.46930 $ & $ i$\\
$ 55687.99363 $ & $   0.00699 $ & $   0.00116 $ & $  10.46610 $ & $ i$\\
$ 55687.99414 $ & $   0.00691 $ & $   0.00117 $ & $  10.46650 $ & $ i$\\
$ 55687.99465 $ & $   0.00892 $ & $   0.00120 $ & $  10.46890 $ & $ i$\\
$ 55687.99514 $ & $   0.01160 $ & $   0.00122 $ & $  10.47100 $ & $ i$\\
$ 55696.77263 $ & $  -0.00165 $ & $   0.00105 $ & $  10.46500 $ & $ i$\\
$ 55696.77317 $ & $  -0.00393 $ & $   0.00106 $ & $  10.46280 $ & $ i$\\
$ 55696.77379 $ & $   0.00068 $ & $   0.00106 $ & $  10.46760 $ & $ i$\\
$ 55696.77442 $ & $  -0.00238 $ & $   0.00105 $ & $  10.46390 $ & $ i$\\
$ 55696.77507 $ & $   0.00306 $ & $   0.00105 $ & $  10.47030 $ & $ i$\\
$ 55696.77566 $ & $  -0.00041 $ & $   0.00106 $ & $  10.46560 $ & $ i$\\
$ 55696.77623 $ & $   0.00258 $ & $   0.00105 $ & $  10.46950 $ & $ i$\\
$ 55696.77678 $ & $  -0.00268 $ & $   0.00106 $ & $  10.46370 $ & $ i$\\
$ 55696.77735 $ & $   0.00292 $ & $   0.00105 $ & $  10.46990 $ & $ i$\\
$ 55696.77792 $ & $  -0.00163 $ & $   0.00105 $ & $  10.46470 $ & $ i$\\
$ 55696.77848 $ & $  -0.00054 $ & $   0.00105 $ & $  10.46520 $ & $ i$\\
$ 55696.77905 $ & $  -0.00080 $ & $   0.00105 $ & $  10.46550 $ & $ i$\\
$ 55696.77961 $ & $   0.00348 $ & $   0.00106 $ & $  10.47000 $ & $ i$\\
$ 55696.78017 $ & $   0.00168 $ & $   0.00105 $ & $  10.46870 $ & $ i$\\
$ 55696.78075 $ & $   0.00081 $ & $   0.00105 $ & $  10.46610 $ & $ i$\\
$ 55696.78131 $ & $   0.00130 $ & $   0.00105 $ & $  10.46730 $ & $ i$\\
$ 55696.78188 $ & $  -0.00021 $ & $   0.00105 $ & $  10.46510 $ & $ i$\\
$ 55696.78243 $ & $   0.00193 $ & $   0.00105 $ & $  10.46860 $ & $ i$\\
$ 55696.78301 $ & $  -0.00175 $ & $   0.00105 $ & $  10.46390 $ & $ i$\\
$ 55696.78357 $ & $  -0.00081 $ & $   0.00104 $ & $  10.46520 $ & $ i$\\
$ 55696.78414 $ & $   0.00359 $ & $   0.00105 $ & $  10.46980 $ & $ i$\\
$ 55696.78471 $ & $  -0.00026 $ & $   0.00105 $ & $  10.46560 $ & $ i$\\
$ 55696.78528 $ & $   0.00148 $ & $   0.00104 $ & $  10.46680 $ & $ i$\\
$ 55696.78586 $ & $   0.00273 $ & $   0.00104 $ & $  10.46880 $ & $ i$\\
$ 55696.78644 $ & $  -0.00156 $ & $   0.00104 $ & $  10.46350 $ & $ i$\\
$ 55696.78699 $ & $  -0.00001 $ & $   0.00103 $ & $  10.46490 $ & $ i$\\
$ 55696.78756 $ & $  -0.00057 $ & $   0.00103 $ & $  10.46520 $ & $ i$\\
$ 55696.78809 $ & $  -0.00006 $ & $   0.00103 $ & $  10.46570 $ & $ i$\\
$ 55696.78864 $ & $   0.00060 $ & $   0.00104 $ & $  10.46660 $ & $ i$\\
$ 55696.78920 $ & $  -0.00159 $ & $   0.00104 $ & $  10.46300 $ & $ i$\\
$ 55696.78977 $ & $   0.00097 $ & $   0.00104 $ & $  10.46650 $ & $ i$\\
$ 55696.79033 $ & $  -0.00101 $ & $   0.00103 $ & $  10.46450 $ & $ i$\\
$ 55696.79090 $ & $   0.00369 $ & $   0.00104 $ & $  10.46920 $ & $ i$\\
$ 55696.79147 $ & $  -0.00171 $ & $   0.00103 $ & $  10.46430 $ & $ i$\\
$ 55696.79203 $ & $  -0.00259 $ & $   0.00103 $ & $  10.46250 $ & $ i$\\
$ 55696.79259 $ & $  -0.00000 $ & $   0.00103 $ & $  10.46460 $ & $ i$\\
$ 55696.79316 $ & $  -0.00496 $ & $   0.00102 $ & $  10.46060 $ & $ i$\\
$ 55696.79373 $ & $   0.00174 $ & $   0.00103 $ & $  10.46640 $ & $ i$\\
$ 55696.79428 $ & $   0.00060 $ & $   0.00103 $ & $  10.46600 $ & $ i$\\
$ 55696.79484 $ & $  -0.00471 $ & $   0.00103 $ & $  10.46110 $ & $ i$\\
$ 55696.79542 $ & $   0.00240 $ & $   0.00103 $ & $  10.46760 $ & $ i$\\
$ 55696.79597 $ & $  -0.00348 $ & $   0.00103 $ & $  10.46200 $ & $ i$\\
$ 55696.79653 $ & $   0.00009 $ & $   0.00103 $ & $  10.46530 $ & $ i$\\
$ 55696.79710 $ & $   0.00040 $ & $   0.00103 $ & $  10.46500 $ & $ i$\\
$ 55696.79766 $ & $  -0.00081 $ & $   0.00103 $ & $  10.46400 $ & $ i$\\
$ 55696.79823 $ & $  -0.00105 $ & $   0.00103 $ & $  10.46400 $ & $ i$\\
$ 55696.79882 $ & $  -0.00296 $ & $   0.00103 $ & $  10.46230 $ & $ i$\\
$ 55696.79937 $ & $  -0.00186 $ & $   0.00103 $ & $  10.46260 $ & $ i$\\
$ 55696.79994 $ & $   0.00093 $ & $   0.00103 $ & $  10.46590 $ & $ i$\\
$ 55696.80051 $ & $  -0.00199 $ & $   0.00102 $ & $  10.46260 $ & $ i$\\
$ 55696.80108 $ & $   0.00076 $ & $   0.00102 $ & $  10.46580 $ & $ i$\\
$ 55696.80163 $ & $   0.00413 $ & $   0.00103 $ & $  10.46870 $ & $ i$\\
$ 55696.80221 $ & $  -0.00208 $ & $   0.00102 $ & $  10.46240 $ & $ i$\\
$ 55696.80277 $ & $  -0.00330 $ & $   0.00102 $ & $  10.46200 $ & $ i$\\
$ 55696.80330 $ & $   0.00319 $ & $   0.00102 $ & $  10.46770 $ & $ i$\\
$ 55696.80388 $ & $   0.00140 $ & $   0.00103 $ & $  10.46710 $ & $ i$\\
$ 55696.80445 $ & $  -0.00005 $ & $   0.00102 $ & $  10.46420 $ & $ i$\\
$ 55696.80501 $ & $  -0.00056 $ & $   0.00102 $ & $  10.46450 $ & $ i$\\
$ 55696.80559 $ & $  -0.00030 $ & $   0.00102 $ & $  10.46450 $ & $ i$\\
$ 55696.80617 $ & $  -0.00181 $ & $   0.00102 $ & $  10.46280 $ & $ i$\\
$ 55696.80674 $ & $   0.00165 $ & $   0.00103 $ & $  10.46620 $ & $ i$\\
$ 55696.80729 $ & $  -0.00060 $ & $   0.00102 $ & $  10.46390 $ & $ i$\\
$ 55696.80785 $ & $   0.00144 $ & $   0.00102 $ & $  10.46620 $ & $ i$\\
$ 55696.80841 $ & $  -0.00087 $ & $   0.00102 $ & $  10.46420 $ & $ i$\\
$ 55696.80898 $ & $   0.00167 $ & $   0.00102 $ & $  10.46670 $ & $ i$\\
$ 55696.80956 $ & $   0.00060 $ & $   0.00103 $ & $  10.46580 $ & $ i$\\
$ 55696.81012 $ & $   0.00372 $ & $   0.00102 $ & $  10.46860 $ & $ i$\\
$ 55696.81070 $ & $   0.00329 $ & $   0.00102 $ & $  10.46880 $ & $ i$\\
$ 55696.81128 $ & $  -0.00072 $ & $   0.00102 $ & $  10.46440 $ & $ i$\\
$ 55696.81183 $ & $  -0.00126 $ & $   0.00101 $ & $  10.46330 $ & $ i$\\
$ 55696.81241 $ & $   0.00146 $ & $   0.00102 $ & $  10.46630 $ & $ i$\\
$ 55696.81297 $ & $   0.00276 $ & $   0.00102 $ & $  10.46760 $ & $ i$\\
$ 55696.81353 $ & $   0.00317 $ & $   0.00102 $ & $  10.46720 $ & $ i$\\
$ 55696.81410 $ & $   0.00368 $ & $   0.00101 $ & $  10.46880 $ & $ i$\\
$ 55696.81473 $ & $   0.00059 $ & $   0.00102 $ & $  10.46530 $ & $ i$\\
$ 55696.81541 $ & $   0.00462 $ & $   0.00102 $ & $  10.46940 $ & $ i$\\
$ 55696.81603 $ & $   0.00179 $ & $   0.00102 $ & $  10.46640 $ & $ i$\\
$ 55696.81669 $ & $   0.00482 $ & $   0.00102 $ & $  10.46960 $ & $ i$\\
$ 55696.81733 $ & $   0.00422 $ & $   0.00102 $ & $  10.46870 $ & $ i$\\
$ 55696.81798 $ & $   0.00172 $ & $   0.00101 $ & $  10.46640 $ & $ i$\\
$ 55696.81917 $ & $   0.00172 $ & $   0.00102 $ & $  10.46650 $ & $ i$\\
$ 55696.81974 $ & $   0.00492 $ & $   0.00101 $ & $  10.46950 $ & $ i$\\
$ 55696.82030 $ & $   0.00347 $ & $   0.00102 $ & $  10.46810 $ & $ i$\\
$ 55696.82086 $ & $   0.00721 $ & $   0.00102 $ & $  10.47180 $ & $ i$\\
$ 55696.82142 $ & $   0.00759 $ & $   0.00101 $ & $  10.47180 $ & $ i$\\
$ 55696.82198 $ & $   0.00470 $ & $   0.00101 $ & $  10.46970 $ & $ i$\\
$ 55696.82256 $ & $   0.00532 $ & $   0.00101 $ & $  10.46950 $ & $ i$\\
$ 55696.82312 $ & $   0.00612 $ & $   0.00101 $ & $  10.47090 $ & $ i$\\
$ 55696.82367 $ & $   0.00513 $ & $   0.00101 $ & $  10.47110 $ & $ i$\\
$ 55696.82425 $ & $   0.00833 $ & $   0.00101 $ & $  10.47260 $ & $ i$\\
$ 55696.82481 $ & $   0.00797 $ & $   0.00101 $ & $  10.47290 $ & $ i$\\
$ 55696.82537 $ & $   0.00831 $ & $   0.00101 $ & $  10.47240 $ & $ i$\\
$ 55696.82595 $ & $   0.00503 $ & $   0.00101 $ & $  10.46930 $ & $ i$\\
$ 55696.82652 $ & $   0.00875 $ & $   0.00102 $ & $  10.47370 $ & $ i$\\
$ 55696.82709 $ & $   0.00952 $ & $   0.00101 $ & $  10.47390 $ & $ i$\\
$ 55696.82767 $ & $   0.01058 $ & $   0.00101 $ & $  10.47610 $ & $ i$\\
$ 55696.82822 $ & $   0.01077 $ & $   0.00102 $ & $  10.47470 $ & $ i$\\
$ 55696.82879 $ & $   0.00691 $ & $   0.00101 $ & $  10.47200 $ & $ i$\\
$ 55696.82938 $ & $   0.00786 $ & $   0.00101 $ & $  10.47170 $ & $ i$\\
$ 55696.82996 $ & $   0.00927 $ & $   0.00101 $ & $  10.47390 $ & $ i$\\
$ 55696.83051 $ & $   0.00893 $ & $   0.00101 $ & $  10.47330 $ & $ i$\\
$ 55696.83108 $ & $   0.01144 $ & $   0.00101 $ & $  10.47590 $ & $ i$\\
$ 55696.83165 $ & $   0.00808 $ & $   0.00101 $ & $  10.47260 $ & $ i$\\
$ 55696.83223 $ & $   0.00917 $ & $   0.00101 $ & $  10.47330 $ & $ i$\\
$ 55696.83276 $ & $   0.01123 $ & $   0.00101 $ & $  10.47560 $ & $ i$\\
$ 55696.83333 $ & $   0.01121 $ & $   0.00101 $ & $  10.47570 $ & $ i$\\
$ 55696.83388 $ & $   0.00875 $ & $   0.00101 $ & $  10.47360 $ & $ i$\\
$ 55696.83444 $ & $   0.00916 $ & $   0.00101 $ & $  10.47370 $ & $ i$\\
$ 55696.83500 $ & $   0.00840 $ & $   0.00100 $ & $  10.47350 $ & $ i$\\
$ 55696.83557 $ & $   0.00978 $ & $   0.00101 $ & $  10.47360 $ & $ i$\\
$ 55696.83612 $ & $   0.00893 $ & $   0.00101 $ & $  10.47400 $ & $ i$\\
$ 55696.83669 $ & $   0.01421 $ & $   0.00101 $ & $  10.47920 $ & $ i$\\
$ 55696.83726 $ & $   0.01047 $ & $   0.00101 $ & $  10.47550 $ & $ i$\\
$ 55696.83783 $ & $   0.00624 $ & $   0.00101 $ & $  10.47110 $ & $ i$\\
$ 55696.83838 $ & $   0.00909 $ & $   0.00101 $ & $  10.47280 $ & $ i$\\
$ 55696.83894 $ & $   0.00688 $ & $   0.00101 $ & $  10.47170 $ & $ i$\\
$ 55696.83951 $ & $   0.00948 $ & $   0.00101 $ & $  10.47360 $ & $ i$\\
$ 55696.84006 $ & $   0.00719 $ & $   0.00101 $ & $  10.47160 $ & $ i$\\
$ 55696.84063 $ & $   0.01085 $ & $   0.00101 $ & $  10.47520 $ & $ i$\\
$ 55696.84116 $ & $   0.01218 $ & $   0.00100 $ & $  10.47590 $ & $ i$\\
$ 55696.84173 $ & $   0.01300 $ & $   0.00101 $ & $  10.47740 $ & $ i$\\
$ 55696.84230 $ & $   0.00974 $ & $   0.00101 $ & $  10.47370 $ & $ i$\\
$ 55696.84286 $ & $   0.01160 $ & $   0.00101 $ & $  10.47530 $ & $ i$\\
$ 55696.84343 $ & $   0.01092 $ & $   0.00101 $ & $  10.47520 $ & $ i$\\
$ 55696.84400 $ & $   0.01220 $ & $   0.00101 $ & $  10.47730 $ & $ i$\\
$ 55696.84457 $ & $   0.00891 $ & $   0.00100 $ & $  10.47320 $ & $ i$\\
$ 55696.84513 $ & $   0.00953 $ & $   0.00101 $ & $  10.47390 $ & $ i$\\
$ 55696.84570 $ & $   0.01003 $ & $   0.00100 $ & $  10.47510 $ & $ i$\\
$ 55696.84628 $ & $   0.01140 $ & $   0.00100 $ & $  10.47520 $ & $ i$\\
$ 55696.84683 $ & $   0.00907 $ & $   0.00100 $ & $  10.47290 $ & $ i$\\
$ 55696.84742 $ & $   0.00820 $ & $   0.00100 $ & $  10.47210 $ & $ i$\\
$ 55696.84799 $ & $   0.01070 $ & $   0.00100 $ & $  10.47530 $ & $ i$\\
$ 55696.84856 $ & $   0.01085 $ & $   0.00101 $ & $  10.47560 $ & $ i$\\
$ 55696.84913 $ & $   0.00915 $ & $   0.00100 $ & $  10.47360 $ & $ i$\\
$ 55696.84968 $ & $   0.01029 $ & $   0.00100 $ & $  10.47400 $ & $ i$\\
$ 55696.85024 $ & $   0.01107 $ & $   0.00101 $ & $  10.47540 $ & $ i$\\
$ 55696.85079 $ & $   0.00947 $ & $   0.00101 $ & $  10.47430 $ & $ i$\\
$ 55696.85137 $ & $   0.00855 $ & $   0.00100 $ & $  10.47280 $ & $ i$\\
$ 55696.85194 $ & $   0.00986 $ & $   0.00101 $ & $  10.47470 $ & $ i$\\
$ 55696.85249 $ & $   0.01085 $ & $   0.00101 $ & $  10.47490 $ & $ i$\\
$ 55696.85304 $ & $   0.00895 $ & $   0.00100 $ & $  10.47270 $ & $ i$\\
$ 55696.85362 $ & $   0.01123 $ & $   0.00101 $ & $  10.47540 $ & $ i$\\
$ 55696.85419 $ & $   0.00888 $ & $   0.00100 $ & $  10.47280 $ & $ i$\\
$ 55696.85477 $ & $   0.01161 $ & $   0.00100 $ & $  10.47490 $ & $ i$\\
$ 55696.85533 $ & $   0.00858 $ & $   0.00100 $ & $  10.47280 $ & $ i$\\
$ 55696.85590 $ & $   0.01183 $ & $   0.00101 $ & $  10.47570 $ & $ i$\\
$ 55696.85646 $ & $   0.01024 $ & $   0.00100 $ & $  10.47370 $ & $ i$\\
$ 55696.85704 $ & $   0.01219 $ & $   0.00100 $ & $  10.47570 $ & $ i$\\
$ 55696.85761 $ & $   0.01038 $ & $   0.00100 $ & $  10.47410 $ & $ i$\\
$ 55696.85819 $ & $   0.01135 $ & $   0.00100 $ & $  10.47520 $ & $ i$\\
$ 55696.85876 $ & $   0.01118 $ & $   0.00099 $ & $  10.47480 $ & $ i$\\
$ 55696.85932 $ & $   0.00811 $ & $   0.00100 $ & $  10.47190 $ & $ i$\\
$ 55696.85989 $ & $   0.01137 $ & $   0.00100 $ & $  10.47550 $ & $ i$\\
$ 55696.86046 $ & $   0.00940 $ & $   0.00100 $ & $  10.47340 $ & $ i$\\
$ 55696.86102 $ & $   0.01209 $ & $   0.00100 $ & $  10.47580 $ & $ i$\\
$ 55696.86160 $ & $   0.01032 $ & $   0.00100 $ & $  10.47440 $ & $ i$\\
$ 55696.86218 $ & $   0.01108 $ & $   0.00100 $ & $  10.47590 $ & $ i$\\
$ 55696.86275 $ & $   0.00801 $ & $   0.00100 $ & $  10.47160 $ & $ i$\\
$ 55696.86332 $ & $   0.01090 $ & $   0.00100 $ & $  10.47520 $ & $ i$\\
$ 55696.86388 $ & $   0.01341 $ & $   0.00100 $ & $  10.47780 $ & $ i$\\
$ 55696.86446 $ & $   0.01141 $ & $   0.00100 $ & $  10.47470 $ & $ i$\\
$ 55696.86502 $ & $   0.00920 $ & $   0.00100 $ & $  10.47390 $ & $ i$\\
$ 55696.86561 $ & $   0.00961 $ & $   0.00100 $ & $  10.47380 $ & $ i$\\
$ 55696.86616 $ & $   0.01022 $ & $   0.00100 $ & $  10.47440 $ & $ i$\\
$ 55696.86675 $ & $   0.01043 $ & $   0.00100 $ & $  10.47400 $ & $ i$\\
$ 55696.86732 $ & $   0.01188 $ & $   0.00100 $ & $  10.47600 $ & $ i$\\
$ 55696.86788 $ & $   0.01119 $ & $   0.00100 $ & $  10.47550 $ & $ i$\\
$ 55696.86843 $ & $   0.00812 $ & $   0.00100 $ & $  10.47250 $ & $ i$\\
$ 55696.86901 $ & $   0.00964 $ & $   0.00100 $ & $  10.47300 $ & $ i$\\
$ 55696.86957 $ & $   0.01152 $ & $   0.00100 $ & $  10.47630 $ & $ i$\\
$ 55696.87016 $ & $   0.01200 $ & $   0.00100 $ & $  10.47620 $ & $ i$\\
$ 55696.87072 $ & $   0.00811 $ & $   0.00100 $ & $  10.47180 $ & $ i$\\
$ 55696.87128 $ & $   0.00975 $ & $   0.00100 $ & $  10.47360 $ & $ i$\\
$ 55696.87185 $ & $   0.01210 $ & $   0.00100 $ & $  10.47620 $ & $ i$\\
$ 55696.87243 $ & $   0.00999 $ & $   0.00100 $ & $  10.47380 $ & $ i$\\
$ 55696.87299 $ & $   0.00934 $ & $   0.00100 $ & $  10.47340 $ & $ i$\\
$ 55696.87356 $ & $   0.00927 $ & $   0.00100 $ & $  10.47320 $ & $ i$\\
$ 55696.87413 $ & $   0.01196 $ & $   0.00100 $ & $  10.47570 $ & $ i$\\
$ 55696.87469 $ & $   0.01227 $ & $   0.00100 $ & $  10.47630 $ & $ i$\\
$ 55696.87539 $ & $   0.01029 $ & $   0.00100 $ & $  10.47390 $ & $ i$\\
$ 55696.87607 $ & $   0.01071 $ & $   0.00100 $ & $  10.47520 $ & $ i$\\
$ 55696.87673 $ & $   0.01050 $ & $   0.00099 $ & $  10.47480 $ & $ i$\\
$ 55696.87730 $ & $   0.01025 $ & $   0.00099 $ & $  10.47360 $ & $ i$\\
$ 55696.87787 $ & $   0.01384 $ & $   0.00100 $ & $  10.47770 $ & $ i$\\
$ 55696.87843 $ & $   0.01014 $ & $   0.00100 $ & $  10.47420 $ & $ i$\\
$ 55696.87901 $ & $   0.01005 $ & $   0.00100 $ & $  10.47400 $ & $ i$\\
$ 55696.87966 $ & $   0.01074 $ & $   0.00100 $ & $  10.47470 $ & $ i$\\
$ 55696.88033 $ & $   0.01274 $ & $   0.00100 $ & $  10.47680 $ & $ i$\\
$ 55696.88100 $ & $   0.01209 $ & $   0.00100 $ & $  10.47670 $ & $ i$\\
$ 55696.88166 $ & $   0.01135 $ & $   0.00100 $ & $  10.47530 $ & $ i$\\
$ 55696.88228 $ & $   0.01003 $ & $   0.00100 $ & $  10.47490 $ & $ i$\\
$ 55696.88284 $ & $   0.01055 $ & $   0.00100 $ & $  10.47470 $ & $ i$\\
$ 55696.88341 $ & $   0.00776 $ & $   0.00099 $ & $  10.47210 $ & $ i$\\
$ 55696.88401 $ & $   0.01299 $ & $   0.00100 $ & $  10.47680 $ & $ i$\\
$ 55696.88457 $ & $   0.00988 $ & $   0.00100 $ & $  10.47410 $ & $ i$\\
$ 55696.88513 $ & $   0.01009 $ & $   0.00100 $ & $  10.47420 $ & $ i$\\
$ 55696.88571 $ & $   0.00997 $ & $   0.00100 $ & $  10.47380 $ & $ i$\\
$ 55696.88629 $ & $   0.01264 $ & $   0.00100 $ & $  10.47670 $ & $ i$\\
$ 55696.88686 $ & $   0.00994 $ & $   0.00100 $ & $  10.47350 $ & $ i$\\
$ 55696.88744 $ & $   0.01231 $ & $   0.00100 $ & $  10.47660 $ & $ i$\\
$ 55696.88797 $ & $   0.01077 $ & $   0.00099 $ & $  10.47540 $ & $ i$\\
$ 55696.88853 $ & $   0.00852 $ & $   0.00100 $ & $  10.47280 $ & $ i$\\
$ 55696.88909 $ & $   0.01024 $ & $   0.00099 $ & $  10.47460 $ & $ i$\\
$ 55696.88967 $ & $   0.01012 $ & $   0.00099 $ & $  10.47450 $ & $ i$\\
$ 55696.89023 $ & $   0.01023 $ & $   0.00099 $ & $  10.47440 $ & $ i$\\
$ 55696.89079 $ & $   0.01010 $ & $   0.00099 $ & $  10.47380 $ & $ i$\\
$ 55696.89137 $ & $   0.00691 $ & $   0.00099 $ & $  10.47100 $ & $ i$\\
$ 55696.89194 $ & $   0.00941 $ & $   0.00100 $ & $  10.47330 $ & $ i$\\
$ 55696.89250 $ & $   0.01175 $ & $   0.00099 $ & $  10.47590 $ & $ i$\\
$ 55696.89307 $ & $   0.00867 $ & $   0.00100 $ & $  10.47270 $ & $ i$\\
$ 55696.89364 $ & $   0.00956 $ & $   0.00099 $ & $  10.47300 $ & $ i$\\
$ 55696.89421 $ & $   0.01061 $ & $   0.00099 $ & $  10.47490 $ & $ i$\\
$ 55696.89478 $ & $   0.01085 $ & $   0.00099 $ & $  10.47530 $ & $ i$\\
$ 55696.89536 $ & $   0.00867 $ & $   0.00099 $ & $  10.47220 $ & $ i$\\
$ 55696.89593 $ & $   0.01234 $ & $   0.00099 $ & $  10.47650 $ & $ i$\\
$ 55696.89648 $ & $   0.01021 $ & $   0.00099 $ & $  10.47440 $ & $ i$\\
$ 55696.89705 $ & $   0.00912 $ & $   0.00099 $ & $  10.47330 $ & $ i$\\
$ 55696.89759 $ & $   0.00975 $ & $   0.00099 $ & $  10.47320 $ & $ i$\\
$ 55696.89816 $ & $   0.00839 $ & $   0.00099 $ & $  10.47250 $ & $ i$\\
$ 55696.89872 $ & $   0.01128 $ & $   0.00100 $ & $  10.47560 $ & $ i$\\
$ 55696.89928 $ & $   0.01016 $ & $   0.00099 $ & $  10.47450 $ & $ i$\\
$ 55696.89985 $ & $   0.00740 $ & $   0.00099 $ & $  10.47120 $ & $ i$\\
$ 55696.90040 $ & $   0.00870 $ & $   0.00099 $ & $  10.47360 $ & $ i$\\
$ 55696.90096 $ & $   0.01177 $ & $   0.00099 $ & $  10.47550 $ & $ i$\\
$ 55696.90152 $ & $   0.00931 $ & $   0.00099 $ & $  10.47400 $ & $ i$\\
$ 55696.90208 $ & $   0.00863 $ & $   0.00099 $ & $  10.47310 $ & $ i$\\
$ 55696.90262 $ & $   0.00971 $ & $   0.00099 $ & $  10.47400 $ & $ i$\\
$ 55696.90319 $ & $   0.00668 $ & $   0.00099 $ & $  10.47100 $ & $ i$\\
$ 55696.90376 $ & $   0.00946 $ & $   0.00099 $ & $  10.47440 $ & $ i$\\
$ 55696.90431 $ & $   0.01122 $ & $   0.00099 $ & $  10.47580 $ & $ i$\\
$ 55696.90489 $ & $   0.00927 $ & $   0.00099 $ & $  10.47340 $ & $ i$\\
$ 55696.90545 $ & $   0.01088 $ & $   0.00100 $ & $  10.47510 $ & $ i$\\
$ 55696.90603 $ & $   0.00847 $ & $   0.00100 $ & $  10.47270 $ & $ i$\\
$ 55696.90659 $ & $   0.01017 $ & $   0.00100 $ & $  10.47480 $ & $ i$\\
$ 55696.90716 $ & $   0.01228 $ & $   0.00099 $ & $  10.47660 $ & $ i$\\
$ 55696.90773 $ & $   0.00918 $ & $   0.00099 $ & $  10.47410 $ & $ i$\\
$ 55696.90830 $ & $   0.00938 $ & $   0.00099 $ & $  10.47370 $ & $ i$\\
$ 55696.90886 $ & $   0.00746 $ & $   0.00099 $ & $  10.47150 $ & $ i$\\
$ 55696.90942 $ & $   0.00714 $ & $   0.00099 $ & $  10.47160 $ & $ i$\\
$ 55696.90998 $ & $   0.00963 $ & $   0.00099 $ & $  10.47410 $ & $ i$\\
$ 55696.91054 $ & $   0.00957 $ & $   0.00099 $ & $  10.47400 $ & $ i$\\
$ 55696.91112 $ & $   0.01063 $ & $   0.00099 $ & $  10.47460 $ & $ i$\\
$ 55696.91169 $ & $   0.00995 $ & $   0.00099 $ & $  10.47400 $ & $ i$\\
$ 55696.91226 $ & $   0.00963 $ & $   0.00099 $ & $  10.47390 $ & $ i$\\
$ 55696.91283 $ & $   0.00748 $ & $   0.00099 $ & $  10.47150 $ & $ i$\\
$ 55696.91339 $ & $   0.01129 $ & $   0.00099 $ & $  10.47590 $ & $ i$\\
$ 55696.91396 $ & $   0.00655 $ & $   0.00099 $ & $  10.47070 $ & $ i$\\
$ 55696.91452 $ & $   0.01196 $ & $   0.00099 $ & $  10.47580 $ & $ i$\\
$ 55696.91509 $ & $   0.00697 $ & $   0.00099 $ & $  10.47130 $ & $ i$\\
$ 55696.91986 $ & $   0.01015 $ & $   0.00099 $ & $  10.47450 $ & $ i$\\
$ 55696.92043 $ & $   0.00975 $ & $   0.00099 $ & $  10.47380 $ & $ i$\\
$ 55696.92099 $ & $   0.00689 $ & $   0.00099 $ & $  10.47090 $ & $ i$\\
$ 55696.92157 $ & $   0.00576 $ & $   0.00099 $ & $  10.46960 $ & $ i$\\
$ 55696.92214 $ & $   0.00765 $ & $   0.00098 $ & $  10.47170 $ & $ i$\\
$ 55696.92271 $ & $   0.00684 $ & $   0.00099 $ & $  10.47090 $ & $ i$\\
$ 55696.92327 $ & $   0.00767 $ & $   0.00099 $ & $  10.47280 $ & $ i$\\
$ 55696.92384 $ & $   0.00822 $ & $   0.00099 $ & $  10.47290 $ & $ i$\\
$ 55696.92440 $ & $   0.00705 $ & $   0.00099 $ & $  10.47090 $ & $ i$\\
$ 55696.92495 $ & $   0.00605 $ & $   0.00098 $ & $  10.47060 $ & $ i$\\
$ 55696.92551 $ & $   0.00625 $ & $   0.00099 $ & $  10.46950 $ & $ i$\\
$ 55696.92610 $ & $   0.00489 $ & $   0.00099 $ & $  10.46970 $ & $ i$\\
$ 55696.92666 $ & $   0.00598 $ & $   0.00098 $ & $  10.47060 $ & $ i$\\
$ 55696.92722 $ & $   0.00552 $ & $   0.00099 $ & $  10.47000 $ & $ i$\\
$ 55696.92781 $ & $   0.00327 $ & $   0.00098 $ & $  10.46750 $ & $ i$\\
$ 55696.92837 $ & $   0.00528 $ & $   0.00098 $ & $  10.46940 $ & $ i$\\
$ 55696.92893 $ & $   0.00180 $ & $   0.00098 $ & $  10.46600 $ & $ i$\\
$ 55696.92951 $ & $   0.00122 $ & $   0.00098 $ & $  10.46570 $ & $ i$\\
$ 55696.93008 $ & $   0.00721 $ & $   0.00099 $ & $  10.47160 $ & $ i$\\
$ 55696.93062 $ & $  -0.00021 $ & $   0.00098 $ & $  10.46490 $ & $ i$\\
$ 55696.93118 $ & $   0.00319 $ & $   0.00099 $ & $  10.46770 $ & $ i$\\
$ 55696.93173 $ & $   0.00409 $ & $   0.00099 $ & $  10.46820 $ & $ i$\\
$ 55696.93231 $ & $   0.00438 $ & $   0.00099 $ & $  10.46840 $ & $ i$\\
$ 55696.93287 $ & $   0.00134 $ & $   0.00098 $ & $  10.46550 $ & $ i$\\
$ 55696.93344 $ & $  -0.00134 $ & $   0.00098 $ & $  10.46280 $ & $ i$\\
$ 55696.93399 $ & $   0.00095 $ & $   0.00098 $ & $  10.46520 $ & $ i$\\
$ 55696.93456 $ & $  -0.00123 $ & $   0.00098 $ & $  10.46350 $ & $ i$\\
$ 55696.93511 $ & $   0.00209 $ & $   0.00099 $ & $  10.46640 $ & $ i$\\
$ 55696.93568 $ & $  -0.00083 $ & $   0.00098 $ & $  10.46370 $ & $ i$\\
$ 55696.93632 $ & $   0.00014 $ & $   0.00098 $ & $  10.46520 $ & $ i$\\
$ 55696.93701 $ & $  -0.00080 $ & $   0.00098 $ & $  10.46380 $ & $ i$\\
$ 55696.93770 $ & $  -0.00066 $ & $   0.00098 $ & $  10.46380 $ & $ i$\\
$ 55696.93825 $ & $  -0.00127 $ & $   0.00098 $ & $  10.46280 $ & $ i$\\
$ 55696.93883 $ & $   0.00043 $ & $   0.00098 $ & $  10.46470 $ & $ i$\\
$ 55696.93939 $ & $  -0.00397 $ & $   0.00098 $ & $  10.46060 $ & $ i$\\
$ 55696.93998 $ & $  -0.00068 $ & $   0.00098 $ & $  10.46430 $ & $ i$\\
$ 55696.94054 $ & $  -0.00037 $ & $   0.00098 $ & $  10.46420 $ & $ i$\\
$ 55696.94119 $ & $   0.00018 $ & $   0.00098 $ & $  10.46450 $ & $ i$\\
$ 55696.94183 $ & $  -0.00034 $ & $   0.00097 $ & $  10.46420 $ & $ i$\\
$ 55696.94249 $ & $  -0.00185 $ & $   0.00097 $ & $  10.46190 $ & $ i$\\
$ 55696.94316 $ & $   0.00168 $ & $   0.00098 $ & $  10.46600 $ & $ i$\\
$ 55696.94378 $ & $  -0.00001 $ & $   0.00098 $ & $  10.46420 $ & $ i$\\
$ 55696.94434 $ & $  -0.00001 $ & $   0.00097 $ & $  10.46510 $ & $ i$\\
$ 55696.94491 $ & $   0.00306 $ & $   0.00097 $ & $  10.46750 $ & $ i$\\
$ 55696.94548 $ & $   0.00048 $ & $   0.00097 $ & $  10.46490 $ & $ i$\\
$ 55696.94606 $ & $   0.00060 $ & $   0.00098 $ & $  10.46570 $ & $ i$\\
$ 55696.94663 $ & $   0.00190 $ & $   0.00097 $ & $  10.46630 $ & $ i$\\
$ 55696.94719 $ & $   0.00141 $ & $   0.00098 $ & $  10.46660 $ & $ i$\\
$ 55696.94775 $ & $   0.00068 $ & $   0.00097 $ & $  10.46470 $ & $ i$\\
$ 55696.94832 $ & $  -0.00098 $ & $   0.00097 $ & $  10.46350 $ & $ i$\\
$ 55696.94890 $ & $   0.00168 $ & $   0.00097 $ & $  10.46600 $ & $ i$\\
$ 55696.94944 $ & $  -0.00100 $ & $   0.00097 $ & $  10.46310 $ & $ i$\\
$ 55696.95000 $ & $  -0.00055 $ & $   0.00097 $ & $  10.46390 $ & $ i$\\
$ 55696.95057 $ & $   0.00067 $ & $   0.00097 $ & $  10.46530 $ & $ i$\\
$ 55696.95113 $ & $   0.00010 $ & $   0.00097 $ & $  10.46460 $ & $ i$\\
$ 55696.95171 $ & $   0.00183 $ & $   0.00097 $ & $  10.46620 $ & $ i$\\
$ 55696.95224 $ & $  -0.00178 $ & $   0.00097 $ & $  10.46270 $ & $ i$\\
$ 55696.95280 $ & $  -0.00082 $ & $   0.00097 $ & $  10.46340 $ & $ i$\\
$ 55696.95337 $ & $   0.00083 $ & $   0.00097 $ & $  10.46540 $ & $ i$\\
$ 55696.95395 $ & $   0.00004 $ & $   0.00097 $ & $  10.46530 $ & $ i$\\
$ 55696.95451 $ & $   0.00123 $ & $   0.00097 $ & $  10.46630 $ & $ i$\\
$ 55696.95508 $ & $   0.00160 $ & $   0.00097 $ & $  10.46630 $ & $ i$\\
$ 55696.95562 $ & $   0.00074 $ & $   0.00097 $ & $  10.46560 $ & $ i$\\
$ 55696.95618 $ & $   0.00080 $ & $   0.00097 $ & $  10.46450 $ & $ i$\\
$ 55696.95676 $ & $  -0.00213 $ & $   0.00097 $ & $  10.46200 $ & $ i$\\
$ 55696.95733 $ & $   0.00092 $ & $   0.00097 $ & $  10.46570 $ & $ i$\\
$ 55696.95789 $ & $   0.00061 $ & $   0.00097 $ & $  10.46480 $ & $ i$\\
$ 55696.95844 $ & $   0.00124 $ & $   0.00097 $ & $  10.46580 $ & $ i$\\
$ 55696.95900 $ & $  -0.00007 $ & $   0.00096 $ & $  10.46480 $ & $ i$\\
$ 55696.95957 $ & $  -0.00184 $ & $   0.00096 $ & $  10.46340 $ & $ i$\\
$ 55696.96014 $ & $  -0.00374 $ & $   0.00097 $ & $  10.46100 $ & $ i$\\
$ 55696.96071 $ & $  -0.00245 $ & $   0.00097 $ & $  10.46240 $ & $ i$\\
$ 55696.96127 $ & $  -0.00063 $ & $   0.00097 $ & $  10.46390 $ & $ i$\\
$ 55696.96242 $ & $  -0.00151 $ & $   0.00097 $ & $  10.46340 $ & $ i$\\
$ 55696.96299 $ & $   0.00133 $ & $   0.00097 $ & $  10.46570 $ & $ i$\\
$ 55696.96354 $ & $  -0.00023 $ & $   0.00097 $ & $  10.46430 $ & $ i$\\
$ 55696.96411 $ & $   0.00087 $ & $   0.00097 $ & $  10.46600 $ & $ i$\\
$ 55696.96469 $ & $   0.00049 $ & $   0.00097 $ & $  10.46590 $ & $ i$\\
$ 55696.96522 $ & $   0.00047 $ & $   0.00097 $ & $  10.46520 $ & $ i$\\
$ 55696.96579 $ & $   0.00122 $ & $   0.00097 $ & $  10.46640 $ & $ i$\\
$ 55696.96635 $ & $   0.00009 $ & $   0.00097 $ & $  10.46420 $ & $ i$\\
$ 55696.96693 $ & $  -0.00094 $ & $   0.00097 $ & $  10.46400 $ & $ i$\\
$ 55696.96748 $ & $   0.00110 $ & $   0.00097 $ & $  10.46600 $ & $ i$\\
$ 55696.96804 $ & $   0.00103 $ & $   0.00097 $ & $  10.46580 $ & $ i$\\
$ 55696.96861 $ & $  -0.00229 $ & $   0.00097 $ & $  10.46230 $ & $ i$\\
$ 55696.96917 $ & $  -0.00150 $ & $   0.00097 $ & $  10.46350 $ & $ i$\\
$ 55696.96975 $ & $  -0.00180 $ & $   0.00097 $ & $  10.46410 $ & $ i$\\
$ 55696.97031 $ & $   0.00069 $ & $   0.00097 $ & $  10.46610 $ & $ i$\\
$ 55696.97088 $ & $   0.00034 $ & $   0.00097 $ & $  10.46630 $ & $ i$\\
$ 55696.97145 $ & $  -0.00105 $ & $   0.00097 $ & $  10.46360 $ & $ i$\\
$ 55696.97198 $ & $  -0.00168 $ & $   0.00097 $ & $  10.46270 $ & $ i$\\
$ 55696.97254 $ & $   0.00090 $ & $   0.00097 $ & $  10.46620 $ & $ i$\\
$ 55696.97309 $ & $  -0.00262 $ & $   0.00097 $ & $  10.46290 $ & $ i$\\
$ 55696.97366 $ & $   0.00350 $ & $   0.00097 $ & $  10.46840 $ & $ i$\\
$ 55696.97422 $ & $   0.00100 $ & $   0.00097 $ & $  10.46650 $ & $ i$\\
$ 55696.97478 $ & $  -0.00177 $ & $   0.00098 $ & $  10.46350 $ & $ i$\\
$ 55696.97534 $ & $   0.00059 $ & $   0.00098 $ & $  10.46580 $ & $ i$\\
$ 55696.97591 $ & $  -0.00011 $ & $   0.00097 $ & $  10.46530 $ & $ i$\\
$ 55696.97648 $ & $  -0.00008 $ & $   0.00098 $ & $  10.46510 $ & $ i$\\
$ 55696.97707 $ & $  -0.00121 $ & $   0.00098 $ & $  10.46340 $ & $ i$\\
$ 55696.97762 $ & $   0.00195 $ & $   0.00098 $ & $  10.46680 $ & $ i$\\
$ 55696.97821 $ & $   0.00078 $ & $   0.00098 $ & $  10.46670 $ & $ i$\\
$ 55696.97876 $ & $   0.00029 $ & $   0.00098 $ & $  10.46550 $ & $ i$\\
$ 55696.97934 $ & $  -0.00125 $ & $   0.00098 $ & $  10.46410 $ & $ i$\\
$ 55696.97992 $ & $  -0.00036 $ & $   0.00098 $ & $  10.46570 $ & $ i$\\
$ 55696.98049 $ & $   0.00042 $ & $   0.00098 $ & $  10.46550 $ & $ i$\\
$ 55696.98105 $ & $   0.00169 $ & $   0.00099 $ & $  10.46710 $ & $ i$\\
$ 55696.98162 $ & $   0.00121 $ & $   0.00099 $ & $  10.46640 $ & $ i$\\
$ 55696.98220 $ & $   0.00069 $ & $   0.00100 $ & $  10.46630 $ & $ i$\\
$ 55696.98276 $ & $   0.00130 $ & $   0.00100 $ & $  10.46710 $ & $ i$\\
$ 55696.98333 $ & $   0.00167 $ & $   0.00101 $ & $  10.46660 $ & $ i$\\
$ 55696.98391 $ & $   0.00155 $ & $   0.00102 $ & $  10.46690 $ & $ i$\\
$ 55696.98447 $ & $  -0.00018 $ & $   0.00102 $ & $  10.46470 $ & $ i$\\
$ 55696.98501 $ & $   0.00084 $ & $   0.00103 $ & $  10.46670 $ & $ i$\\
$ 55696.98558 $ & $   0.00331 $ & $   0.00104 $ & $  10.46920 $ & $ i$\\
$ 55696.98614 $ & $  -0.00311 $ & $   0.00105 $ & $  10.46300 $ & $ i$\\
$ 55696.98669 $ & $  -0.00284 $ & $   0.00106 $ & $  10.46330 $ & $ i$\\
$ 55705.76796 $ & $   0.00881 $ & $   0.00114 $ & $  10.37650 $ & $ i$\\
$ 55705.76841 $ & $   0.00749 $ & $   0.00114 $ & $  10.37540 $ & $ i$\\
$ 55705.76902 $ & $   0.01281 $ & $   0.00114 $ & $  10.38250 $ & $ i$\\
$ 55705.76948 $ & $   0.00952 $ & $   0.00114 $ & $  10.37840 $ & $ i$\\
$ 55705.76994 $ & $   0.00875 $ & $   0.00113 $ & $  10.37770 $ & $ i$\\
$ 55705.77038 $ & $   0.00938 $ & $   0.00114 $ & $  10.37750 $ & $ i$\\
$ 55705.77082 $ & $   0.01064 $ & $   0.00113 $ & $  10.37960 $ & $ i$\\
$ 55705.77143 $ & $   0.01185 $ & $   0.00113 $ & $  10.38130 $ & $ i$\\
$ 55705.77187 $ & $   0.00752 $ & $   0.00114 $ & $  10.37590 $ & $ i$\\
$ 55705.77232 $ & $   0.01247 $ & $   0.00113 $ & $  10.38080 $ & $ i$\\
$ 55705.77275 $ & $   0.01364 $ & $   0.00114 $ & $  10.38330 $ & $ i$\\
$ 55705.77321 $ & $   0.01099 $ & $   0.00113 $ & $  10.37830 $ & $ i$\\
$ 55705.77384 $ & $   0.00894 $ & $   0.00113 $ & $  10.37940 $ & $ i$\\
$ 55705.77429 $ & $   0.00887 $ & $   0.00113 $ & $  10.37790 $ & $ i$\\
$ 55705.77474 $ & $   0.00998 $ & $   0.00113 $ & $  10.37860 $ & $ i$\\
$ 55705.77519 $ & $   0.00961 $ & $   0.00113 $ & $  10.37820 $ & $ i$\\
$ 55705.77564 $ & $   0.00695 $ & $   0.00114 $ & $  10.37530 $ & $ i$\\
$ 55705.77628 $ & $   0.00855 $ & $   0.00113 $ & $  10.37780 $ & $ i$\\
$ 55705.77674 $ & $   0.00762 $ & $   0.00113 $ & $  10.37670 $ & $ i$\\
$ 55705.77718 $ & $   0.00981 $ & $   0.00113 $ & $  10.37830 $ & $ i$\\
$ 55705.77764 $ & $   0.00933 $ & $   0.00113 $ & $  10.37820 $ & $ i$\\
$ 55705.77808 $ & $   0.01234 $ & $   0.00113 $ & $  10.38140 $ & $ i$\\
$ 55705.77868 $ & $   0.00994 $ & $   0.00113 $ & $  10.37980 $ & $ i$\\
$ 55705.77914 $ & $   0.00804 $ & $   0.00113 $ & $  10.37650 $ & $ i$\\
$ 55705.77957 $ & $   0.01108 $ & $   0.00113 $ & $  10.37990 $ & $ i$\\
$ 55705.78002 $ & $   0.00789 $ & $   0.00113 $ & $  10.37770 $ & $ i$\\
$ 55705.78048 $ & $   0.01163 $ & $   0.00113 $ & $  10.38070 $ & $ i$\\
$ 55705.78110 $ & $   0.00806 $ & $   0.00113 $ & $  10.37740 $ & $ i$\\
$ 55705.78154 $ & $   0.01007 $ & $   0.00113 $ & $  10.37950 $ & $ i$\\
$ 55705.78200 $ & $   0.01154 $ & $   0.00113 $ & $  10.38080 $ & $ i$\\
$ 55705.78245 $ & $   0.00957 $ & $   0.00113 $ & $  10.37830 $ & $ i$\\
$ 55705.78289 $ & $   0.01068 $ & $   0.00113 $ & $  10.37950 $ & $ i$\\
$ 55705.78350 $ & $   0.01066 $ & $   0.00113 $ & $  10.37880 $ & $ i$\\
$ 55705.78394 $ & $   0.01093 $ & $   0.00113 $ & $  10.37970 $ & $ i$\\
$ 55705.78441 $ & $   0.00819 $ & $   0.00113 $ & $  10.37590 $ & $ i$\\
$ 55705.78486 $ & $   0.01428 $ & $   0.00113 $ & $  10.38220 $ & $ i$\\
$ 55705.78531 $ & $   0.01276 $ & $   0.00113 $ & $  10.38200 $ & $ i$\\
$ 55705.78596 $ & $   0.01083 $ & $   0.00113 $ & $  10.37950 $ & $ i$\\
$ 55705.78642 $ & $   0.00875 $ & $   0.00113 $ & $  10.37660 $ & $ i$\\
$ 55705.78688 $ & $   0.01197 $ & $   0.00113 $ & $  10.38120 $ & $ i$\\
$ 55705.78734 $ & $   0.01458 $ & $   0.00113 $ & $  10.38280 $ & $ i$\\
$ 55705.78779 $ & $   0.00966 $ & $   0.00113 $ & $  10.37910 $ & $ i$\\
$ 55705.78839 $ & $   0.00835 $ & $   0.00112 $ & $  10.37820 $ & $ i$\\
$ 55705.78885 $ & $   0.01233 $ & $   0.00113 $ & $  10.38120 $ & $ i$\\
$ 55705.78929 $ & $   0.00913 $ & $   0.00112 $ & $  10.37740 $ & $ i$\\
$ 55705.78972 $ & $   0.01014 $ & $   0.00113 $ & $  10.37890 $ & $ i$\\
$ 55705.79017 $ & $   0.00991 $ & $   0.00113 $ & $  10.37780 $ & $ i$\\
$ 55705.79081 $ & $   0.01145 $ & $   0.00113 $ & $  10.38020 $ & $ i$\\
$ 55705.79126 $ & $   0.01504 $ & $   0.00113 $ & $  10.38250 $ & $ i$\\
$ 55705.79171 $ & $   0.00979 $ & $   0.00113 $ & $  10.37800 $ & $ i$\\
$ 55705.79216 $ & $   0.01260 $ & $   0.00113 $ & $  10.37940 $ & $ i$\\
$ 55705.79259 $ & $   0.01267 $ & $   0.00113 $ & $  10.38090 $ & $ i$\\
$ 55705.79320 $ & $   0.00767 $ & $   0.00113 $ & $  10.37590 $ & $ i$\\
$ 55705.79365 $ & $   0.01066 $ & $   0.00113 $ & $  10.37940 $ & $ i$\\
$ 55705.79411 $ & $   0.00979 $ & $   0.00114 $ & $  10.37740 $ & $ i$\\
$ 55705.79453 $ & $   0.01191 $ & $   0.00114 $ & $  10.38030 $ & $ i$\\
$ 55705.79497 $ & $   0.01339 $ & $   0.00113 $ & $  10.38170 $ & $ i$\\
$ 55705.79560 $ & $   0.01512 $ & $   0.00114 $ & $  10.38250 $ & $ i$\\
$ 55705.79605 $ & $   0.00998 $ & $   0.00115 $ & $  10.37750 $ & $ i$\\
$ 55705.79650 $ & $   0.01001 $ & $   0.00115 $ & $  10.37760 $ & $ i$\\
$ 55705.79697 $ & $   0.01176 $ & $   0.00114 $ & $  10.37950 $ & $ i$\\
$ 55705.79743 $ & $   0.01305 $ & $   0.00113 $ & $  10.38140 $ & $ i$\\
$ 55705.79804 $ & $   0.01222 $ & $   0.00113 $ & $  10.38020 $ & $ i$\\
$ 55705.79850 $ & $   0.00942 $ & $   0.00113 $ & $  10.37730 $ & $ i$\\
$ 55705.79896 $ & $   0.01096 $ & $   0.00113 $ & $  10.37890 $ & $ i$\\
$ 55705.79941 $ & $   0.00849 $ & $   0.00113 $ & $  10.37580 $ & $ i$\\
$ 55705.79986 $ & $   0.00927 $ & $   0.00113 $ & $  10.37670 $ & $ i$\\
$ 55705.80048 $ & $   0.01036 $ & $   0.00113 $ & $  10.37850 $ & $ i$\\
$ 55705.80093 $ & $   0.01032 $ & $   0.00113 $ & $  10.37750 $ & $ i$\\
$ 55705.80139 $ & $   0.01100 $ & $   0.00114 $ & $  10.37820 $ & $ i$\\
$ 55705.80184 $ & $   0.00860 $ & $   0.00113 $ & $  10.37650 $ & $ i$\\
$ 55705.80229 $ & $   0.00919 $ & $   0.00113 $ & $  10.37640 $ & $ i$\\
$ 55705.80291 $ & $   0.00973 $ & $   0.00113 $ & $  10.37780 $ & $ i$\\
$ 55705.80338 $ & $   0.01104 $ & $   0.00113 $ & $  10.37820 $ & $ i$\\
$ 55705.80383 $ & $   0.00827 $ & $   0.00112 $ & $  10.37600 $ & $ i$\\
$ 55705.80428 $ & $   0.00950 $ & $   0.00113 $ & $  10.37760 $ & $ i$\\
$ 55705.80473 $ & $   0.00786 $ & $   0.00113 $ & $  10.37600 $ & $ i$\\
$ 55705.80537 $ & $   0.01043 $ & $   0.00113 $ & $  10.37850 $ & $ i$\\
$ 55705.80583 $ & $   0.01171 $ & $   0.00113 $ & $  10.38020 $ & $ i$\\
$ 55705.80629 $ & $   0.01372 $ & $   0.00113 $ & $  10.38130 $ & $ i$\\
$ 55705.80672 $ & $   0.01019 $ & $   0.00113 $ & $  10.37770 $ & $ i$\\
$ 55705.80717 $ & $   0.01269 $ & $   0.00113 $ & $  10.38130 $ & $ i$\\
$ 55705.80779 $ & $   0.00967 $ & $   0.00113 $ & $  10.37770 $ & $ i$\\
$ 55705.80824 $ & $   0.01040 $ & $   0.00113 $ & $  10.37830 $ & $ i$\\
$ 55705.80870 $ & $   0.00684 $ & $   0.00112 $ & $  10.37460 $ & $ i$\\
$ 55705.80917 $ & $   0.00633 $ & $   0.00112 $ & $  10.37480 $ & $ i$\\
$ 55705.80960 $ & $   0.00982 $ & $   0.00112 $ & $  10.37820 $ & $ i$\\
$ 55705.81024 $ & $   0.01160 $ & $   0.00112 $ & $  10.37950 $ & $ i$\\
$ 55705.81069 $ & $   0.00990 $ & $   0.00112 $ & $  10.37770 $ & $ i$\\
$ 55705.81114 $ & $   0.01129 $ & $   0.00113 $ & $  10.37960 $ & $ i$\\
$ 55705.81160 $ & $   0.00872 $ & $   0.00112 $ & $  10.37730 $ & $ i$\\
$ 55705.81205 $ & $   0.00717 $ & $   0.00112 $ & $  10.37490 $ & $ i$\\
$ 55705.81267 $ & $   0.01126 $ & $   0.00112 $ & $  10.38050 $ & $ i$\\
$ 55705.81314 $ & $   0.01220 $ & $   0.00113 $ & $  10.38110 $ & $ i$\\
$ 55705.81360 $ & $   0.01232 $ & $   0.00112 $ & $  10.38160 $ & $ i$\\
$ 55705.81403 $ & $   0.00867 $ & $   0.00113 $ & $  10.37770 $ & $ i$\\
$ 55705.81447 $ & $   0.01024 $ & $   0.00112 $ & $  10.37940 $ & $ i$\\
$ 55705.81509 $ & $   0.00800 $ & $   0.00114 $ & $  10.37560 $ & $ i$\\
$ 55705.81554 $ & $   0.00941 $ & $   0.00113 $ & $  10.37800 $ & $ i$\\
$ 55705.81597 $ & $   0.01089 $ & $   0.00113 $ & $  10.37820 $ & $ i$\\
$ 55705.81641 $ & $   0.01104 $ & $   0.00113 $ & $  10.38010 $ & $ i$\\
$ 55705.81686 $ & $   0.00665 $ & $   0.00112 $ & $  10.37580 $ & $ i$\\
$ 55705.81749 $ & $   0.00734 $ & $   0.00113 $ & $  10.37510 $ & $ i$\\
$ 55705.81795 $ & $   0.00703 $ & $   0.00112 $ & $  10.37520 $ & $ i$\\
$ 55705.81840 $ & $   0.01125 $ & $   0.00112 $ & $  10.37970 $ & $ i$\\
$ 55705.81885 $ & $   0.00866 $ & $   0.00113 $ & $  10.37690 $ & $ i$\\
$ 55705.81929 $ & $   0.00904 $ & $   0.00113 $ & $  10.37680 $ & $ i$\\
$ 55705.81991 $ & $   0.00807 $ & $   0.00112 $ & $  10.37690 $ & $ i$\\
$ 55705.82036 $ & $   0.01130 $ & $   0.00113 $ & $  10.37960 $ & $ i$\\
$ 55705.82080 $ & $   0.00857 $ & $   0.00113 $ & $  10.37740 $ & $ i$\\
$ 55705.82124 $ & $   0.01118 $ & $   0.00113 $ & $  10.37960 $ & $ i$\\
$ 55705.82167 $ & $   0.00862 $ & $   0.00112 $ & $  10.37690 $ & $ i$\\
$ 55705.82228 $ & $   0.00795 $ & $   0.00112 $ & $  10.37700 $ & $ i$\\
$ 55705.82274 $ & $   0.00757 $ & $   0.00112 $ & $  10.37590 $ & $ i$\\
$ 55705.82320 $ & $   0.01086 $ & $   0.00112 $ & $  10.37950 $ & $ i$\\
$ 55705.82364 $ & $   0.00757 $ & $   0.00112 $ & $  10.37530 $ & $ i$\\
$ 55705.82410 $ & $   0.00995 $ & $   0.00112 $ & $  10.37850 $ & $ i$\\
$ 55705.82474 $ & $   0.00985 $ & $   0.00112 $ & $  10.37850 $ & $ i$\\
$ 55705.82518 $ & $   0.00865 $ & $   0.00112 $ & $  10.37710 $ & $ i$\\
$ 55705.82565 $ & $   0.00937 $ & $   0.00112 $ & $  10.37790 $ & $ i$\\
$ 55705.82611 $ & $   0.00869 $ & $   0.00112 $ & $  10.37660 $ & $ i$\\
$ 55705.82654 $ & $   0.01059 $ & $   0.00112 $ & $  10.37940 $ & $ i$\\
$ 55705.82715 $ & $   0.01175 $ & $   0.00112 $ & $  10.38030 $ & $ i$\\
$ 55705.82761 $ & $   0.01169 $ & $   0.00113 $ & $  10.38030 $ & $ i$\\
$ 55705.82807 $ & $   0.01012 $ & $   0.00112 $ & $  10.37840 $ & $ i$\\
$ 55705.82852 $ & $   0.01015 $ & $   0.00112 $ & $  10.37870 $ & $ i$\\
$ 55705.82897 $ & $   0.00850 $ & $   0.00112 $ & $  10.37670 $ & $ i$\\
$ 55705.82961 $ & $   0.01282 $ & $   0.00112 $ & $  10.38140 $ & $ i$\\
$ 55705.83006 $ & $   0.00997 $ & $   0.00112 $ & $  10.37940 $ & $ i$\\
$ 55705.83051 $ & $   0.01426 $ & $   0.00112 $ & $  10.38230 $ & $ i$\\
$ 55705.83097 $ & $   0.01017 $ & $   0.00112 $ & $  10.37810 $ & $ i$\\
$ 55705.83142 $ & $   0.00925 $ & $   0.00112 $ & $  10.37670 $ & $ i$\\
$ 55705.83204 $ & $   0.01463 $ & $   0.00112 $ & $  10.38350 $ & $ i$\\
$ 55705.83250 $ & $   0.01095 $ & $   0.00112 $ & $  10.37950 $ & $ i$\\
$ 55705.83295 $ & $   0.01101 $ & $   0.00112 $ & $  10.37960 $ & $ i$\\
$ 55705.83340 $ & $   0.01098 $ & $   0.00113 $ & $  10.37950 $ & $ i$\\
$ 55705.83387 $ & $   0.01083 $ & $   0.00112 $ & $  10.37960 $ & $ i$\\
$ 55705.83447 $ & $   0.01318 $ & $   0.00112 $ & $  10.38190 $ & $ i$\\
$ 55705.83493 $ & $   0.01048 $ & $   0.00112 $ & $  10.37890 $ & $ i$\\
$ 55705.83538 $ & $   0.00627 $ & $   0.00112 $ & $  10.37520 $ & $ i$\\
$ 55705.83583 $ & $   0.01006 $ & $   0.00112 $ & $  10.37930 $ & $ i$\\
$ 55705.83626 $ & $   0.01309 $ & $   0.00113 $ & $  10.38190 $ & $ i$\\
$ 55705.83689 $ & $   0.00793 $ & $   0.00112 $ & $  10.37700 $ & $ i$\\
$ 55705.83734 $ & $   0.01151 $ & $   0.00113 $ & $  10.38060 $ & $ i$\\
$ 55705.83778 $ & $   0.00666 $ & $   0.00112 $ & $  10.37510 $ & $ i$\\
$ 55705.83821 $ & $   0.01188 $ & $   0.00112 $ & $  10.38060 $ & $ i$\\
$ 55705.83866 $ & $   0.01119 $ & $   0.00112 $ & $  10.37930 $ & $ i$\\
$ 55705.83927 $ & $   0.00697 $ & $   0.00112 $ & $  10.37570 $ & $ i$\\
$ 55705.83971 $ & $   0.00916 $ & $   0.00112 $ & $  10.37790 $ & $ i$\\
$ 55705.84015 $ & $   0.00933 $ & $   0.00112 $ & $  10.37800 $ & $ i$\\
$ 55705.84061 $ & $   0.00713 $ & $   0.00112 $ & $  10.37630 $ & $ i$\\
$ 55705.84106 $ & $   0.00569 $ & $   0.00112 $ & $  10.37510 $ & $ i$\\
$ 55705.84168 $ & $   0.01111 $ & $   0.00112 $ & $  10.37980 $ & $ i$\\
$ 55705.84214 $ & $   0.00649 $ & $   0.00112 $ & $  10.37450 $ & $ i$\\
$ 55705.84258 $ & $   0.00982 $ & $   0.00112 $ & $  10.37850 $ & $ i$\\
$ 55705.84304 $ & $   0.01174 $ & $   0.00112 $ & $  10.38000 $ & $ i$\\
$ 55705.84349 $ & $   0.01027 $ & $   0.00112 $ & $  10.37960 $ & $ i$\\
$ 55705.84413 $ & $   0.00913 $ & $   0.00111 $ & $  10.37800 $ & $ i$\\
$ 55705.84459 $ & $   0.00811 $ & $   0.00112 $ & $  10.37640 $ & $ i$\\
$ 55705.84502 $ & $   0.00721 $ & $   0.00112 $ & $  10.37600 $ & $ i$\\
$ 55705.84546 $ & $   0.00920 $ & $   0.00112 $ & $  10.37810 $ & $ i$\\
$ 55705.84589 $ & $   0.00787 $ & $   0.00112 $ & $  10.37690 $ & $ i$\\
$ 55705.84652 $ & $   0.00771 $ & $   0.00111 $ & $  10.37740 $ & $ i$\\
$ 55705.84697 $ & $   0.00892 $ & $   0.00112 $ & $  10.37690 $ & $ i$\\
$ 55705.84741 $ & $   0.00668 $ & $   0.00112 $ & $  10.37510 $ & $ i$\\
$ 55705.84785 $ & $   0.00831 $ & $   0.00112 $ & $  10.37660 $ & $ i$\\
$ 55705.84829 $ & $   0.00899 $ & $   0.00112 $ & $  10.37780 $ & $ i$\\
$ 55705.84888 $ & $   0.00632 $ & $   0.00112 $ & $  10.37550 $ & $ i$\\
$ 55705.84933 $ & $   0.00801 $ & $   0.00113 $ & $  10.37640 $ & $ i$\\
$ 55705.84977 $ & $   0.00776 $ & $   0.00112 $ & $  10.37660 $ & $ i$\\
$ 55705.85021 $ & $   0.00822 $ & $   0.00113 $ & $  10.37700 $ & $ i$\\
$ 55705.85065 $ & $   0.00509 $ & $   0.00112 $ & $  10.37400 $ & $ i$\\
$ 55705.85126 $ & $   0.00262 $ & $   0.00112 $ & $  10.37270 $ & $ i$\\
$ 55705.85171 $ & $   0.00651 $ & $   0.00112 $ & $  10.37640 $ & $ i$\\
$ 55705.85216 $ & $   0.00445 $ & $   0.00113 $ & $  10.37450 $ & $ i$\\
$ 55705.85259 $ & $   0.00864 $ & $   0.00112 $ & $  10.37770 $ & $ i$\\
$ 55705.85369 $ & $   0.00274 $ & $   0.00112 $ & $  10.37230 $ & $ i$\\
$ 55705.85417 $ & $   0.00210 $ & $   0.00112 $ & $  10.37240 $ & $ i$\\
$ 55705.85461 $ & $   0.00398 $ & $   0.00112 $ & $  10.37440 $ & $ i$\\
$ 55705.85505 $ & $   0.00115 $ & $   0.00111 $ & $  10.37020 $ & $ i$\\
$ 55705.85549 $ & $   0.00119 $ & $   0.00111 $ & $  10.37020 $ & $ i$\\
$ 55705.85611 $ & $   0.00567 $ & $   0.00112 $ & $  10.37610 $ & $ i$\\
$ 55705.85655 $ & $   0.00316 $ & $   0.00112 $ & $  10.37300 $ & $ i$\\
$ 55705.85700 $ & $   0.00439 $ & $   0.00112 $ & $  10.37380 $ & $ i$\\
$ 55705.85744 $ & $   0.00202 $ & $   0.00112 $ & $  10.37210 $ & $ i$\\
$ 55705.85787 $ & $   0.00666 $ & $   0.00112 $ & $  10.37630 $ & $ i$\\
$ 55705.85848 $ & $   0.00035 $ & $   0.00112 $ & $  10.37030 $ & $ i$\\
$ 55705.85894 $ & $   0.00094 $ & $   0.00111 $ & $  10.37130 $ & $ i$\\
$ 55705.85938 $ & $   0.00632 $ & $   0.00111 $ & $  10.37650 $ & $ i$\\
$ 55705.85983 $ & $  -0.00077 $ & $   0.00112 $ & $  10.37010 $ & $ i$\\
$ 55705.86028 $ & $  -0.00036 $ & $   0.00112 $ & $  10.36940 $ & $ i$\\
$ 55705.86088 $ & $   0.00201 $ & $   0.00112 $ & $  10.37160 $ & $ i$\\
$ 55705.86133 $ & $   0.00225 $ & $   0.00112 $ & $  10.37210 $ & $ i$\\
$ 55705.86179 $ & $   0.00127 $ & $   0.00112 $ & $  10.37140 $ & $ i$\\
$ 55705.86223 $ & $   0.00435 $ & $   0.00112 $ & $  10.37470 $ & $ i$\\
$ 55705.86267 $ & $   0.00051 $ & $   0.00111 $ & $  10.37110 $ & $ i$\\
$ 55705.86331 $ & $  -0.00098 $ & $   0.00111 $ & $  10.37040 $ & $ i$\\
$ 55705.86377 $ & $  -0.00116 $ & $   0.00111 $ & $  10.36900 $ & $ i$\\
$ 55705.86420 $ & $  -0.00372 $ & $   0.00111 $ & $  10.36760 $ & $ i$\\
$ 55705.86465 $ & $   0.00237 $ & $   0.00111 $ & $  10.37310 $ & $ i$\\
$ 55705.86512 $ & $   0.00083 $ & $   0.00111 $ & $  10.37130 $ & $ i$\\
$ 55705.86572 $ & $  -0.00138 $ & $   0.00111 $ & $  10.36910 $ & $ i$\\
$ 55705.86618 $ & $   0.00039 $ & $   0.00111 $ & $  10.37080 $ & $ i$\\
$ 55705.86664 $ & $  -0.00008 $ & $   0.00111 $ & $  10.37070 $ & $ i$\\
$ 55705.86707 $ & $  -0.00147 $ & $   0.00111 $ & $  10.36820 $ & $ i$\\
$ 55705.86751 $ & $  -0.00064 $ & $   0.00111 $ & $  10.37030 $ & $ i$\\
$ 55705.86810 $ & $  -0.00057 $ & $   0.00112 $ & $  10.37000 $ & $ i$\\
$ 55705.86857 $ & $  -0.00288 $ & $   0.00111 $ & $  10.36770 $ & $ i$\\
$ 55705.86899 $ & $   0.00332 $ & $   0.00111 $ & $  10.37380 $ & $ i$\\
$ 55705.86943 $ & $   0.00064 $ & $   0.00111 $ & $  10.37110 $ & $ i$\\
$ 55705.86987 $ & $  -0.00037 $ & $   0.00111 $ & $  10.36980 $ & $ i$\\
$ 55705.87049 $ & $  -0.00127 $ & $   0.00111 $ & $  10.36940 $ & $ i$\\
$ 55705.87094 $ & $   0.00029 $ & $   0.00111 $ & $  10.37030 $ & $ i$\\
$ 55705.87139 $ & $  -0.00021 $ & $   0.00111 $ & $  10.37000 $ & $ i$\\
$ 55705.87184 $ & $   0.00493 $ & $   0.00112 $ & $  10.37560 $ & $ i$\\
$ 55705.87229 $ & $  -0.00377 $ & $   0.00111 $ & $  10.36530 $ & $ i$\\
$ 55705.87293 $ & $  -0.00278 $ & $   0.00111 $ & $  10.36700 $ & $ i$\\
$ 55705.87339 $ & $   0.00011 $ & $   0.00111 $ & $  10.37050 $ & $ i$\\
$ 55705.87383 $ & $   0.00014 $ & $   0.00111 $ & $  10.37110 $ & $ i$\\
$ 55705.87428 $ & $  -0.00054 $ & $   0.00111 $ & $  10.37000 $ & $ i$\\
$ 55705.87472 $ & $   0.00065 $ & $   0.00111 $ & $  10.37090 $ & $ i$\\
$ 55705.87536 $ & $  -0.00114 $ & $   0.00112 $ & $  10.37050 $ & $ i$\\
$ 55705.87580 $ & $   0.00402 $ & $   0.00112 $ & $  10.37590 $ & $ i$\\
$ 55705.87626 $ & $  -0.00165 $ & $   0.00112 $ & $  10.36940 $ & $ i$\\
$ 55705.87673 $ & $  -0.00094 $ & $   0.00111 $ & $  10.37070 $ & $ i$\\
$ 55705.87718 $ & $   0.00192 $ & $   0.00112 $ & $  10.37390 $ & $ i$\\
$ 55705.87781 $ & $  -0.00267 $ & $   0.00111 $ & $  10.36850 $ & $ i$\\
$ 55705.87827 $ & $  -0.00033 $ & $   0.00112 $ & $  10.37100 $ & $ i$\\
$ 55705.87871 $ & $  -0.00016 $ & $   0.00111 $ & $  10.37040 $ & $ i$\\
$ 55705.87913 $ & $   0.00294 $ & $   0.00111 $ & $  10.37390 $ & $ i$\\
$ 55705.87960 $ & $   0.00044 $ & $   0.00112 $ & $  10.37080 $ & $ i$\\
$ 55705.88020 $ & $   0.00202 $ & $   0.00112 $ & $  10.37410 $ & $ i$\\
$ 55705.88065 $ & $  -0.00121 $ & $   0.00111 $ & $  10.37030 $ & $ i$\\
$ 55705.88109 $ & $   0.00220 $ & $   0.00112 $ & $  10.37300 $ & $ i$\\
$ 55705.88153 $ & $  -0.00087 $ & $   0.00112 $ & $  10.37060 $ & $ i$\\
$ 55705.88198 $ & $  -0.00307 $ & $   0.00111 $ & $  10.36930 $ & $ i$\\
$ 55705.88261 $ & $   0.00024 $ & $   0.00111 $ & $  10.37240 $ & $ i$\\
$ 55705.88306 $ & $  -0.00115 $ & $   0.00112 $ & $  10.37110 $ & $ i$\\


==> data/HTR432-011_phfu_tab_short.tex <==
$ 55687.79447 $ & $  -0.00440 $ & $   0.00112 $ & $  10.45700 $ & $ i$\\
$ 55687.79497 $ & $   0.00288 $ & $   0.00113 $ & $  10.46460 $ & $ i$\\
$ 55687.79596 $ & $  -0.00087 $ & $   0.00113 $ & $  10.46190 $ & $ i$\\
$ 55687.79647 $ & $  -0.00065 $ & $   0.00113 $ & $  10.46210 $ & $ i$\\
$ 55687.79699 $ & $  -0.00327 $ & $   0.00112 $ & $  10.45850 $ & $ i$\\
$ 55687.79749 $ & $   0.00222 $ & $   0.00112 $ & $  10.46330 $ & $ i$\\
$ 55687.79798 $ & $   0.00089 $ & $   0.00113 $ & $  10.46300 $ & $ i$\\
$ 55687.79850 $ & $  -0.00339 $ & $   0.00112 $ & $  10.45840 $ & $ i$\\
$ 55687.79901 $ & $   0.00378 $ & $   0.00112 $ & $  10.46610 $ & $ i$\\
$ 55687.79952 $ & $   0.00308 $ & $   0.00113 $ & $  10.46470 $ & $ i$\\


==> data/HTR432-011_rvtable.tex <==
$ 1696.90831 $ & $    -3.49 $ & $     5.78 $ & $    -3.77 $ & $     5.30 $ & $    0.1310 $ & $   0.008 $\\
$ 1696.91767 $ & \nodata      & \nodata      & $    13.10 $ & $     8.21 $ & $    0.1280 $ & $   0.010 $\\
$ 1697.89794 $ & $   -60.41 $ & $     5.22 $ & $     3.55 $ & $     4.74 $ & $    0.1290 $ & $   0.230 $\\
$ 1698.90686 $ & $   -38.37 $ & $     5.28 $ & $    -0.87 $ & $    10.21 $ & $    0.1510 $ & $   0.456 $\\
$ 1699.89562 $ & $    -0.43 $ & $     4.90 $ & $    -1.79 $ & $     3.95 $ & $    0.1250 $ & $   0.677 $\\
$ 1703.89107 $ & $   -24.17 $ & $     4.57 $ & $     4.96 $ & $     5.79 $ & $    0.1260 $ & $   0.572 $\\
$ 1704.88237 $ & $    -3.19 $ & $     5.33 $ & $     2.79 $ & $     8.88 $ & $    0.1240 $ & $   0.794 $\\
$ 1705.87529 $ & $   -55.16 $ & $     5.20 $ & $    -9.04 $ & $     7.16 $ & $    0.1270 $ & $   0.017 $\\
$ 1706.87230 $ & $  -115.33 $ & $     5.57 $ & $    -1.42 $ & $     3.72 $ & $    0.1270 $ & $   0.240 $\\
$ 1853.71982 $ & $   -63.30 $ & $     5.34 $ & \nodata      & \nodata      & \nodata      & $   0.143 $\\
$ 1997.09764 $ & $    20.23 $ & $    13.90 $ & \nodata      & \nodata      & \nodata      & $   0.268 $\\
$ 2113.77814 $ & $   -87.17 $ & $     6.61 $ & \nodata      & \nodata      & \nodata      & $   0.411 $\\
$ 2195.72876 $ & $    26.55 $ & $     5.74 $ & \nodata      & \nodata      & \nodata      & $   0.773 $\\


==> data/HTR433-003_phfu_tab.tex <==
$ 55654.89724 $ & $   0.01314 $ & $   0.00112 $ & $  11.34410 $ & $ i$\\
$ 55654.89809 $ & $   0.01315 $ & $   0.00112 $ & $  11.34380 $ & $ i$\\
$ 55654.89894 $ & $   0.01560 $ & $   0.00112 $ & $  11.34390 $ & $ i$\\
$ 55654.89981 $ & $   0.01522 $ & $   0.00112 $ & $  11.34580 $ & $ i$\\
$ 55654.90065 $ & $   0.01456 $ & $   0.00113 $ & $  11.34380 $ & $ i$\\
$ 55654.90152 $ & $   0.01758 $ & $   0.00112 $ & $  11.34740 $ & $ i$\\
$ 55654.90235 $ & $   0.01425 $ & $   0.00112 $ & $  11.34350 $ & $ i$\\
$ 55654.90322 $ & $   0.01632 $ & $   0.00112 $ & $  11.34700 $ & $ i$\\
$ 55654.90407 $ & $   0.01552 $ & $   0.00113 $ & $  11.34650 $ & $ i$\\
$ 55654.90491 $ & $   0.01267 $ & $   0.00112 $ & $  11.34330 $ & $ i$\\
$ 55654.90577 $ & $   0.01688 $ & $   0.00113 $ & $  11.34770 $ & $ i$\\
$ 55654.90662 $ & $   0.01535 $ & $   0.00112 $ & $  11.34620 $ & $ i$\\
$ 55654.90749 $ & $   0.01581 $ & $   0.00112 $ & $  11.34470 $ & $ i$\\
$ 55654.90835 $ & $   0.01709 $ & $   0.00112 $ & $  11.34730 $ & $ i$\\
$ 55654.90920 $ & $   0.01419 $ & $   0.00112 $ & $  11.34550 $ & $ i$\\
$ 55654.91004 $ & $   0.01360 $ & $   0.00113 $ & $  11.34550 $ & $ i$\\
$ 55654.91090 $ & $   0.01764 $ & $   0.00114 $ & $  11.34850 $ & $ i$\\
$ 55654.91172 $ & $   0.01572 $ & $   0.00114 $ & $  11.34520 $ & $ i$\\
$ 55654.91256 $ & $   0.01795 $ & $   0.00114 $ & $  11.34830 $ & $ i$\\
$ 55654.91340 $ & $   0.01382 $ & $   0.00114 $ & $  11.34650 $ & $ i$\\
$ 55654.91425 $ & $   0.01660 $ & $   0.00114 $ & $  11.34690 $ & $ i$\\
$ 55654.91510 $ & $   0.01941 $ & $   0.00114 $ & $  11.34770 $ & $ i$\\
$ 55654.91594 $ & $   0.01457 $ & $   0.00114 $ & $  11.34360 $ & $ i$\\
$ 55654.91679 $ & $   0.01336 $ & $   0.00113 $ & $  11.34290 $ & $ i$\\
$ 55654.91763 $ & $   0.01605 $ & $   0.00115 $ & $  11.34540 $ & $ i$\\
$ 55654.91849 $ & $   0.01362 $ & $   0.00115 $ & $  11.34470 $ & $ i$\\
$ 55654.91936 $ & $   0.01265 $ & $   0.00112 $ & $  11.34300 $ & $ i$\\
$ 55654.92021 $ & $   0.00944 $ & $   0.00112 $ & $  11.34120 $ & $ i$\\
$ 55654.92106 $ & $   0.01388 $ & $   0.00112 $ & $  11.34490 $ & $ i$\\
$ 55654.92193 $ & $   0.01420 $ & $   0.00112 $ & $  11.34410 $ & $ i$\\
$ 55654.92277 $ & $   0.01302 $ & $   0.00114 $ & $  11.34510 $ & $ i$\\
$ 55654.92362 $ & $   0.01733 $ & $   0.00112 $ & $  11.34720 $ & $ i$\\
$ 55654.92447 $ & $   0.00942 $ & $   0.00114 $ & $  11.33870 $ & $ i$\\
$ 55654.92533 $ & $   0.01435 $ & $   0.00118 $ & $  11.34570 $ & $ i$\\
$ 55654.92617 $ & $   0.01871 $ & $   0.00112 $ & $  11.34870 $ & $ i$\\
$ 55654.92703 $ & $   0.01508 $ & $   0.00111 $ & $  11.34530 $ & $ i$\\
$ 55654.92789 $ & $   0.01396 $ & $   0.00111 $ & $  11.34450 $ & $ i$\\
$ 55654.92876 $ & $   0.01430 $ & $   0.00114 $ & $  11.34550 $ & $ i$\\
$ 55654.92960 $ & $   0.00887 $ & $   0.00118 $ & $  11.34120 $ & $ i$\\
$ 55654.93046 $ & $   0.01757 $ & $   0.00118 $ & $  11.34900 $ & $ i$\\
$ 55654.93130 $ & $   0.01352 $ & $   0.00120 $ & $  11.34400 $ & $ i$\\
$ 55654.93216 $ & $   0.01211 $ & $   0.00122 $ & $  11.34310 $ & $ i$\\
$ 55654.93302 $ & $   0.01288 $ & $   0.00118 $ & $  11.34460 $ & $ i$\\
$ 55654.93387 $ & $   0.01198 $ & $   0.00120 $ & $  11.34490 $ & $ i$\\
$ 55654.93473 $ & $   0.01365 $ & $   0.00114 $ & $  11.34490 $ & $ i$\\
$ 55654.93558 $ & $   0.01242 $ & $   0.00111 $ & $  11.34340 $ & $ i$\\
$ 55654.93643 $ & $   0.01440 $ & $   0.00113 $ & $  11.34920 $ & $ i$\\
$ 55654.93727 $ & $   0.01122 $ & $   0.00115 $ & $  11.34570 $ & $ i$\\
$ 55654.93813 $ & $   0.01637 $ & $   0.00114 $ & $  11.34910 $ & $ i$\\
$ 55654.93899 $ & $   0.01192 $ & $   0.00111 $ & $  11.34420 $ & $ i$\\
$ 55654.93986 $ & $   0.01570 $ & $   0.00112 $ & $  11.34650 $ & $ i$\\
$ 55654.94069 $ & $   0.01154 $ & $   0.00111 $ & $  11.34260 $ & $ i$\\
$ 55654.94155 $ & $   0.01406 $ & $   0.00111 $ & $  11.34410 $ & $ i$\\
$ 55654.94241 $ & $   0.01530 $ & $   0.00111 $ & $  11.34650 $ & $ i$\\
$ 55654.94326 $ & $   0.01575 $ & $   0.00111 $ & $  11.34610 $ & $ i$\\
$ 55654.94412 $ & $   0.01263 $ & $   0.00111 $ & $  11.34310 $ & $ i$\\
$ 55654.94495 $ & $   0.01471 $ & $   0.00111 $ & $  11.34510 $ & $ i$\\
$ 55654.94582 $ & $   0.01344 $ & $   0.00110 $ & $  11.34370 $ & $ i$\\
$ 55654.94667 $ & $   0.01186 $ & $   0.00110 $ & $  11.34240 $ & $ i$\\
$ 55654.94752 $ & $   0.00874 $ & $   0.00111 $ & $  11.34050 $ & $ i$\\
$ 55654.94838 $ & $   0.01440 $ & $   0.00111 $ & $  11.34520 $ & $ i$\\
$ 55654.94924 $ & $   0.01104 $ & $   0.00111 $ & $  11.34300 $ & $ i$\\
$ 55654.95010 $ & $   0.00600 $ & $   0.00111 $ & $  11.33790 $ & $ i$\\
$ 55654.95097 $ & $   0.00778 $ & $   0.00111 $ & $  11.33930 $ & $ i$\\
$ 55654.95181 $ & $   0.00709 $ & $   0.00112 $ & $  11.33980 $ & $ i$\\
$ 55654.95267 $ & $   0.00894 $ & $   0.00114 $ & $  11.34030 $ & $ i$\\
$ 55654.95354 $ & $   0.00309 $ & $   0.00112 $ & $  11.33420 $ & $ i$\\
$ 55654.95438 $ & $   0.00696 $ & $   0.00112 $ & $  11.33690 $ & $ i$\\
$ 55654.95525 $ & $   0.00405 $ & $   0.00112 $ & $  11.33580 $ & $ i$\\
$ 55654.95611 $ & $   0.00296 $ & $   0.00111 $ & $  11.33370 $ & $ i$\\
$ 55654.95695 $ & $   0.00408 $ & $   0.00114 $ & $  11.33570 $ & $ i$\\
$ 55654.95780 $ & $   0.00234 $ & $   0.00114 $ & $  11.33400 $ & $ i$\\
$ 55654.95867 $ & $   0.00392 $ & $   0.00116 $ & $  11.33480 $ & $ i$\\
$ 55654.95951 $ & $  -0.00366 $ & $   0.00116 $ & $  11.32790 $ & $ i$\\
$ 55654.96033 $ & $   0.00174 $ & $   0.00113 $ & $  11.33210 $ & $ i$\\
$ 55654.96121 $ & $   0.00371 $ & $   0.00114 $ & $  11.33390 $ & $ i$\\
$ 55654.96205 $ & $  -0.00088 $ & $   0.00116 $ & $  11.33050 $ & $ i$\\
$ 55654.96291 $ & $   0.00041 $ & $   0.00116 $ & $  11.33120 $ & $ i$\\
$ 55654.96377 $ & $   0.00024 $ & $   0.00115 $ & $  11.33030 $ & $ i$\\
$ 55654.96460 $ & $   0.00165 $ & $   0.00116 $ & $  11.33160 $ & $ i$\\
$ 55654.96547 $ & $  -0.00262 $ & $   0.00115 $ & $  11.32940 $ & $ i$\\
$ 55654.96633 $ & $  -0.00016 $ & $   0.00122 $ & $  11.32950 $ & $ i$\\
$ 55654.96717 $ & $  -0.00181 $ & $   0.00118 $ & $  11.32710 $ & $ i$\\
$ 55654.96804 $ & $  -0.00088 $ & $   0.00116 $ & $  11.33050 $ & $ i$\\
$ 55654.96890 $ & $  -0.00091 $ & $   0.00116 $ & $  11.32810 $ & $ i$\\
$ 55654.96975 $ & $   0.00097 $ & $   0.00116 $ & $  11.33130 $ & $ i$\\
$ 55654.97060 $ & $  -0.00122 $ & $   0.00115 $ & $  11.32860 $ & $ i$\\
$ 55654.97144 $ & $   0.00117 $ & $   0.00112 $ & $  11.32990 $ & $ i$\\
$ 55654.97231 $ & $  -0.00004 $ & $   0.00118 $ & $  11.33150 $ & $ i$\\
$ 55654.97318 $ & $  -0.00036 $ & $   0.00117 $ & $  11.33000 $ & $ i$\\
$ 55654.97401 $ & $   0.00086 $ & $   0.00124 $ & $  11.32940 $ & $ i$\\
$ 55654.97487 $ & $   0.00061 $ & $   0.00120 $ & $  11.33090 $ & $ i$\\
$ 55654.97574 $ & $   0.00057 $ & $   0.00118 $ & $  11.33080 $ & $ i$\\
$ 55654.97656 $ & $  -0.00094 $ & $   0.00118 $ & $  11.32880 $ & $ i$\\
$ 55654.97743 $ & $   0.00333 $ & $   0.00121 $ & $  11.33470 $ & $ i$\\
$ 55654.97827 $ & $  -0.00196 $ & $   0.00124 $ & $  11.32610 $ & $ i$\\
$ 55654.97912 $ & $   0.00207 $ & $   0.00115 $ & $  11.33100 $ & $ i$\\
$ 55654.97996 $ & $  -0.00131 $ & $   0.00121 $ & $  11.32920 $ & $ i$\\
$ 55654.98082 $ & $  -0.00113 $ & $   0.00116 $ & $  11.32850 $ & $ i$\\
$ 55654.98169 $ & $  -0.00187 $ & $   0.00115 $ & $  11.32660 $ & $ i$\\
$ 55654.98256 $ & $   0.00092 $ & $   0.00117 $ & $  11.33410 $ & $ i$\\
$ 55654.98360 $ & $  -0.00131 $ & $   0.00117 $ & $  11.32990 $ & $ i$\\
$ 55654.98452 $ & $  -0.00045 $ & $   0.00123 $ & $  11.33000 $ & $ i$\\
$ 55654.98537 $ & $  -0.00139 $ & $   0.00118 $ & $  11.32820 $ & $ i$\\
$ 55654.98623 $ & $  -0.00035 $ & $   0.00115 $ & $  11.32910 $ & $ i$\\
$ 55654.98708 $ & $  -0.00119 $ & $   0.00114 $ & $  11.32820 $ & $ i$\\
$ 55654.98795 $ & $  -0.00109 $ & $   0.00116 $ & $  11.32740 $ & $ i$\\
$ 55654.98881 $ & $   0.00198 $ & $   0.00119 $ & $  11.33110 $ & $ i$\\
$ 55654.98966 $ & $  -0.00107 $ & $   0.00121 $ & $  11.32850 $ & $ i$\\
$ 55654.99051 $ & $   0.00144 $ & $   0.00119 $ & $  11.33050 $ & $ i$\\
$ 55654.99137 $ & $   0.00111 $ & $   0.00119 $ & $  11.33340 $ & $ i$\\
$ 55654.99222 $ & $   0.00132 $ & $   0.00118 $ & $  11.33010 $ & $ i$\\
$ 55654.99308 $ & $  -0.00014 $ & $   0.00122 $ & $  11.32820 $ & $ i$\\
$ 55654.99393 $ & $  -0.00062 $ & $   0.00121 $ & $  11.32990 $ & $ i$\\
$ 55654.99479 $ & $  -0.00316 $ & $   0.00123 $ & $  11.32820 $ & $ i$\\
$ 55654.99564 $ & $   0.00193 $ & $   0.00124 $ & $  11.33320 $ & $ i$\\
$ 55654.99649 $ & $  -0.00014 $ & $   0.00125 $ & $  11.32970 $ & $ i$\\
$ 55654.99734 $ & $   0.00195 $ & $   0.00122 $ & $  11.33180 $ & $ i$\\
$ 55654.99819 $ & $   0.00062 $ & $   0.00123 $ & $  11.33060 $ & $ i$\\
$ 55654.99906 $ & $  -0.00207 $ & $   0.00130 $ & $  11.32990 $ & $ i$\\
$ 55654.99991 $ & $   0.00186 $ & $   0.00125 $ & $  11.33260 $ & $ i$\\
$ 55655.00076 $ & $  -0.00163 $ & $   0.00124 $ & $  11.32920 $ & $ i$\\
$ 55655.00164 $ & $   0.00217 $ & $   0.00128 $ & $  11.33050 $ & $ i$\\
$ 55655.00248 $ & $   0.00212 $ & $   0.00127 $ & $  11.33270 $ & $ i$\\
$ 55655.00335 $ & $  -0.00254 $ & $   0.00126 $ & $  11.32800 $ & $ i$\\
$ 55655.00421 $ & $  -0.00150 $ & $   0.00124 $ & $  11.32860 $ & $ i$\\
$ 55655.00507 $ & $   0.00229 $ & $   0.00128 $ & $  11.33260 $ & $ i$\\
$ 55655.00591 $ & $   0.00238 $ & $   0.00125 $ & $  11.33170 $ & $ i$\\
$ 55655.00676 $ & $  -0.00102 $ & $   0.00131 $ & $  11.33030 $ & $ i$\\
$ 55655.00763 $ & $   0.00112 $ & $   0.00126 $ & $  11.33150 $ & $ i$\\
$ 55655.00846 $ & $  -0.00295 $ & $   0.00124 $ & $  11.32780 $ & $ i$\\
$ 55655.00932 $ & $   0.00169 $ & $   0.00132 $ & $  11.33030 $ & $ i$\\
$ 55655.01018 $ & $  -0.00213 $ & $   0.00143 $ & $  11.32890 $ & $ i$\\
$ 55657.90089 $ & $   0.00400 $ & $   0.00089 $ & $  11.21250 $ & $ i$\\
$ 55657.90215 $ & $  -0.00038 $ & $   0.00089 $ & $  11.20790 $ & $ i$\\
$ 55657.90335 $ & $  -0.00243 $ & $   0.00088 $ & $  11.20620 $ & $ i$\\
$ 55657.90455 $ & $   0.00026 $ & $   0.00089 $ & $  11.20710 $ & $ i$\\
$ 55657.90574 $ & $  -0.00157 $ & $   0.00088 $ & $  11.20800 $ & $ i$\\
$ 55657.90813 $ & $  -0.00232 $ & $   0.00089 $ & $  11.20850 $ & $ i$\\
$ 55657.90929 $ & $  -0.00173 $ & $   0.00089 $ & $  11.20410 $ & $ i$\\
$ 55657.91048 $ & $   0.00145 $ & $   0.00089 $ & $  11.20860 $ & $ i$\\
$ 55657.91168 $ & $  -0.00171 $ & $   0.00088 $ & $  11.20700 $ & $ i$\\
$ 55657.91288 $ & $   0.00158 $ & $   0.00089 $ & $  11.21240 $ & $ i$\\
$ 55657.91409 $ & $  -0.00007 $ & $   0.00088 $ & $  11.20840 $ & $ i$\\
$ 55657.91527 $ & $   0.00065 $ & $   0.00088 $ & $  11.20920 $ & $ i$\\
$ 55657.91646 $ & $   0.00255 $ & $   0.00089 $ & $  11.21270 $ & $ i$\\
$ 55657.91765 $ & $   0.00394 $ & $   0.00089 $ & $  11.21230 $ & $ i$\\
$ 55657.91886 $ & $  -0.00098 $ & $   0.00088 $ & $  11.20830 $ & $ i$\\
$ 55657.92006 $ & $  -0.00098 $ & $   0.00088 $ & $  11.20940 $ & $ i$\\
$ 55657.92127 $ & $   0.00263 $ & $   0.00089 $ & $  11.20880 $ & $ i$\\
$ 55657.92246 $ & $  -0.00345 $ & $   0.00088 $ & $  11.20420 $ & $ i$\\
$ 55657.92366 $ & $   0.00065 $ & $   0.00090 $ & $  11.20530 $ & $ i$\\
$ 55657.92485 $ & $  -0.00225 $ & $   0.00088 $ & $  11.20360 $ & $ i$\\
$ 55657.92608 $ & $   0.00078 $ & $   0.00088 $ & $  11.20870 $ & $ i$\\
$ 55657.92727 $ & $   0.00027 $ & $   0.00088 $ & $  11.21090 $ & $ i$\\
$ 55657.92847 $ & $  -0.00101 $ & $   0.00088 $ & $  11.20830 $ & $ i$\\
$ 55657.92963 $ & $   0.00066 $ & $   0.00088 $ & $  11.20960 $ & $ i$\\
$ 55657.93085 $ & $  -0.00152 $ & $   0.00088 $ & $  11.20440 $ & $ i$\\
$ 55657.93208 $ & $   0.00163 $ & $   0.00088 $ & $  11.20810 $ & $ i$\\
$ 55657.93334 $ & $  -0.00026 $ & $   0.00090 $ & $  11.21150 $ & $ i$\\
$ 55657.93456 $ & $  -0.00051 $ & $   0.00092 $ & $  11.21240 $ & $ i$\\
$ 55657.93576 $ & $  -0.00086 $ & $   0.00093 $ & $  11.20080 $ & $ i$\\
$ 55657.93695 $ & $   0.00071 $ & $   0.00094 $ & $  11.20680 $ & $ i$\\
$ 55657.96229 $ & $   0.01327 $ & $   0.00087 $ & $  11.21820 $ & $ i$\\
$ 55657.96351 $ & $   0.01091 $ & $   0.00090 $ & $  11.21720 $ & $ i$\\
$ 55657.97850 $ & $   0.01311 $ & $   0.00088 $ & $  11.22200 $ & $ i$\\
$ 55657.99219 $ & $   0.01578 $ & $   0.00090 $ & $  11.22290 $ & $ i$\\
$ 55657.99338 $ & $   0.01380 $ & $   0.00087 $ & $  11.21800 $ & $ i$\\
$ 55657.99458 $ & $   0.01401 $ & $   0.00087 $ & $  11.22300 $ & $ i$\\
$ 55657.99577 $ & $   0.01609 $ & $   0.00087 $ & $  11.22250 $ & $ i$\\
$ 55657.99699 $ & $   0.01728 $ & $   0.00087 $ & $  11.22010 $ & $ i$\\
$ 55657.99819 $ & $   0.01632 $ & $   0.00087 $ & $  11.22080 $ & $ i$\\
$ 55657.99940 $ & $   0.01391 $ & $   0.00087 $ & $  11.21890 $ & $ i$\\
$ 55658.00061 $ & $   0.01498 $ & $   0.00087 $ & $  11.22050 $ & $ i$\\
$ 55658.00179 $ & $   0.01442 $ & $   0.00087 $ & $  11.21840 $ & $ i$\\
$ 55658.00300 $ & $   0.01375 $ & $   0.00088 $ & $  11.21670 $ & $ i$\\
$ 55682.92878 $ & $   0.00106 $ & $   0.00087 $ & $   9.98533 $ & $ i$\\
$ 55682.92938 $ & $  -0.00062 $ & $   0.00087 $ & $   9.98167 $ & $ i$\\
$ 55682.92990 $ & $  -0.00107 $ & $   0.00088 $ & $   9.98425 $ & $ i$\\
$ 55682.93047 $ & $   0.00092 $ & $   0.00088 $ & $   9.98013 $ & $ i$\\
$ 55682.93156 $ & $  -0.00146 $ & $   0.00089 $ & $   9.98281 $ & $ i$\\
$ 55682.93214 $ & $   0.00238 $ & $   0.00088 $ & $   9.98523 $ & $ i$\\
$ 55682.93270 $ & $  -0.00107 $ & $   0.00088 $ & $   9.97952 $ & $ i$\\
$ 55682.93327 $ & $  -0.00093 $ & $   0.00087 $ & $   9.98344 $ & $ i$\\
$ 55682.93381 $ & $  -0.00006 $ & $   0.00087 $ & $   9.98466 $ & $ i$\\
$ 55682.93437 $ & $   0.00341 $ & $   0.00087 $ & $   9.98528 $ & $ i$\\
$ 55682.93495 $ & $  -0.00250 $ & $   0.00087 $ & $   9.97903 $ & $ i$\\
$ 55682.93551 $ & $   0.00105 $ & $   0.00087 $ & $   9.98914 $ & $ i$\\
$ 55682.93609 $ & $  -0.00144 $ & $   0.00086 $ & $   9.98149 $ & $ i$\\
$ 55682.93661 $ & $  -0.00040 $ & $   0.00086 $ & $   9.98154 $ & $ i$\\
$ 55682.93717 $ & $  -0.00107 $ & $   0.00086 $ & $   9.98156 $ & $ i$\\
$ 55682.93774 $ & $  -0.00238 $ & $   0.00086 $ & $   9.97912 $ & $ i$\\
$ 55682.93826 $ & $  -0.00058 $ & $   0.00086 $ & $   9.98251 $ & $ i$\\
$ 55682.93884 $ & $  -0.00232 $ & $   0.00086 $ & $   9.98584 $ & $ i$\\
$ 55682.93941 $ & $  -0.00237 $ & $   0.00086 $ & $   9.98588 $ & $ i$\\
$ 55682.93994 $ & $   0.00208 $ & $   0.00086 $ & $   9.98847 $ & $ i$\\
$ 55682.94047 $ & $  -0.00166 $ & $   0.00086 $ & $   9.98410 $ & $ i$\\
$ 55682.94107 $ & $   0.00012 $ & $   0.00086 $ & $   9.98199 $ & $ i$\\
$ 55682.94163 $ & $  -0.00001 $ & $   0.00087 $ & $   9.98301 $ & $ i$\\
$ 55682.94221 $ & $  -0.00048 $ & $   0.00087 $ & $   9.98473 $ & $ i$\\
$ 55682.94278 $ & $  -0.00212 $ & $   0.00086 $ & $   9.97885 $ & $ i$\\
$ 55682.94332 $ & $   0.00086 $ & $   0.00086 $ & $   9.98406 $ & $ i$\\
$ 55682.94390 $ & $   0.00326 $ & $   0.00086 $ & $   9.98774 $ & $ i$\\
$ 55682.94442 $ & $  -0.00293 $ & $   0.00086 $ & $   9.98619 $ & $ i$\\
$ 55682.94557 $ & $   0.00079 $ & $   0.00088 $ & $   9.98085 $ & $ i$\\
$ 55682.94614 $ & $  -0.00320 $ & $   0.00087 $ & $   9.98092 $ & $ i$\\
$ 55682.94669 $ & $   0.00019 $ & $   0.00087 $ & $   9.98038 $ & $ i$\\
$ 55682.94725 $ & $   0.00098 $ & $   0.00088 $ & $   9.98626 $ & $ i$\\
$ 55682.94781 $ & $   0.00041 $ & $   0.00086 $ & $   9.98419 $ & $ i$\\
$ 55682.94837 $ & $  -0.00066 $ & $   0.00087 $ & $   9.98852 $ & $ i$\\
$ 55682.94890 $ & $   0.00111 $ & $   0.00086 $ & $   9.98869 $ & $ i$\\
$ 55682.94950 $ & $   0.00012 $ & $   0.00086 $ & $   9.98361 $ & $ i$\\
$ 55682.95007 $ & $   0.00328 $ & $   0.00086 $ & $   9.98729 $ & $ i$\\
$ 55682.95064 $ & $  -0.00005 $ & $   0.00085 $ & $   9.98406 $ & $ i$\\
$ 55682.95120 $ & $   0.00212 $ & $   0.00086 $ & $   9.98669 $ & $ i$\\
$ 55682.95173 $ & $   0.00007 $ & $   0.00086 $ & $   9.98178 $ & $ i$\\
$ 55682.95230 $ & $   0.00116 $ & $   0.00086 $ & $   9.98633 $ & $ i$\\
$ 55682.95287 $ & $   0.00243 $ & $   0.00085 $ & $   9.98473 $ & $ i$\\
$ 55682.95345 $ & $  -0.00005 $ & $   0.00085 $ & $   9.98725 $ & $ i$\\
$ 55682.95401 $ & $   0.00203 $ & $   0.00085 $ & $   9.98066 $ & $ i$\\
$ 55682.95454 $ & $   0.00300 $ & $   0.00085 $ & $   9.98799 $ & $ i$\\
$ 55682.95510 $ & $   0.00190 $ & $   0.00085 $ & $   9.98607 $ & $ i$\\
$ 55682.95566 $ & $   0.00427 $ & $   0.00085 $ & $   9.99083 $ & $ i$\\
$ 55682.95620 $ & $   0.00067 $ & $   0.00085 $ & $   9.98400 $ & $ i$\\
$ 55682.95734 $ & $  -0.00138 $ & $   0.00085 $ & $   9.98093 $ & $ i$\\
$ 55682.95794 $ & $   0.00210 $ & $   0.00085 $ & $   9.98262 $ & $ i$\\
$ 55682.95851 $ & $   0.00202 $ & $   0.00085 $ & $   9.98701 $ & $ i$\\
$ 55682.95907 $ & $  -0.00033 $ & $   0.00086 $ & $   9.98815 $ & $ i$\\
$ 55682.95962 $ & $  -0.00008 $ & $   0.00085 $ & $   9.98574 $ & $ i$\\
$ 55682.96421 $ & $   0.00154 $ & $   0.00086 $ & $   9.98738 $ & $ i$\\
$ 55682.96478 $ & $   0.00168 $ & $   0.00086 $ & $   9.98543 $ & $ i$\\
$ 55682.96534 $ & $  -0.00238 $ & $   0.00086 $ & $   9.98395 $ & $ i$\\
$ 55682.96587 $ & $  -0.00056 $ & $   0.00086 $ & $   9.98383 $ & $ i$\\
$ 55682.96644 $ & $  -0.00224 $ & $   0.00086 $ & $   9.97924 $ & $ i$\\
$ 55682.96698 $ & $  -0.00027 $ & $   0.00086 $ & $   9.98565 $ & $ i$\\
$ 55682.96754 $ & $  -0.00287 $ & $   0.00085 $ & $   9.98157 $ & $ i$\\
$ 55682.96809 $ & $   0.00045 $ & $   0.00085 $ & $   9.98404 $ & $ i$\\
$ 55682.96920 $ & $   0.00251 $ & $   0.00085 $ & $   9.99011 $ & $ i$\\
$ 55682.96980 $ & $  -0.00185 $ & $   0.00085 $ & $   9.98265 $ & $ i$\\
$ 55682.97033 $ & $  -0.00184 $ & $   0.00085 $ & $   9.98546 $ & $ i$\\
$ 55682.97093 $ & $  -0.00115 $ & $   0.00085 $ & $   9.98670 $ & $ i$\\
$ 55682.97149 $ & $  -0.00174 $ & $   0.00084 $ & $   9.98384 $ & $ i$\\
$ 55682.97316 $ & $  -0.00100 $ & $   0.00085 $ & $   9.98393 $ & $ i$\\
$ 55682.97376 $ & $   0.00137 $ & $   0.00086 $ & $   9.98421 $ & $ i$\\
$ 55682.97430 $ & $  -0.00261 $ & $   0.00085 $ & $   9.98549 $ & $ i$\\
$ 55682.97546 $ & $   0.00017 $ & $   0.00085 $ & $   9.98319 $ & $ i$\\
$ 55682.97598 $ & $   0.00190 $ & $   0.00085 $ & $   9.98608 $ & $ i$\\
$ 55682.97655 $ & $   0.00043 $ & $   0.00085 $ & $   9.98659 $ & $ i$\\
$ 55682.97709 $ & $  -0.00011 $ & $   0.00085 $ & $   9.98269 $ & $ i$\\
$ 55682.97766 $ & $   0.00035 $ & $   0.00085 $ & $   9.98646 $ & $ i$\\
$ 55682.97822 $ & $  -0.00070 $ & $   0.00085 $ & $   9.98613 $ & $ i$\\
$ 55682.97878 $ & $   0.00011 $ & $   0.00085 $ & $   9.98706 $ & $ i$\\
$ 55682.97930 $ & $   0.00137 $ & $   0.00085 $ & $   9.98631 $ & $ i$\\
$ 55682.97986 $ & $  -0.00115 $ & $   0.00085 $ & $   9.98419 $ & $ i$\\
$ 55682.98042 $ & $  -0.00018 $ & $   0.00085 $ & $   9.98493 $ & $ i$\\
$ 55682.98095 $ & $  -0.00125 $ & $   0.00085 $ & $   9.98343 $ & $ i$\\
$ 55682.98148 $ & $  -0.00209 $ & $   0.00085 $ & $   9.98252 $ & $ i$\\
$ 55682.98205 $ & $   0.00284 $ & $   0.00085 $ & $   9.98956 $ & $ i$\\
$ 55682.98261 $ & $   0.00055 $ & $   0.00085 $ & $   9.98660 $ & $ i$\\
$ 55682.98317 $ & $   0.00041 $ & $   0.00084 $ & $   9.98371 $ & $ i$\\
$ 55682.98430 $ & $   0.00078 $ & $   0.00087 $ & $   9.98347 $ & $ i$\\
$ 55682.98484 $ & $   0.00586 $ & $   0.00085 $ & $   9.99118 $ & $ i$\\
$ 55682.98540 $ & $   0.00092 $ & $   0.00085 $ & $   9.98441 $ & $ i$\\
$ 55682.98596 $ & $   0.00713 $ & $   0.00085 $ & $   9.99050 $ & $ i$\\
$ 55682.98650 $ & $   0.00208 $ & $   0.00085 $ & $   9.98558 $ & $ i$\\
$ 55682.98710 $ & $   0.00342 $ & $   0.00085 $ & $   9.99030 $ & $ i$\\
$ 55682.98767 $ & $   0.00487 $ & $   0.00085 $ & $   9.99062 $ & $ i$\\
$ 55682.98827 $ & $   0.00631 $ & $   0.00085 $ & $   9.99181 $ & $ i$\\
$ 55682.98881 $ & $   0.00664 $ & $   0.00084 $ & $   9.99217 $ & $ i$\\
$ 55682.98936 $ & $   0.00814 $ & $   0.00085 $ & $   9.99178 $ & $ i$\\
$ 55682.98990 $ & $   0.00840 $ & $   0.00085 $ & $   9.99291 $ & $ i$\\
$ 55682.99048 $ & $   0.00958 $ & $   0.00085 $ & $   9.99860 $ & $ i$\\
$ 55682.99103 $ & $   0.01176 $ & $   0.00085 $ & $   9.99825 $ & $ i$\\
$ 55682.99159 $ & $   0.01150 $ & $   0.00085 $ & $   9.99517 $ & $ i$\\
$ 55682.99215 $ & $   0.00564 $ & $   0.00084 $ & $   9.98888 $ & $ i$\\
$ 55682.99267 $ & $   0.01050 $ & $   0.00084 $ & $   9.99490 $ & $ i$\\
$ 55682.99326 $ & $   0.00929 $ & $   0.00085 $ & $   9.99700 $ & $ i$\\
$ 55682.99379 $ & $   0.01277 $ & $   0.00085 $ & $   9.99960 $ & $ i$\\
$ 55682.99432 $ & $   0.01477 $ & $   0.00085 $ & $   9.99763 $ & $ i$\\
$ 55682.99492 $ & $   0.01373 $ & $   0.00085 $ & $  10.00020 $ & $ i$\\
$ 55682.99548 $ & $   0.01087 $ & $   0.00085 $ & $   9.99925 $ & $ i$\\
$ 55682.99601 $ & $   0.01684 $ & $   0.00086 $ & $  10.00260 $ & $ i$\\
$ 55682.99654 $ & $   0.01191 $ & $   0.00085 $ & $   9.99595 $ & $ i$\\
$ 55682.99709 $ & $   0.01309 $ & $   0.00085 $ & $  10.00080 $ & $ i$\\
$ 55682.99767 $ & $   0.01117 $ & $   0.00085 $ & $   9.99645 $ & $ i$\\
$ 55682.99826 $ & $   0.01356 $ & $   0.00085 $ & $  10.00180 $ & $ i$\\
$ 55682.99879 $ & $   0.01188 $ & $   0.00084 $ & $   9.99679 $ & $ i$\\
$ 55682.99991 $ & $   0.00907 $ & $   0.00085 $ & $   9.99652 $ & $ i$\\
$ 55683.00044 $ & $   0.01243 $ & $   0.00085 $ & $  10.00020 $ & $ i$\\
$ 55683.00101 $ & $   0.01317 $ & $   0.00085 $ & $   9.99600 $ & $ i$\\
$ 55683.00160 $ & $   0.01424 $ & $   0.00085 $ & $   9.99966 $ & $ i$\\
$ 55683.00217 $ & $   0.01129 $ & $   0.00085 $ & $   9.99699 $ & $ i$\\
$ 55683.00274 $ & $   0.01271 $ & $   0.00085 $ & $   9.99419 $ & $ i$\\
$ 55683.00329 $ & $   0.01414 $ & $   0.00085 $ & $  10.00240 $ & $ i$\\
$ 55683.00382 $ & $   0.01350 $ & $   0.00085 $ & $  10.00060 $ & $ i$\\
$ 55683.00440 $ & $   0.01357 $ & $   0.00085 $ & $   9.99744 $ & $ i$\\
$ 55683.00497 $ & $   0.01262 $ & $   0.00085 $ & $   9.99655 $ & $ i$\\
$ 55683.00551 $ & $   0.01293 $ & $   0.00085 $ & $   9.99672 $ & $ i$\\
$ 55683.00607 $ & $   0.01379 $ & $   0.00085 $ & $  10.00050 $ & $ i$\\
$ 55683.00664 $ & $   0.01064 $ & $   0.00084 $ & $   9.99481 $ & $ i$\\
$ 55683.00716 $ & $   0.01046 $ & $   0.00085 $ & $   9.99279 $ & $ i$\\
$ 55683.00773 $ & $   0.01126 $ & $   0.00085 $ & $   9.99619 $ & $ i$\\
$ 55683.00830 $ & $   0.01560 $ & $   0.00085 $ & $  10.00000 $ & $ i$\\
$ 55683.00886 $ & $   0.01409 $ & $   0.00086 $ & $   9.99685 $ & $ i$\\
$ 55683.00942 $ & $   0.01637 $ & $   0.00085 $ & $  10.00090 $ & $ i$\\
$ 55683.00995 $ & $   0.01590 $ & $   0.00086 $ & $   9.99896 $ & $ i$\\
$ 55683.01052 $ & $   0.01479 $ & $   0.00085 $ & $  10.00020 $ & $ i$\\
$ 55683.01110 $ & $   0.01655 $ & $   0.00085 $ & $  10.00200 $ & $ i$\\
$ 55683.01224 $ & $   0.01306 $ & $   0.00085 $ & $   9.99886 $ & $ i$\\
$ 55683.01276 $ & $   0.01348 $ & $   0.00085 $ & $  10.00550 $ & $ i$\\
$ 55683.01332 $ & $   0.01391 $ & $   0.00085 $ & $  10.00180 $ & $ i$\\
$ 55683.01390 $ & $   0.01231 $ & $   0.00085 $ & $   9.99790 $ & $ i$\\
$ 55683.01447 $ & $   0.01312 $ & $   0.00085 $ & $   9.99753 $ & $ i$\\
$ 55683.01504 $ & $   0.01808 $ & $   0.00086 $ & $  10.00260 $ & $ i$\\
$ 55683.01561 $ & $   0.01583 $ & $   0.00086 $ & $  10.00030 $ & $ i$\\
$ 55683.01617 $ & $   0.01391 $ & $   0.00085 $ & $  10.00020 $ & $ i$\\
$ 55683.01669 $ & $   0.01374 $ & $   0.00085 $ & $   9.99978 $ & $ i$\\
$ 55683.01726 $ & $   0.01422 $ & $   0.00085 $ & $   9.99887 $ & $ i$\\
$ 55683.01784 $ & $   0.01407 $ & $   0.00084 $ & $   9.99795 $ & $ i$\\
$ 55683.01837 $ & $   0.01332 $ & $   0.00085 $ & $   9.99924 $ & $ i$\\
$ 55683.01893 $ & $   0.01421 $ & $   0.00085 $ & $   9.99799 $ & $ i$\\
$ 55683.01950 $ & $   0.01578 $ & $   0.00085 $ & $  10.00110 $ & $ i$\\
$ 55683.02060 $ & $   0.01768 $ & $   0.00085 $ & $  10.00460 $ & $ i$\\
$ 55683.02116 $ & $   0.01455 $ & $   0.00085 $ & $   9.99849 $ & $ i$\\
$ 55683.02178 $ & $   0.01252 $ & $   0.00085 $ & $   9.99969 $ & $ i$\\
$ 55683.02231 $ & $   0.01733 $ & $   0.00084 $ & $   9.99903 $ & $ i$\\
$ 55683.02287 $ & $   0.01370 $ & $   0.00084 $ & $   9.99837 $ & $ i$\\
$ 55683.02339 $ & $   0.01375 $ & $   0.00085 $ & $   9.99825 $ & $ i$\\
$ 55683.02395 $ & $   0.01574 $ & $   0.00085 $ & $   9.99704 $ & $ i$\\
$ 55683.02455 $ & $   0.01870 $ & $   0.00084 $ & $  10.00290 $ & $ i$\\
$ 55683.02509 $ & $   0.01409 $ & $   0.00085 $ & $   9.99941 $ & $ i$\\
$ 55683.02565 $ & $   0.01758 $ & $   0.00085 $ & $  10.00860 $ & $ i$\\
$ 55683.02620 $ & $   0.01200 $ & $   0.00085 $ & $   9.99787 $ & $ i$\\
$ 55683.02677 $ & $   0.01428 $ & $   0.00085 $ & $   9.99928 $ & $ i$\\
$ 55683.02731 $ & $   0.01571 $ & $   0.00085 $ & $  10.00220 $ & $ i$\\
$ 55683.02792 $ & $   0.01461 $ & $   0.00085 $ & $  10.00030 $ & $ i$\\
$ 55683.02849 $ & $   0.01387 $ & $   0.00085 $ & $   9.99750 $ & $ i$\\
$ 55683.02901 $ & $   0.01595 $ & $   0.00084 $ & $  10.00170 $ & $ i$\\
$ 55683.03015 $ & $   0.01536 $ & $   0.00084 $ & $  10.00120 $ & $ i$\\
$ 55683.03072 $ & $   0.01486 $ & $   0.00084 $ & $  10.00220 $ & $ i$\\
$ 55683.03126 $ & $   0.01413 $ & $   0.00084 $ & $   9.99665 $ & $ i$\\
$ 55683.03182 $ & $   0.01471 $ & $   0.00084 $ & $   9.99968 $ & $ i$\\
$ 55683.03234 $ & $   0.01670 $ & $   0.00084 $ & $  10.00310 $ & $ i$\\
$ 55683.03291 $ & $   0.01515 $ & $   0.00084 $ & $  10.00190 $ & $ i$\\
$ 55683.03345 $ & $   0.01465 $ & $   0.00084 $ & $  10.00060 $ & $ i$\\
$ 55683.03399 $ & $   0.01586 $ & $   0.00084 $ & $   9.99808 $ & $ i$\\
$ 55683.03456 $ & $   0.01326 $ & $   0.00084 $ & $   9.99678 $ & $ i$\\
$ 55683.03510 $ & $   0.01547 $ & $   0.00084 $ & $  10.00280 $ & $ i$\\
$ 55683.03566 $ & $   0.01505 $ & $   0.00084 $ & $   9.99877 $ & $ i$\\
$ 55683.03620 $ & $   0.01565 $ & $   0.00085 $ & $  10.00480 $ & $ i$\\
$ 55683.03676 $ & $   0.01381 $ & $   0.00084 $ & $   9.99742 $ & $ i$\\
$ 55683.03730 $ & $   0.01510 $ & $   0.00084 $ & $  10.00340 $ & $ i$\\
$ 55683.03787 $ & $   0.01679 $ & $   0.00084 $ & $  10.00380 $ & $ i$\\
$ 55683.03843 $ & $   0.01811 $ & $   0.00084 $ & $  10.00490 $ & $ i$\\
$ 55683.03896 $ & $   0.01751 $ & $   0.00085 $ & $  10.00420 $ & $ i$\\
$ 55683.03952 $ & $   0.01430 $ & $   0.00084 $ & $   9.99967 $ & $ i$\\
$ 55683.04009 $ & $   0.01390 $ & $   0.00084 $ & $   9.99842 $ & $ i$\\
$ 55683.04061 $ & $   0.01521 $ & $   0.00085 $ & $  10.00550 $ & $ i$\\
$ 55683.04117 $ & $   0.01711 $ & $   0.00084 $ & $  10.00650 $ & $ i$\\
$ 55683.04170 $ & $   0.01587 $ & $   0.00086 $ & $  10.00060 $ & $ i$\\
$ 55683.04228 $ & $   0.01258 $ & $   0.00084 $ & $   9.99972 $ & $ i$\\
$ 55683.04284 $ & $   0.01670 $ & $   0.00085 $ & $  10.00390 $ & $ i$\\
$ 55683.04337 $ & $   0.01550 $ & $   0.00085 $ & $  10.00340 $ & $ i$\\
$ 55683.04394 $ & $   0.01417 $ & $   0.00084 $ & $   9.99966 $ & $ i$\\
$ 55683.04447 $ & $   0.01603 $ & $   0.00087 $ & $  10.00600 $ & $ i$\\
$ 55683.04503 $ & $   0.01629 $ & $   0.00085 $ & $  10.00430 $ & $ i$\\
$ 55683.04556 $ & $   0.01371 $ & $   0.00086 $ & $   9.99847 $ & $ i$\\
$ 55683.04613 $ & $   0.01405 $ & $   0.00084 $ & $   9.99834 $ & $ i$\\
$ 55683.04665 $ & $   0.01329 $ & $   0.00085 $ & $  10.00100 $ & $ i$\\
$ 55683.04721 $ & $   0.01384 $ & $   0.00084 $ & $   9.99858 $ & $ i$\\
$ 55683.04778 $ & $   0.01749 $ & $   0.00086 $ & $  10.01110 $ & $ i$\\
$ 55683.04832 $ & $   0.01315 $ & $   0.00085 $ & $   9.99672 $ & $ i$\\
$ 55683.04887 $ & $   0.01487 $ & $   0.00085 $ & $  10.00220 $ & $ i$\\
$ 55704.83372 $ & $  -0.00107 $ & $   0.00120 $ & $  11.86235 $ & $ i$\\
$ 55704.83446 $ & $  -0.00082 $ & $   0.00121 $ & $  11.86698 $ & $ i$\\
$ 55704.83534 $ & $   0.00244 $ & $   0.00120 $ & $  11.87092 $ & $ i$\\
$ 55704.83607 $ & $   0.00201 $ & $   0.00120 $ & $  11.86747 $ & $ i$\\
$ 55704.83693 $ & $  -0.00224 $ & $   0.00119 $ & $  11.86431 $ & $ i$\\
$ 55704.83767 $ & $  -0.00218 $ & $   0.00120 $ & $  11.86664 $ & $ i$\\
$ 55704.83859 $ & $  -0.00075 $ & $   0.00119 $ & $  11.86524 $ & $ i$\\
$ 55704.83931 $ & $  -0.00323 $ & $   0.00121 $ & $  11.86325 $ & $ i$\\
$ 55704.84020 $ & $  -0.00236 $ & $   0.00119 $ & $  11.86283 $ & $ i$\\
$ 55704.84093 $ & $   0.00073 $ & $   0.00120 $ & $  11.86811 $ & $ i$\\
$ 55704.84188 $ & $   0.00176 $ & $   0.00120 $ & $  11.86747 $ & $ i$\\
$ 55704.84259 $ & $   0.00060 $ & $   0.00121 $ & $  11.86547 $ & $ i$\\
$ 55704.84352 $ & $  -0.00204 $ & $   0.00120 $ & $  11.86412 $ & $ i$\\
$ 55704.84425 $ & $   0.00269 $ & $   0.00119 $ & $  11.86779 $ & $ i$\\
$ 55704.84515 $ & $  -0.00126 $ & $   0.00120 $ & $  11.86559 $ & $ i$\\
$ 55704.84589 $ & $   0.00040 $ & $   0.00120 $ & $  11.86796 $ & $ i$\\
$ 55704.84682 $ & $  -0.00406 $ & $   0.00120 $ & $  11.86312 $ & $ i$\\
$ 55704.84755 $ & $   0.00248 $ & $   0.00121 $ & $  11.87054 $ & $ i$\\
$ 55704.84845 $ & $  -0.00065 $ & $   0.00119 $ & $  11.86642 $ & $ i$\\
$ 55704.84919 $ & $  -0.00083 $ & $   0.00120 $ & $  11.86656 $ & $ i$\\
$ 55704.85011 $ & $  -0.00170 $ & $   0.00120 $ & $  11.86581 $ & $ i$\\
$ 55704.85082 $ & $  -0.00146 $ & $   0.00121 $ & $  11.86617 $ & $ i$\\
$ 55704.85173 $ & $   0.00316 $ & $   0.00120 $ & $  11.87136 $ & $ i$\\
$ 55704.85245 $ & $   0.00163 $ & $   0.00120 $ & $  11.86604 $ & $ i$\\
$ 55704.85335 $ & $  -0.00108 $ & $   0.00119 $ & $  11.86440 $ & $ i$\\
$ 55704.85409 $ & $  -0.00081 $ & $   0.00120 $ & $  11.86691 $ & $ i$\\
$ 55704.85497 $ & $   0.00028 $ & $   0.00120 $ & $  11.86609 $ & $ i$\\
$ 55704.85568 $ & $   0.00259 $ & $   0.00120 $ & $  11.86814 $ & $ i$\\
$ 55704.85659 $ & $   0.00239 $ & $   0.00121 $ & $  11.86643 $ & $ i$\\
$ 55704.85731 $ & $  -0.00097 $ & $   0.00120 $ & $  11.86762 $ & $ i$\\
$ 55704.85823 $ & $   0.00337 $ & $   0.00120 $ & $  11.87014 $ & $ i$\\
$ 55704.85897 $ & $  -0.00161 $ & $   0.00120 $ & $  11.86498 $ & $ i$\\
$ 55704.85987 $ & $  -0.00257 $ & $   0.00120 $ & $  11.86494 $ & $ i$\\
$ 55704.86059 $ & $   0.00178 $ & $   0.00120 $ & $  11.86755 $ & $ i$\\
$ 55704.86150 $ & $   0.00142 $ & $   0.00120 $ & $  11.86949 $ & $ i$\\
$ 55704.86226 $ & $  -0.00257 $ & $   0.00119 $ & $  11.86368 $ & $ i$\\
$ 55704.86316 $ & $   0.00134 $ & $   0.00120 $ & $  11.87043 $ & $ i$\\
$ 55704.86390 $ & $  -0.00071 $ & $   0.00120 $ & $  11.86376 $ & $ i$\\
$ 55704.86481 $ & $   0.00104 $ & $   0.00119 $ & $  11.86744 $ & $ i$\\
$ 55704.86553 $ & $  -0.00061 $ & $   0.00119 $ & $  11.86521 $ & $ i$\\
$ 55704.86647 $ & $   0.00142 $ & $   0.00119 $ & $  11.86774 $ & $ i$\\
$ 55704.86721 $ & $   0.00106 $ & $   0.00120 $ & $  11.86806 $ & $ i$\\
$ 55704.86813 $ & $  -0.00129 $ & $   0.00119 $ & $  11.86583 $ & $ i$\\
$ 55704.86884 $ & $  -0.00033 $ & $   0.00120 $ & $  11.86416 $ & $ i$\\
$ 55704.86975 $ & $  -0.00086 $ & $   0.00120 $ & $  11.86374 $ & $ i$\\
$ 55704.87047 $ & $   0.00145 $ & $   0.00119 $ & $  11.86681 $ & $ i$\\
$ 55704.87138 $ & $  -0.00056 $ & $   0.00119 $ & $  11.86524 $ & $ i$\\
$ 55704.87212 $ & $   0.00451 $ & $   0.00120 $ & $  11.86967 $ & $ i$\\
$ 55704.87304 $ & $   0.00128 $ & $   0.00119 $ & $  11.86902 $ & $ i$\\
$ 55704.87375 $ & $   0.00152 $ & $   0.00120 $ & $  11.86902 $ & $ i$\\
$ 55704.87468 $ & $   0.00184 $ & $   0.00121 $ & $  11.86848 $ & $ i$\\
$ 55704.87541 $ & $   0.00138 $ & $   0.00121 $ & $  11.86759 $ & $ i$\\
$ 55704.87630 $ & $  -0.00082 $ & $   0.00120 $ & $  11.86549 $ & $ i$\\
$ 55704.87704 $ & $  -0.00108 $ & $   0.00120 $ & $  11.86231 $ & $ i$\\
$ 55704.87794 $ & $  -0.00285 $ & $   0.00120 $ & $  11.86581 $ & $ i$\\
$ 55704.87867 $ & $  -0.00045 $ & $   0.00120 $ & $  11.86524 $ & $ i$\\
$ 55704.87956 $ & $  -0.00114 $ & $   0.00119 $ & $  11.86556 $ & $ i$\\
$ 55704.88029 $ & $  -0.00111 $ & $   0.00120 $ & $  11.86485 $ & $ i$\\
$ 55704.88116 $ & $  -0.00161 $ & $   0.00119 $ & $  11.86413 $ & $ i$\\
$ 55704.88190 $ & $   0.00097 $ & $   0.00121 $ & $  11.86713 $ & $ i$\\
$ 55704.88283 $ & $   0.00119 $ & $   0.00119 $ & $  11.86570 $ & $ i$\\
$ 55704.88357 $ & $  -0.00086 $ & $   0.00120 $ & $  11.86704 $ & $ i$\\
$ 55704.88445 $ & $  -0.00064 $ & $   0.00120 $ & $  11.86714 $ & $ i$\\
$ 55704.88519 $ & $   0.00565 $ & $   0.00120 $ & $  11.87254 $ & $ i$\\
$ 55704.88609 $ & $   0.00462 $ & $   0.00119 $ & $  11.86885 $ & $ i$\\
$ 55704.88683 $ & $   0.00312 $ & $   0.00120 $ & $  11.86904 $ & $ i$\\
$ 55704.88773 $ & $   0.00159 $ & $   0.00120 $ & $  11.86644 $ & $ i$\\
$ 55704.88846 $ & $   0.00254 $ & $   0.00120 $ & $  11.87003 $ & $ i$\\
$ 55704.88935 $ & $   0.00546 $ & $   0.00119 $ & $  11.86831 $ & $ i$\\
$ 55704.89008 $ & $   0.00325 $ & $   0.00119 $ & $  11.86739 $ & $ i$\\
$ 55704.89101 $ & $   0.00661 $ & $   0.00119 $ & $  11.87058 $ & $ i$\\
$ 55704.89175 $ & $   0.00556 $ & $   0.00119 $ & $  11.86899 $ & $ i$\\
$ 55704.89268 $ & $   0.00871 $ & $   0.00120 $ & $  11.87075 $ & $ i$\\
$ 55704.89341 $ & $   0.00999 $ & $   0.00120 $ & $  11.87437 $ & $ i$\\
$ 55704.89426 $ & $   0.01023 $ & $   0.00121 $ & $  11.87579 $ & $ i$\\
$ 55704.89500 $ & $   0.00699 $ & $   0.00121 $ & $  11.87203 $ & $ i$\\
$ 55704.89592 $ & $   0.01120 $ & $   0.00120 $ & $  11.87543 $ & $ i$\\
$ 55704.89665 $ & $   0.01096 $ & $   0.00120 $ & $  11.87284 $ & $ i$\\
$ 55704.89756 $ & $   0.01118 $ & $   0.00120 $ & $  11.87260 $ & $ i$\\
$ 55704.89830 $ & $   0.01449 $ & $   0.00121 $ & $  11.87705 $ & $ i$\\
$ 55704.89923 $ & $   0.01242 $ & $   0.00121 $ & $  11.87676 $ & $ i$\\
$ 55704.89996 $ & $   0.01181 $ & $   0.00121 $ & $  11.87666 $ & $ i$\\
$ 55704.90085 $ & $   0.01005 $ & $   0.00121 $ & $  11.87687 $ & $ i$\\
$ 55704.90158 $ & $   0.00874 $ & $   0.00120 $ & $  11.87084 $ & $ i$\\
$ 55704.90247 $ & $   0.01355 $ & $   0.00120 $ & $  11.87652 $ & $ i$\\
$ 55704.90321 $ & $   0.01824 $ & $   0.00121 $ & $  11.88083 $ & $ i$\\
$ 55704.90411 $ & $   0.01366 $ & $   0.00120 $ & $  11.87766 $ & $ i$\\
$ 55704.90485 $ & $   0.01599 $ & $   0.00121 $ & $  11.88233 $ & $ i$\\
$ 55704.90574 $ & $   0.01373 $ & $   0.00121 $ & $  11.87941 $ & $ i$\\
$ 55704.90649 $ & $   0.01825 $ & $   0.00121 $ & $  11.88163 $ & $ i$\\
$ 55704.90741 $ & $   0.01874 $ & $   0.00120 $ & $  11.88316 $ & $ i$\\
$ 55704.90814 $ & $   0.01185 $ & $   0.00120 $ & $  11.87473 $ & $ i$\\
$ 55704.90906 $ & $   0.01237 $ & $   0.00121 $ & $  11.87618 $ & $ i$\\
$ 55704.90978 $ & $   0.01069 $ & $   0.00121 $ & $  11.87224 $ & $ i$\\
$ 55704.91070 $ & $   0.01729 $ & $   0.00121 $ & $  11.88123 $ & $ i$\\
$ 55704.91144 $ & $   0.01159 $ & $   0.00120 $ & $  11.87463 $ & $ i$\\
$ 55704.91234 $ & $   0.01470 $ & $   0.00121 $ & $  11.87872 $ & $ i$\\
$ 55704.91311 $ & $   0.01283 $ & $   0.00121 $ & $  11.87598 $ & $ i$\\
$ 55704.91401 $ & $   0.01627 $ & $   0.00120 $ & $  11.87992 $ & $ i$\\
$ 55704.91474 $ & $   0.01482 $ & $   0.00121 $ & $  11.87662 $ & $ i$\\
$ 55704.91566 $ & $   0.01337 $ & $   0.00120 $ & $  11.87676 $ & $ i$\\
$ 55704.91641 $ & $   0.01267 $ & $   0.00121 $ & $  11.87609 $ & $ i$\\
$ 55704.91727 $ & $   0.01136 $ & $   0.00121 $ & $  11.87530 $ & $ i$\\
$ 55704.91801 $ & $   0.01320 $ & $   0.00120 $ & $  11.87705 $ & $ i$\\
$ 55704.91893 $ & $   0.01057 $ & $   0.00120 $ & $  11.87387 $ & $ i$\\
$ 55704.91965 $ & $   0.01218 $ & $   0.00121 $ & $  11.87640 $ & $ i$\\
$ 55704.92055 $ & $   0.01486 $ & $   0.00121 $ & $  11.87844 $ & $ i$\\
$ 55704.92128 $ & $   0.01120 $ & $   0.00120 $ & $  11.87407 $ & $ i$\\
$ 55704.92219 $ & $   0.01174 $ & $   0.00120 $ & $  11.87605 $ & $ i$\\
$ 55704.92293 $ & $   0.01751 $ & $   0.00122 $ & $  11.88208 $ & $ i$\\
$ 55704.92384 $ & $   0.01340 $ & $   0.00121 $ & $  11.87880 $ & $ i$\\
$ 55704.92458 $ & $   0.01956 $ & $   0.00121 $ & $  11.88205 $ & $ i$\\
$ 55704.92548 $ & $   0.01935 $ & $   0.00121 $ & $  11.88202 $ & $ i$\\
$ 55704.92621 $ & $   0.01587 $ & $   0.00121 $ & $  11.88146 $ & $ i$\\
$ 55704.92712 $ & $   0.01599 $ & $   0.00120 $ & $  11.88147 $ & $ i$\\
$ 55704.92786 $ & $   0.01470 $ & $   0.00120 $ & $  11.87852 $ & $ i$\\
$ 55704.92877 $ & $   0.01628 $ & $   0.00122 $ & $  11.87783 $ & $ i$\\
$ 55704.92951 $ & $   0.01967 $ & $   0.00121 $ & $  11.88324 $ & $ i$\\
$ 55704.93041 $ & $   0.01328 $ & $   0.00121 $ & $  11.87344 $ & $ i$\\
$ 55704.93115 $ & $   0.01384 $ & $   0.00121 $ & $  11.87607 $ & $ i$\\
$ 55704.93208 $ & $   0.01184 $ & $   0.00121 $ & $  11.87427 $ & $ i$\\
$ 55704.93282 $ & $   0.01454 $ & $   0.00121 $ & $  11.87745 $ & $ i$\\
$ 55704.93372 $ & $   0.01634 $ & $   0.00120 $ & $  11.88026 $ & $ i$\\
$ 55704.93445 $ & $   0.01488 $ & $   0.00120 $ & $  11.87899 $ & $ i$\\
$ 55704.93535 $ & $   0.01688 $ & $   0.00121 $ & $  11.88131 $ & $ i$\\
$ 55704.93608 $ & $   0.01440 $ & $   0.00121 $ & $  11.87804 $ & $ i$\\
$ 55704.93700 $ & $   0.01326 $ & $   0.00120 $ & $  11.87501 $ & $ i$\\
$ 55704.93773 $ & $   0.01173 $ & $   0.00121 $ & $  11.87490 $ & $ i$\\
$ 55704.93864 $ & $   0.01541 $ & $   0.00121 $ & $  11.87809 $ & $ i$\\
$ 55704.93938 $ & $   0.01143 $ & $   0.00121 $ & $  11.87631 $ & $ i$\\
$ 55704.94031 $ & $   0.01085 $ & $   0.00120 $ & $  11.87370 $ & $ i$\\
$ 55704.94105 $ & $   0.01300 $ & $   0.00121 $ & $  11.87595 $ & $ i$\\
$ 55704.94193 $ & $   0.01281 $ & $   0.00121 $ & $  11.87644 $ & $ i$\\
$ 55704.94266 $ & $   0.01299 $ & $   0.00120 $ & $  11.87750 $ & $ i$\\
$ 55704.94357 $ & $   0.01281 $ & $   0.00121 $ & $  11.87564 $ & $ i$\\
$ 55704.94431 $ & $   0.01702 $ & $   0.00121 $ & $  11.88182 $ & $ i$\\
$ 55704.94521 $ & $   0.01477 $ & $   0.00121 $ & $  11.87830 $ & $ i$\\
$ 55704.94596 $ & $   0.01275 $ & $   0.00121 $ & $  11.87680 $ & $ i$\\
$ 55704.94686 $ & $   0.01777 $ & $   0.00121 $ & $  11.88120 $ & $ i$\\
$ 55704.94759 $ & $   0.01479 $ & $   0.00121 $ & $  11.87897 $ & $ i$\\
$ 55704.94854 $ & $   0.01937 $ & $   0.00121 $ & $  11.88178 $ & $ i$\\
$ 55704.94925 $ & $   0.01614 $ & $   0.00121 $ & $  11.87979 $ & $ i$\\
$ 55704.95016 $ & $   0.01579 $ & $   0.00121 $ & $  11.87968 $ & $ i$\\
$ 55704.95089 $ & $   0.01309 $ & $   0.00120 $ & $  11.87580 $ & $ i$\\
$ 55704.95180 $ & $   0.01344 $ & $   0.00120 $ & $  11.87511 $ & $ i$\\
$ 55704.95254 $ & $   0.01222 $ & $   0.00120 $ & $  11.87584 $ & $ i$\\
$ 55704.95342 $ & $   0.01423 $ & $   0.00120 $ & $  11.88077 $ & $ i$\\
$ 55704.95415 $ & $   0.01347 $ & $   0.00120 $ & $  11.87918 $ & $ i$\\
$ 55704.95506 $ & $   0.01413 $ & $   0.00120 $ & $  11.87504 $ & $ i$\\
$ 55704.95579 $ & $   0.01457 $ & $   0.00121 $ & $  11.87867 $ & $ i$\\
$ 55704.95671 $ & $   0.01592 $ & $   0.00121 $ & $  11.88129 $ & $ i$\\
$ 55704.95745 $ & $   0.01566 $ & $   0.00121 $ & $  11.87902 $ & $ i$\\
$ 55704.95835 $ & $   0.01591 $ & $   0.00120 $ & $  11.87869 $ & $ i$\\
$ 55704.95908 $ & $   0.01440 $ & $   0.00120 $ & $  11.87945 $ & $ i$\\
$ 55704.96000 $ & $   0.01601 $ & $   0.00120 $ & $  11.88016 $ & $ i$\\
$ 55704.96074 $ & $   0.02032 $ & $   0.00121 $ & $  11.88369 $ & $ i$\\
$ 55704.96164 $ & $   0.01653 $ & $   0.00121 $ & $  11.88037 $ & $ i$\\
$ 55704.96237 $ & $   0.01397 $ & $   0.00120 $ & $  11.87978 $ & $ i$\\
$ 55704.96327 $ & $   0.01616 $ & $   0.00121 $ & $  11.88073 $ & $ i$\\
$ 55704.96400 $ & $   0.01322 $ & $   0.00120 $ & $  11.87979 $ & $ i$\\
$ 55704.96494 $ & $   0.01910 $ & $   0.00121 $ & $  11.88213 $ & $ i$\\
$ 55704.96568 $ & $   0.01552 $ & $   0.00121 $ & $  11.88020 $ & $ i$\\
$ 55704.96658 $ & $   0.01923 $ & $   0.00122 $ & $  11.88386 $ & $ i$\\
$ 55704.96732 $ & $   0.01478 $ & $   0.00121 $ & $  11.87787 $ & $ i$\\
$ 55704.96822 $ & $   0.01707 $ & $   0.00121 $ & $  11.88048 $ & $ i$\\
$ 55704.96897 $ & $   0.01272 $ & $   0.00120 $ & $  11.87535 $ & $ i$\\
$ 55704.96987 $ & $   0.01543 $ & $   0.00121 $ & $  11.88023 $ & $ i$\\
$ 55704.97060 $ & $   0.01290 $ & $   0.00121 $ & $  11.87764 $ & $ i$\\
$ 55704.97151 $ & $   0.01364 $ & $   0.00120 $ & $  11.87941 $ & $ i$\\
$ 55704.97224 $ & $   0.01437 $ & $   0.00122 $ & $  11.87772 $ & $ i$\\
$ 55704.97319 $ & $   0.01510 $ & $   0.00122 $ & $  11.88109 $ & $ i$\\
$ 55704.97392 $ & $   0.01803 $ & $   0.00123 $ & $  11.88233 $ & $ i$\\
$ 55704.97483 $ & $   0.01822 $ & $   0.00121 $ & $  11.88231 $ & $ i$\\
$ 55704.97556 $ & $   0.01329 $ & $   0.00122 $ & $  11.88142 $ & $ i$\\
$ 55723.71630 $ & $   0.01731 $ & $   0.00108 $ & $  11.88388 $ & $ i$\\
$ 55723.71703 $ & $   0.01506 $ & $   0.00107 $ & $  11.88095 $ & $ i$\\
$ 55723.71795 $ & $   0.01500 $ & $   0.00108 $ & $  11.88050 $ & $ i$\\
$ 55723.71960 $ & $   0.01732 $ & $   0.00108 $ & $  11.88106 $ & $ i$\\
$ 55723.72033 $ & $   0.01482 $ & $   0.00107 $ & $  11.87821 $ & $ i$\\
$ 55723.72124 $ & $   0.01504 $ & $   0.00107 $ & $  11.87838 $ & $ i$\\
$ 55723.72197 $ & $   0.01378 $ & $   0.00107 $ & $  11.87686 $ & $ i$\\
$ 55723.72289 $ & $   0.01766 $ & $   0.00108 $ & $  11.88163 $ & $ i$\\
$ 55723.72363 $ & $   0.01665 $ & $   0.00108 $ & $  11.88218 $ & $ i$\\
$ 55723.72455 $ & $   0.01421 $ & $   0.00107 $ & $  11.87987 $ & $ i$\\
$ 55723.72528 $ & $   0.01199 $ & $   0.00107 $ & $  11.87762 $ & $ i$\\
$ 55723.72618 $ & $   0.01426 $ & $   0.00107 $ & $  11.87850 $ & $ i$\\
$ 55723.72690 $ & $   0.01591 $ & $   0.00107 $ & $  11.88074 $ & $ i$\\
$ 55723.72780 $ & $   0.01370 $ & $   0.00107 $ & $  11.87829 $ & $ i$\\
$ 55723.72854 $ & $   0.01484 $ & $   0.00108 $ & $  11.88028 $ & $ i$\\
$ 55723.72944 $ & $   0.01263 $ & $   0.00107 $ & $  11.87718 $ & $ i$\\
$ 55723.73017 $ & $   0.01868 $ & $   0.00107 $ & $  11.88403 $ & $ i$\\
$ 55723.73108 $ & $   0.01646 $ & $   0.00107 $ & $  11.88187 $ & $ i$\\
$ 55723.73181 $ & $   0.01201 $ & $   0.00107 $ & $  11.87489 $ & $ i$\\
$ 55723.73273 $ & $   0.01689 $ & $   0.00108 $ & $  11.87882 $ & $ i$\\
$ 55723.73346 $ & $   0.01329 $ & $   0.00108 $ & $  11.87813 $ & $ i$\\
$ 55723.73435 $ & $   0.01368 $ & $   0.00108 $ & $  11.87965 $ & $ i$\\
$ 55723.73508 $ & $   0.01397 $ & $   0.00107 $ & $  11.87828 $ & $ i$\\
$ 55723.73597 $ & $   0.01388 $ & $   0.00108 $ & $  11.87940 $ & $ i$\\
$ 55723.73671 $ & $   0.01106 $ & $   0.00108 $ & $  11.87912 $ & $ i$\\
$ 55723.73761 $ & $   0.01548 $ & $   0.00108 $ & $  11.88060 $ & $ i$\\
$ 55723.73835 $ & $   0.01432 $ & $   0.00107 $ & $  11.87898 $ & $ i$\\
$ 55723.73927 $ & $   0.01775 $ & $   0.00108 $ & $  11.88211 $ & $ i$\\
$ 55723.74001 $ & $   0.01787 $ & $   0.00107 $ & $  11.88185 $ & $ i$\\
$ 55723.74093 $ & $   0.01455 $ & $   0.00108 $ & $  11.87859 $ & $ i$\\
$ 55723.74166 $ & $   0.01773 $ & $   0.00107 $ & $  11.88243 $ & $ i$\\
$ 55723.74255 $ & $   0.01184 $ & $   0.00107 $ & $  11.87669 $ & $ i$\\
$ 55723.74329 $ & $   0.01599 $ & $   0.00107 $ & $  11.87988 $ & $ i$\\
$ 55723.74420 $ & $   0.01375 $ & $   0.00107 $ & $  11.87641 $ & $ i$\\
$ 55723.74494 $ & $   0.01420 $ & $   0.00108 $ & $  11.88023 $ & $ i$\\
$ 55723.74582 $ & $   0.01380 $ & $   0.00107 $ & $  11.87757 $ & $ i$\\
$ 55723.74655 $ & $   0.01651 $ & $   0.00108 $ & $  11.88162 $ & $ i$\\
$ 55723.74744 $ & $   0.01823 $ & $   0.00108 $ & $  11.88267 $ & $ i$\\
$ 55723.74818 $ & $   0.01194 $ & $   0.00107 $ & $  11.87432 $ & $ i$\\
$ 55723.74910 $ & $   0.01692 $ & $   0.00108 $ & $  11.88007 $ & $ i$\\
$ 55723.74983 $ & $   0.01473 $ & $   0.00107 $ & $  11.87985 $ & $ i$\\
$ 55723.75075 $ & $   0.01307 $ & $   0.00107 $ & $  11.87670 $ & $ i$\\
$ 55723.75148 $ & $   0.01456 $ & $   0.00107 $ & $  11.87870 $ & $ i$\\
$ 55723.75239 $ & $   0.01477 $ & $   0.00108 $ & $  11.87885 $ & $ i$\\
$ 55723.75313 $ & $   0.01704 $ & $   0.00107 $ & $  11.88286 $ & $ i$\\
$ 55723.75405 $ & $   0.01569 $ & $   0.00108 $ & $  11.88053 $ & $ i$\\
$ 55723.75478 $ & $   0.01492 $ & $   0.00108 $ & $  11.88200 $ & $ i$\\
$ 55723.75567 $ & $   0.01301 $ & $   0.00107 $ & $  11.87674 $ & $ i$\\
$ 55723.75641 $ & $   0.01860 $ & $   0.00108 $ & $  11.88472 $ & $ i$\\
$ 55723.75733 $ & $   0.01412 $ & $   0.00108 $ & $  11.87865 $ & $ i$\\
$ 55723.75807 $ & $   0.01958 $ & $   0.00108 $ & $  11.88273 $ & $ i$\\
$ 55723.75898 $ & $   0.01439 $ & $   0.00107 $ & $  11.87824 $ & $ i$\\
$ 55723.75971 $ & $   0.01596 $ & $   0.00108 $ & $  11.88205 $ & $ i$\\
$ 55723.76062 $ & $   0.01498 $ & $   0.00108 $ & $  11.87985 $ & $ i$\\
$ 55723.76135 $ & $   0.01403 $ & $   0.00108 $ & $  11.88016 $ & $ i$\\
$ 55723.76226 $ & $   0.01560 $ & $   0.00107 $ & $  11.88079 $ & $ i$\\
$ 55723.76300 $ & $   0.01294 $ & $   0.00107 $ & $  11.87660 $ & $ i$\\
$ 55723.76388 $ & $   0.01356 $ & $   0.00107 $ & $  11.87805 $ & $ i$\\
$ 55723.76460 $ & $   0.01576 $ & $   0.00107 $ & $  11.88020 $ & $ i$\\
$ 55723.76553 $ & $   0.01571 $ & $   0.00107 $ & $  11.87992 $ & $ i$\\
$ 55723.76627 $ & $   0.01424 $ & $   0.00107 $ & $  11.88076 $ & $ i$\\
$ 55723.76718 $ & $   0.01288 $ & $   0.00107 $ & $  11.87725 $ & $ i$\\
$ 55723.76792 $ & $   0.01922 $ & $   0.00109 $ & $  11.88599 $ & $ i$\\
$ 55723.76881 $ & $   0.01145 $ & $   0.00107 $ & $  11.87754 $ & $ i$\\
$ 55723.76960 $ & $   0.01372 $ & $   0.00107 $ & $  11.87739 $ & $ i$\\
$ 55723.77056 $ & $   0.01569 $ & $   0.00107 $ & $  11.87869 $ & $ i$\\
$ 55723.77135 $ & $   0.01441 $ & $   0.00108 $ & $  11.88030 $ & $ i$\\
$ 55723.77228 $ & $   0.01254 $ & $   0.00107 $ & $  11.87794 $ & $ i$\\
$ 55723.77300 $ & $   0.01666 $ & $   0.00107 $ & $  11.88291 $ & $ i$\\
$ 55723.77395 $ & $   0.01090 $ & $   0.00107 $ & $  11.87428 $ & $ i$\\
$ 55723.77468 $ & $   0.01256 $ & $   0.00107 $ & $  11.87686 $ & $ i$\\
$ 55723.77560 $ & $   0.01284 $ & $   0.00107 $ & $  11.87660 $ & $ i$\\
$ 55723.77633 $ & $   0.01351 $ & $   0.00107 $ & $  11.87872 $ & $ i$\\
$ 55723.77724 $ & $   0.01206 $ & $   0.00107 $ & $  11.87691 $ & $ i$\\
$ 55723.77796 $ & $   0.01158 $ & $   0.00107 $ & $  11.87439 $ & $ i$\\
$ 55723.77883 $ & $   0.01430 $ & $   0.00108 $ & $  11.87980 $ & $ i$\\
$ 55723.77956 $ & $   0.01054 $ & $   0.00107 $ & $  11.87306 $ & $ i$\\
$ 55723.78045 $ & $   0.01334 $ & $   0.00108 $ & $  11.87860 $ & $ i$\\
$ 55723.78119 $ & $   0.01176 $ & $   0.00108 $ & $  11.87760 $ & $ i$\\
$ 55723.78213 $ & $   0.01313 $ & $   0.00107 $ & $  11.87777 $ & $ i$\\
$ 55723.78286 $ & $   0.01519 $ & $   0.00108 $ & $  11.87880 $ & $ i$\\
$ 55723.78377 $ & $   0.01062 $ & $   0.00107 $ & $  11.87591 $ & $ i$\\
$ 55723.78449 $ & $   0.01432 $ & $   0.00108 $ & $  11.88078 $ & $ i$\\
$ 55723.78539 $ & $   0.01273 $ & $   0.00108 $ & $  11.87966 $ & $ i$\\
$ 55723.78612 $ & $   0.01168 $ & $   0.00108 $ & $  11.87767 $ & $ i$\\
$ 55723.78703 $ & $   0.00807 $ & $   0.00107 $ & $  11.87254 $ & $ i$\\
$ 55723.78777 $ & $   0.00512 $ & $   0.00107 $ & $  11.87076 $ & $ i$\\
$ 55723.78868 $ & $   0.00790 $ & $   0.00107 $ & $  11.87292 $ & $ i$\\
$ 55723.78942 $ & $   0.00411 $ & $   0.00106 $ & $  11.87187 $ & $ i$\\
$ 55723.79034 $ & $   0.00648 $ & $   0.00107 $ & $  11.87202 $ & $ i$\\
$ 55723.79108 $ & $   0.00927 $ & $   0.00108 $ & $  11.87638 $ & $ i$\\
$ 55723.79200 $ & $   0.00780 $ & $   0.00107 $ & $  11.87361 $ & $ i$\\
$ 55723.79276 $ & $  -0.00094 $ & $   0.00106 $ & $  11.86695 $ & $ i$\\
$ 55723.79367 $ & $   0.00421 $ & $   0.00107 $ & $  11.87032 $ & $ i$\\
$ 55723.79441 $ & $   0.00291 $ & $   0.00107 $ & $  11.86796 $ & $ i$\\
$ 55723.79531 $ & $   0.00335 $ & $   0.00107 $ & $  11.86961 $ & $ i$\\
$ 55723.79603 $ & $   0.00267 $ & $   0.00107 $ & $  11.87148 $ & $ i$\\
$ 55723.79693 $ & $   0.00233 $ & $   0.00107 $ & $  11.87016 $ & $ i$\\
$ 55723.79766 $ & $   0.00225 $ & $   0.00107 $ & $  11.86904 $ & $ i$\\
$ 55723.79860 $ & $   0.00291 $ & $   0.00108 $ & $  11.87140 $ & $ i$\\
$ 55723.79934 $ & $   0.00254 $ & $   0.00107 $ & $  11.87033 $ & $ i$\\
$ 55723.80024 $ & $  -0.00022 $ & $   0.00108 $ & $  11.86751 $ & $ i$\\
$ 55723.80097 $ & $  -0.00059 $ & $   0.00107 $ & $  11.86450 $ & $ i$\\
$ 55723.80186 $ & $  -0.00081 $ & $   0.00107 $ & $  11.86704 $ & $ i$\\
$ 55723.80260 $ & $  -0.00140 $ & $   0.00106 $ & $  11.86486 $ & $ i$\\
$ 55723.80348 $ & $  -0.00141 $ & $   0.00106 $ & $  11.86597 $ & $ i$\\
$ 55723.80422 $ & $   0.00064 $ & $   0.00107 $ & $  11.86756 $ & $ i$\\
$ 55723.80512 $ & $   0.00214 $ & $   0.00107 $ & $  11.86975 $ & $ i$\\
$ 55723.80585 $ & $  -0.00103 $ & $   0.00107 $ & $  11.86678 $ & $ i$\\
$ 55723.80680 $ & $   0.00135 $ & $   0.00106 $ & $  11.86802 $ & $ i$\\
$ 55723.80753 $ & $  -0.00173 $ & $   0.00107 $ & $  11.86623 $ & $ i$\\
$ 55723.80845 $ & $   0.00206 $ & $   0.00107 $ & $  11.86934 $ & $ i$\\
$ 55723.80917 $ & $  -0.00153 $ & $   0.00107 $ & $  11.86400 $ & $ i$\\
$ 55723.81007 $ & $   0.00007 $ & $   0.00107 $ & $  11.86595 $ & $ i$\\
$ 55723.81081 $ & $   0.00078 $ & $   0.00107 $ & $  11.86839 $ & $ i$\\
$ 55723.81171 $ & $  -0.00160 $ & $   0.00106 $ & $  11.86452 $ & $ i$\\
$ 55723.81245 $ & $  -0.00265 $ & $   0.00106 $ & $  11.86532 $ & $ i$\\
$ 55723.81411 $ & $  -0.00023 $ & $   0.00107 $ & $  11.86826 $ & $ i$\\
$ 55723.81502 $ & $   0.00240 $ & $   0.00107 $ & $  11.86938 $ & $ i$\\
$ 55723.81575 $ & $   0.00023 $ & $   0.00106 $ & $  11.86666 $ & $ i$\\
$ 55723.81666 $ & $  -0.00274 $ & $   0.00106 $ & $  11.86424 $ & $ i$\\
$ 55723.81740 $ & $   0.00018 $ & $   0.00107 $ & $  11.86934 $ & $ i$\\
$ 55723.81831 $ & $   0.00027 $ & $   0.00107 $ & $  11.86679 $ & $ i$\\
$ 55723.81905 $ & $   0.00025 $ & $   0.00107 $ & $  11.86681 $ & $ i$\\
$ 55723.81996 $ & $  -0.00015 $ & $   0.00107 $ & $  11.86819 $ & $ i$\\
$ 55723.82069 $ & $   0.00217 $ & $   0.00107 $ & $  11.86817 $ & $ i$\\
$ 55723.82161 $ & $   0.00147 $ & $   0.00107 $ & $  11.86944 $ & $ i$\\
$ 55723.82232 $ & $   0.00135 $ & $   0.00106 $ & $  11.86814 $ & $ i$\\
$ 55723.82325 $ & $  -0.00084 $ & $   0.00106 $ & $  11.86666 $ & $ i$\\
$ 55723.82399 $ & $   0.00063 $ & $   0.00107 $ & $  11.86798 $ & $ i$\\
$ 55723.82489 $ & $   0.00022 $ & $   0.00107 $ & $  11.86749 $ & $ i$\\
$ 55723.82561 $ & $  -0.00230 $ & $   0.00106 $ & $  11.86522 $ & $ i$\\
$ 55723.82651 $ & $  -0.00148 $ & $   0.00106 $ & $  11.86672 $ & $ i$\\
$ 55723.82725 $ & $  -0.00299 $ & $   0.00106 $ & $  11.86482 $ & $ i$\\
$ 55723.82816 $ & $  -0.00151 $ & $   0.00107 $ & $  11.86681 $ & $ i$\\
$ 55723.82890 $ & $  -0.00011 $ & $   0.00107 $ & $  11.86750 $ & $ i$\\
$ 55723.82978 $ & $   0.00018 $ & $   0.00106 $ & $  11.86905 $ & $ i$\\
$ 55723.83052 $ & $   0.00182 $ & $   0.00106 $ & $  11.86990 $ & $ i$\\
$ 55723.83142 $ & $  -0.00005 $ & $   0.00107 $ & $  11.86803 $ & $ i$\\
$ 55723.83216 $ & $  -0.00242 $ & $   0.00106 $ & $  11.86688 $ & $ i$\\
$ 55723.83308 $ & $   0.00055 $ & $   0.00106 $ & $  11.86978 $ & $ i$\\
$ 55723.83381 $ & $  -0.00209 $ & $   0.00106 $ & $  11.86661 $ & $ i$\\
$ 55723.83472 $ & $   0.00276 $ & $   0.00107 $ & $  11.87299 $ & $ i$\\
$ 55723.83544 $ & $   0.00245 $ & $   0.00107 $ & $  11.86905 $ & $ i$\\
$ 55723.83633 $ & $   0.00370 $ & $   0.00107 $ & $  11.87167 $ & $ i$\\
$ 55723.83706 $ & $  -0.00205 $ & $   0.00106 $ & $  11.86819 $ & $ i$\\
$ 55748.71705 $ & $   0.00968 $ & $   0.00087 $ & $  11.86738 $ & $ i$\\
$ 55748.71826 $ & $   0.01371 $ & $   0.00087 $ & $  11.87038 $ & $ i$\\
$ 55748.71945 $ & $   0.01488 $ & $   0.00087 $ & $  11.87518 $ & $ i$\\
$ 55748.72066 $ & $   0.01296 $ & $   0.00087 $ & $  11.87107 $ & $ i$\\
$ 55748.72186 $ & $   0.01783 $ & $   0.00088 $ & $  11.88019 $ & $ i$\\
$ 55748.72306 $ & $   0.01799 $ & $   0.00088 $ & $  11.87544 $ & $ i$\\
$ 55748.72787 $ & $   0.01729 $ & $   0.00088 $ & $  11.87457 $ & $ i$\\
$ 55748.72906 $ & $   0.01682 $ & $   0.00088 $ & $  11.87803 $ & $ i$\\
$ 55748.73028 $ & $   0.01374 $ & $   0.00087 $ & $  11.87124 $ & $ i$\\
$ 55748.73148 $ & $   0.01384 $ & $   0.00087 $ & $  11.86769 $ & $ i$\\
$ 55748.73268 $ & $   0.01396 $ & $   0.00088 $ & $  11.87375 $ & $ i$\\
$ 55748.73387 $ & $   0.01647 $ & $   0.00087 $ & $  11.87388 $ & $ i$\\
$ 55748.73507 $ & $   0.01690 $ & $   0.00088 $ & $  11.87418 $ & $ i$\\
$ 55748.73628 $ & $   0.01533 $ & $   0.00088 $ & $  11.87275 $ & $ i$\\
$ 55748.73747 $ & $   0.01524 $ & $   0.00087 $ & $  11.87171 $ & $ i$\\
$ 55748.73868 $ & $   0.01512 $ & $   0.00087 $ & $  11.87124 $ & $ i$\\
$ 55748.73986 $ & $   0.01689 $ & $   0.00087 $ & $  11.87282 $ & $ i$\\
$ 55748.74104 $ & $   0.01257 $ & $   0.00087 $ & $  11.87106 $ & $ i$\\
$ 55748.74224 $ & $   0.01274 $ & $   0.00087 $ & $  11.87031 $ & $ i$\\
$ 55748.74345 $ & $   0.00961 $ & $   0.00087 $ & $  11.86416 $ & $ i$\\
$ 55748.74465 $ & $   0.01425 $ & $   0.00088 $ & $  11.87121 $ & $ i$\\
$ 55748.74587 $ & $   0.01755 $ & $   0.00087 $ & $  11.87115 $ & $ i$\\
$ 55748.74708 $ & $   0.01418 $ & $   0.00087 $ & $  11.87013 $ & $ i$\\
$ 55748.74827 $ & $   0.01499 $ & $   0.00087 $ & $  11.87044 $ & $ i$\\
$ 55748.74946 $ & $   0.01371 $ & $   0.00088 $ & $  11.86967 $ & $ i$\\
$ 55748.75068 $ & $   0.01373 $ & $   0.00087 $ & $  11.86921 $ & $ i$\\
$ 55748.75188 $ & $   0.01324 $ & $   0.00087 $ & $  11.86768 $ & $ i$\\
$ 55748.75309 $ & $   0.01437 $ & $   0.00088 $ & $  11.87287 $ & $ i$\\
$ 55748.75429 $ & $   0.01575 $ & $   0.00087 $ & $  11.87093 $ & $ i$\\
$ 55748.75551 $ & $   0.01630 $ & $   0.00087 $ & $  11.87114 $ & $ i$\\
$ 55748.75670 $ & $   0.01473 $ & $   0.00087 $ & $  11.86865 $ & $ i$\\
$ 55748.75791 $ & $   0.01448 $ & $   0.00087 $ & $  11.87083 $ & $ i$\\
$ 55748.75912 $ & $   0.01329 $ & $   0.00088 $ & $  11.87203 $ & $ i$\\
$ 55748.76032 $ & $   0.01916 $ & $   0.00088 $ & $  11.87633 $ & $ i$\\
$ 55748.76152 $ & $   0.01651 $ & $   0.00088 $ & $  11.87316 $ & $ i$\\
$ 55748.76272 $ & $   0.01425 $ & $   0.00088 $ & $  11.87037 $ & $ i$\\
$ 55748.76393 $ & $   0.01377 $ & $   0.00087 $ & $  11.86739 $ & $ i$\\
$ 55748.76514 $ & $   0.01551 $ & $   0.00087 $ & $  11.87158 $ & $ i$\\
$ 55748.76633 $ & $   0.01505 $ & $   0.00087 $ & $  11.87317 $ & $ i$\\
$ 55748.76752 $ & $   0.01427 $ & $   0.00087 $ & $  11.86806 $ & $ i$\\
$ 55748.76872 $ & $   0.01791 $ & $   0.00087 $ & $  11.87492 $ & $ i$\\
$ 55748.76994 $ & $   0.01673 $ & $   0.00087 $ & $  11.86963 $ & $ i$\\
$ 55748.77114 $ & $   0.01471 $ & $   0.00087 $ & $  11.86990 $ & $ i$\\
$ 55748.77232 $ & $   0.01675 $ & $   0.00087 $ & $  11.87351 $ & $ i$\\
$ 55748.77353 $ & $   0.01298 $ & $   0.00087 $ & $  11.86820 $ & $ i$\\
$ 55748.77472 $ & $   0.01655 $ & $   0.00088 $ & $  11.87314 $ & $ i$\\
$ 55748.77592 $ & $   0.01542 $ & $   0.00087 $ & $  11.87113 $ & $ i$\\
$ 55748.77715 $ & $   0.01526 $ & $   0.00087 $ & $  11.87357 $ & $ i$\\
$ 55748.77834 $ & $   0.01583 $ & $   0.00087 $ & $  11.87123 $ & $ i$\\
$ 55748.77953 $ & $   0.01787 $ & $   0.00087 $ & $  11.87276 $ & $ i$\\
$ 55748.78075 $ & $   0.01596 $ & $   0.00087 $ & $  11.87208 $ & $ i$\\
$ 55748.78195 $ & $   0.01112 $ & $   0.00087 $ & $  11.86733 $ & $ i$\\
$ 55748.78317 $ & $   0.01536 $ & $   0.00088 $ & $  11.86968 $ & $ i$\\
$ 55748.78436 $ & $   0.01338 $ & $   0.00087 $ & $  11.87127 $ & $ i$\\
$ 55748.78555 $ & $   0.01281 $ & $   0.00087 $ & $  11.86797 $ & $ i$\\
$ 55748.78677 $ & $   0.01597 $ & $   0.00088 $ & $  11.87274 $ & $ i$\\
$ 55748.78795 $ & $   0.01402 $ & $   0.00087 $ & $  11.86996 $ & $ i$\\
$ 55748.78915 $ & $   0.01329 $ & $   0.00087 $ & $  11.86747 $ & $ i$\\
$ 55748.79036 $ & $   0.01069 $ & $   0.00086 $ & $  11.86582 $ & $ i$\\
$ 55748.79155 $ & $   0.01502 $ & $   0.00087 $ & $  11.87163 $ & $ i$\\
$ 55748.79277 $ & $   0.01319 $ & $   0.00087 $ & $  11.86866 $ & $ i$\\
$ 55748.79397 $ & $   0.01695 $ & $   0.00088 $ & $  11.87305 $ & $ i$\\
$ 55748.79517 $ & $   0.01382 $ & $   0.00087 $ & $  11.87179 $ & $ i$\\
$ 55748.79636 $ & $   0.01374 $ & $   0.00087 $ & $  11.86941 $ & $ i$\\
$ 55748.79754 $ & $   0.01242 $ & $   0.00087 $ & $  11.86834 $ & $ i$\\
$ 55748.79875 $ & $   0.01290 $ & $   0.00087 $ & $  11.86794 $ & $ i$\\
$ 55748.79994 $ & $   0.01393 $ & $   0.00087 $ & $  11.87131 $ & $ i$\\
$ 55748.80115 $ & $   0.01502 $ & $   0.00087 $ & $  11.86949 $ & $ i$\\
$ 55748.80236 $ & $   0.01757 $ & $   0.00087 $ & $  11.87341 $ & $ i$\\
$ 55748.80355 $ & $   0.01337 $ & $   0.00087 $ & $  11.87035 $ & $ i$\\
$ 55748.80475 $ & $   0.01500 $ & $   0.00088 $ & $  11.87263 $ & $ i$\\
$ 55748.80595 $ & $   0.01274 $ & $   0.00088 $ & $  11.86877 $ & $ i$\\
$ 55748.80717 $ & $   0.01287 $ & $   0.00087 $ & $  11.86833 $ & $ i$\\
$ 55748.80838 $ & $   0.01198 $ & $   0.00086 $ & $  11.86448 $ & $ i$\\
$ 55748.80958 $ & $   0.01454 $ & $   0.00087 $ & $  11.86896 $ & $ i$\\
$ 55748.81077 $ & $   0.01477 $ & $   0.00088 $ & $  11.87005 $ & $ i$\\
$ 55748.81199 $ & $   0.01479 $ & $   0.00088 $ & $  11.86992 $ & $ i$\\
$ 55748.81317 $ & $   0.01282 $ & $   0.00087 $ & $  11.86734 $ & $ i$\\
$ 55748.81437 $ & $   0.01228 $ & $   0.00088 $ & $  11.86808 $ & $ i$\\
$ 55748.81557 $ & $   0.01605 $ & $   0.00087 $ & $  11.87145 $ & $ i$\\
$ 55748.81678 $ & $   0.00878 $ & $   0.00087 $ & $  11.86432 $ & $ i$\\
$ 55748.81799 $ & $   0.01424 $ & $   0.00087 $ & $  11.87017 $ & $ i$\\
$ 55748.81919 $ & $   0.01160 $ & $   0.00087 $ & $  11.86853 $ & $ i$\\
$ 55748.82037 $ & $   0.00683 $ & $   0.00087 $ & $  11.86266 $ & $ i$\\
$ 55748.82158 $ & $   0.00897 $ & $   0.00087 $ & $  11.86502 $ & $ i$\\
$ 55748.82278 $ & $   0.00502 $ & $   0.00087 $ & $  11.86227 $ & $ i$\\
$ 55748.82399 $ & $   0.00432 $ & $   0.00087 $ & $  11.86092 $ & $ i$\\
$ 55748.82519 $ & $   0.00705 $ & $   0.00087 $ & $  11.86436 $ & $ i$\\
$ 55748.83724 $ & $  -0.00017 $ & $   0.00087 $ & $  11.86030 $ & $ i$\\
$ 55748.83844 $ & $  -0.00018 $ & $   0.00087 $ & $  11.85526 $ & $ i$\\
$ 55748.83964 $ & $   0.00227 $ & $   0.00087 $ & $  11.86161 $ & $ i$\\
$ 55748.84083 $ & $   0.00018 $ & $   0.00087 $ & $  11.85776 $ & $ i$\\
$ 55748.84204 $ & $  -0.00026 $ & $   0.00087 $ & $  11.85912 $ & $ i$\\
$ 55748.84325 $ & $   0.00096 $ & $   0.00087 $ & $  11.85784 $ & $ i$\\
$ 55748.84446 $ & $  -0.00054 $ & $   0.00087 $ & $  11.85837 $ & $ i$\\
$ 55748.84568 $ & $   0.00020 $ & $   0.00087 $ & $  11.85939 $ & $ i$\\
$ 55748.84704 $ & $  -0.00163 $ & $   0.00087 $ & $  11.85659 $ & $ i$\\
$ 55748.84844 $ & $  -0.00237 $ & $   0.00087 $ & $  11.85413 $ & $ i$\\
$ 55748.84964 $ & $  -0.00141 $ & $   0.00087 $ & $  11.85678 $ & $ i$\\
$ 56433.79947 $ & $  -0.01179 $ & $   0.00324 $ & $  12.66990 $ & $ g$\\
$ 56433.79998 $ & $   0.00171 $ & $   0.00327 $ & $  12.68340 $ & $ g$\\
$ 56433.80049 $ & $  -0.01009 $ & $   0.00322 $ & $  12.67160 $ & $ g$\\
$ 56433.80101 $ & $  -0.00529 $ & $   0.00321 $ & $  12.67640 $ & $ g$\\
$ 56433.80205 $ & $  -0.00389 $ & $   0.00321 $ & $  12.67780 $ & $ g$\\
$ 56433.80258 $ & $   0.00071 $ & $   0.00320 $ & $  12.68240 $ & $ g$\\
$ 56433.80306 $ & $   0.00191 $ & $   0.00323 $ & $  12.68360 $ & $ g$\\
$ 56433.80358 $ & $  -0.00309 $ & $   0.00319 $ & $  12.67860 $ & $ g$\\
$ 56433.80409 $ & $   0.00491 $ & $   0.00325 $ & $  12.68660 $ & $ g$\\
$ 56433.80520 $ & $   0.00361 $ & $   0.00323 $ & $  12.68530 $ & $ g$\\
$ 56433.80587 $ & $   0.00001 $ & $   0.00326 $ & $  12.68170 $ & $ g$\\
$ 56433.80710 $ & $   0.00111 $ & $   0.00317 $ & $  12.68280 $ & $ g$\\
$ 56433.80767 $ & $   0.00391 $ & $   0.00320 $ & $  12.68560 $ & $ g$\\
$ 56433.80826 $ & $   0.00271 $ & $   0.00320 $ & $  12.68440 $ & $ g$\\
$ 56433.80883 $ & $   0.00281 $ & $   0.00320 $ & $  12.68450 $ & $ g$\\
$ 56433.80940 $ & $   0.00971 $ & $   0.00320 $ & $  12.69140 $ & $ g$\\
$ 56433.81065 $ & $  -0.00319 $ & $   0.00314 $ & $  12.67850 $ & $ g$\\
$ 56433.81132 $ & $  -0.00009 $ & $   0.00317 $ & $  12.68160 $ & $ g$\\
$ 56433.81189 $ & $   0.00801 $ & $   0.00320 $ & $  12.68970 $ & $ g$\\
$ 56433.81245 $ & $  -0.00639 $ & $   0.00316 $ & $  12.67530 $ & $ g$\\
$ 56433.81300 $ & $  -0.01069 $ & $   0.00320 $ & $  12.67100 $ & $ g$\\
$ 56433.81414 $ & $  -0.00039 $ & $   0.00319 $ & $  12.68130 $ & $ g$\\
$ 56433.81472 $ & $  -0.00569 $ & $   0.00314 $ & $  12.67600 $ & $ g$\\
$ 56433.81531 $ & $   0.00631 $ & $   0.00318 $ & $  12.68800 $ & $ g$\\
$ 56433.81588 $ & $  -0.00909 $ & $   0.00318 $ & $  12.67260 $ & $ g$\\
$ 56433.81644 $ & $  -0.01099 $ & $   0.00317 $ & $  12.67070 $ & $ g$\\
$ 56433.81702 $ & $  -0.00609 $ & $   0.00313 $ & $  12.67560 $ & $ g$\\
$ 56433.81759 $ & $  -0.00359 $ & $   0.00318 $ & $  12.67810 $ & $ g$\\
$ 56433.81817 $ & $   0.00371 $ & $   0.00316 $ & $  12.68540 $ & $ g$\\
$ 56433.81875 $ & $   0.00011 $ & $   0.00320 $ & $  12.68180 $ & $ g$\\
$ 56433.81931 $ & $   0.00411 $ & $   0.00310 $ & $  12.68580 $ & $ g$\\
$ 56433.82045 $ & $  -0.00099 $ & $   0.00317 $ & $  12.68070 $ & $ g$\\
$ 56433.82157 $ & $  -0.00709 $ & $   0.00315 $ & $  12.67460 $ & $ g$\\
$ 56433.82349 $ & $   0.00371 $ & $   0.00313 $ & $  12.68540 $ & $ g$\\
$ 56433.82405 $ & $   0.00581 $ & $   0.00315 $ & $  12.68750 $ & $ g$\\
$ 56433.82520 $ & $  -0.00999 $ & $   0.00317 $ & $  12.67170 $ & $ g$\\
$ 56433.82577 $ & $  -0.00269 $ & $   0.00314 $ & $  12.67900 $ & $ g$\\
$ 56433.82634 $ & $  -0.00139 $ & $   0.00312 $ & $  12.68030 $ & $ g$\\
$ 56433.82691 $ & $  -0.00309 $ & $   0.00312 $ & $  12.67860 $ & $ g$\\
$ 56433.82751 $ & $   0.01771 $ & $   0.00309 $ & $  12.69940 $ & $ g$\\
$ 56433.82809 $ & $  -0.00259 $ & $   0.00315 $ & $  12.67910 $ & $ g$\\
$ 56433.82921 $ & $   0.00341 $ & $   0.00311 $ & $  12.68510 $ & $ g$\\
$ 56433.82978 $ & $  -0.00049 $ & $   0.00313 $ & $  12.68120 $ & $ g$\\
$ 56433.83042 $ & $  -0.00579 $ & $   0.00312 $ & $  12.67590 $ & $ g$\\
$ 56433.83102 $ & $  -0.00529 $ & $   0.00309 $ & $  12.67640 $ & $ g$\\
$ 56433.83158 $ & $  -0.00139 $ & $   0.00311 $ & $  12.68030 $ & $ g$\\
$ 56433.83216 $ & $   0.01011 $ & $   0.00313 $ & $  12.69180 $ & $ g$\\
$ 56433.83274 $ & $  -0.00509 $ & $   0.00311 $ & $  12.67660 $ & $ g$\\
$ 56433.83333 $ & $  -0.00909 $ & $   0.00314 $ & $  12.67260 $ & $ g$\\
$ 56433.83522 $ & $   0.00191 $ & $   0.00312 $ & $  12.68360 $ & $ g$\\
$ 56433.83581 $ & $   0.00511 $ & $   0.00309 $ & $  12.68680 $ & $ g$\\
$ 56433.83637 $ & $   0.00181 $ & $   0.00308 $ & $  12.68350 $ & $ g$\\
$ 56433.83693 $ & $   0.00751 $ & $   0.00309 $ & $  12.68920 $ & $ g$\\
$ 56433.83810 $ & $   0.00991 $ & $   0.00309 $ & $  12.69160 $ & $ g$\\
$ 56433.83869 $ & $  -0.00049 $ & $   0.00310 $ & $  12.68120 $ & $ g$\\
$ 56433.83927 $ & $  -0.00559 $ & $   0.00311 $ & $  12.67610 $ & $ g$\\
$ 56433.83983 $ & $   0.00301 $ & $   0.00312 $ & $  12.68470 $ & $ g$\\
$ 56433.84099 $ & $  -0.00219 $ & $   0.00312 $ & $  12.67950 $ & $ g$\\
$ 56433.84272 $ & $   0.00771 $ & $   0.00311 $ & $  12.68940 $ & $ g$\\
$ 56433.84328 $ & $  -0.00059 $ & $   0.00310 $ & $  12.68110 $ & $ g$\\
$ 56433.84385 $ & $  -0.00059 $ & $   0.00309 $ & $  12.68110 $ & $ g$\\
$ 56433.84441 $ & $   0.00231 $ & $   0.00307 $ & $  12.68400 $ & $ g$\\
$ 56433.84507 $ & $  -0.00879 $ & $   0.00310 $ & $  12.67290 $ & $ g$\\
$ 56433.84574 $ & $  -0.01059 $ & $   0.00308 $ & $  12.67110 $ & $ g$\\
$ 56433.84629 $ & $   0.00431 $ & $   0.00313 $ & $  12.68600 $ & $ g$\\
$ 56433.84686 $ & $   0.00451 $ & $   0.00311 $ & $  12.68620 $ & $ g$\\
$ 56433.84745 $ & $   0.00541 $ & $   0.00312 $ & $  12.68710 $ & $ g$\\
$ 56433.84801 $ & $  -0.01139 $ & $   0.00310 $ & $  12.67030 $ & $ g$\\
$ 56433.84925 $ & $  -0.00489 $ & $   0.00315 $ & $  12.67680 $ & $ g$\\
$ 56433.84991 $ & $   0.00071 $ & $   0.00312 $ & $  12.68240 $ & $ g$\\
$ 56433.85050 $ & $  -0.00049 $ & $   0.00318 $ & $  12.68120 $ & $ g$\\
$ 56433.85105 $ & $   0.00011 $ & $   0.00314 $ & $  12.68180 $ & $ g$\\
$ 56433.85173 $ & $  -0.00629 $ & $   0.00309 $ & $  12.67540 $ & $ g$\\
$ 56433.85230 $ & $  -0.00019 $ & $   0.00309 $ & $  12.68150 $ & $ g$\\
$ 56433.85287 $ & $   0.00621 $ & $   0.00311 $ & $  12.68790 $ & $ g$\\
$ 56433.85346 $ & $  -0.00589 $ & $   0.00313 $ & $  12.67580 $ & $ g$\\
$ 56433.85404 $ & $  -0.00679 $ & $   0.00309 $ & $  12.67490 $ & $ g$\\
$ 56433.85462 $ & $   0.00371 $ & $   0.00310 $ & $  12.68540 $ & $ g$\\
$ 56433.85517 $ & $   0.00481 $ & $   0.00310 $ & $  12.68650 $ & $ g$\\
$ 56433.85574 $ & $   0.00181 $ & $   0.00312 $ & $  12.68350 $ & $ g$\\
$ 56433.85750 $ & $   0.00381 $ & $   0.00311 $ & $  12.68550 $ & $ g$\\
$ 56433.85867 $ & $  -0.01339 $ & $   0.00315 $ & $  12.66830 $ & $ g$\\
$ 56433.85923 $ & $  -0.00159 $ & $   0.00309 $ & $  12.68010 $ & $ g$\\
$ 56433.85979 $ & $   0.00931 $ & $   0.00312 $ & $  12.69100 $ & $ g$\\
$ 56433.86037 $ & $   0.01541 $ & $   0.00308 $ & $  12.69710 $ & $ g$\\
$ 56433.86148 $ & $   0.01271 $ & $   0.00313 $ & $  12.69440 $ & $ g$\\
$ 56433.86205 $ & $   0.00501 $ & $   0.00313 $ & $  12.68670 $ & $ g$\\
$ 56433.86263 $ & $   0.00031 $ & $   0.00313 $ & $  12.68200 $ & $ g$\\
$ 56433.86320 $ & $   0.00241 $ & $   0.00312 $ & $  12.68410 $ & $ g$\\
$ 56433.86378 $ & $   0.00731 $ & $   0.00313 $ & $  12.68900 $ & $ g$\\
$ 56433.86438 $ & $   0.00011 $ & $   0.00305 $ & $  12.68180 $ & $ g$\\
$ 56433.86504 $ & $   0.00041 $ & $   0.00313 $ & $  12.68210 $ & $ g$\\
$ 56433.86574 $ & $  -0.01799 $ & $   0.00306 $ & $  12.66370 $ & $ g$\\
$ 56433.86641 $ & $  -0.00879 $ & $   0.00309 $ & $  12.67290 $ & $ g$\\
$ 56433.86700 $ & $   0.00801 $ & $   0.00305 $ & $  12.68970 $ & $ g$\\
$ 56433.86874 $ & $  -0.00039 $ & $   0.00306 $ & $  12.68130 $ & $ g$\\
$ 56433.86930 $ & $  -0.00869 $ & $   0.00306 $ & $  12.67300 $ & $ g$\\
$ 56433.86988 $ & $  -0.00049 $ & $   0.00304 $ & $  12.68120 $ & $ g$\\
$ 56433.87045 $ & $   0.01321 $ & $   0.00304 $ & $  12.69490 $ & $ g$\\
$ 56433.87102 $ & $   0.00361 $ & $   0.00304 $ & $  12.68530 $ & $ g$\\
$ 56433.87158 $ & $   0.00211 $ & $   0.00305 $ & $  12.68380 $ & $ g$\\
$ 56433.87215 $ & $   0.00871 $ & $   0.00300 $ & $  12.69040 $ & $ g$\\
$ 56433.87281 $ & $   0.00821 $ & $   0.00300 $ & $  12.68990 $ & $ g$\\
$ 56433.87338 $ & $   0.01741 $ & $   0.00301 $ & $  12.69910 $ & $ g$\\
$ 56433.87452 $ & $  -0.00539 $ & $   0.00298 $ & $  12.67630 $ & $ g$\\
$ 56433.87509 $ & $  -0.00699 $ & $   0.00297 $ & $  12.67470 $ & $ g$\\
$ 56433.87569 $ & $   0.00141 $ & $   0.00296 $ & $  12.68310 $ & $ g$\\
$ 56433.87627 $ & $  -0.00689 $ & $   0.00297 $ & $  12.67480 $ & $ g$\\
$ 56433.87748 $ & $   0.02201 $ & $   0.00298 $ & $  12.70370 $ & $ g$\\
$ 56433.87803 $ & $  -0.00379 $ & $   0.00299 $ & $  12.67790 $ & $ g$\\
$ 56433.87860 $ & $   0.00081 $ & $   0.00297 $ & $  12.68250 $ & $ g$\\
$ 56433.87918 $ & $   0.00671 $ & $   0.00298 $ & $  12.68840 $ & $ g$\\
$ 56433.87977 $ & $   0.01101 $ & $   0.00298 $ & $  12.69270 $ & $ g$\\
$ 56433.88282 $ & $  -0.00089 $ & $   0.00297 $ & $  12.68080 $ & $ g$\\
$ 56433.88338 $ & $   0.00571 $ & $   0.00297 $ & $  12.68740 $ & $ g$\\
$ 56433.88406 $ & $   0.01941 $ & $   0.00299 $ & $  12.70110 $ & $ g$\\
$ 56433.88474 $ & $  -0.00199 $ & $   0.00300 $ & $  12.67970 $ & $ g$\\
$ 56433.88540 $ & $  -0.01279 $ & $   0.00296 $ & $  12.66890 $ & $ g$\\
$ 56433.88596 $ & $   0.00451 $ & $   0.00294 $ & $  12.68620 $ & $ g$\\
$ 56433.88651 $ & $  -0.00049 $ & $   0.00293 $ & $  12.68120 $ & $ g$\\
$ 56433.88708 $ & $  -0.01149 $ & $   0.00292 $ & $  12.67020 $ & $ g$\\
$ 56433.88766 $ & $   0.00351 $ & $   0.00292 $ & $  12.68520 $ & $ g$\\
$ 56433.88825 $ & $   0.01291 $ & $   0.00293 $ & $  12.69460 $ & $ g$\\
$ 56433.88882 $ & $   0.00401 $ & $   0.00295 $ & $  12.68570 $ & $ g$\\
$ 56433.88995 $ & $  -0.00709 $ & $   0.00292 $ & $  12.67460 $ & $ g$\\
$ 56433.89052 $ & $   0.01001 $ & $   0.00291 $ & $  12.69170 $ & $ g$\\
$ 56433.89109 $ & $  -0.00019 $ & $   0.00290 $ & $  12.68150 $ & $ g$\\
$ 56433.89220 $ & $   0.00011 $ & $   0.00290 $ & $  12.68180 $ & $ g$\\
$ 56433.89278 $ & $  -0.00309 $ & $   0.00290 $ & $  12.67860 $ & $ g$\\
$ 56433.89334 $ & $  -0.00399 $ & $   0.00288 $ & $  12.67770 $ & $ g$\\
$ 56433.89567 $ & $   0.00461 $ & $   0.00287 $ & $  12.68630 $ & $ g$\\
$ 56433.89624 $ & $  -0.00209 $ & $   0.00287 $ & $  12.67960 $ & $ g$\\
$ 56433.89681 $ & $   0.00281 $ & $   0.00286 $ & $  12.68450 $ & $ g$\\
$ 56433.89737 $ & $  -0.00739 $ & $   0.00286 $ & $  12.67430 $ & $ g$\\
$ 56433.89793 $ & $   0.00431 $ & $   0.00288 $ & $  12.68600 $ & $ g$\\
$ 56433.89848 $ & $   0.00021 $ & $   0.00284 $ & $  12.68190 $ & $ g$\\
$ 56433.89962 $ & $  -0.00969 $ & $   0.00287 $ & $  12.67200 $ & $ g$\\
$ 56433.90017 $ & $  -0.00579 $ & $   0.00286 $ & $  12.67590 $ & $ g$\\
$ 56433.90074 $ & $  -0.00789 $ & $   0.00287 $ & $  12.67380 $ & $ g$\\
$ 56433.90132 $ & $  -0.00739 $ & $   0.00287 $ & $  12.67430 $ & $ g$\\
$ 56433.90190 $ & $  -0.00019 $ & $   0.00285 $ & $  12.68150 $ & $ g$\\
$ 56433.90248 $ & $   0.00581 $ & $   0.00287 $ & $  12.68750 $ & $ g$\\
$ 56433.90312 $ & $  -0.00749 $ & $   0.00286 $ & $  12.67420 $ & $ g$\\
$ 56433.90435 $ & $  -0.00339 $ & $   0.00287 $ & $  12.67830 $ & $ g$\\
$ 56433.90500 $ & $   0.00751 $ & $   0.00286 $ & $  12.68920 $ & $ g$\\
$ 56433.90567 $ & $  -0.00209 $ & $   0.00286 $ & $  12.67960 $ & $ g$\\
$ 56433.90681 $ & $  -0.00469 $ & $   0.00286 $ & $  12.67700 $ & $ g$\\
$ 56433.90804 $ & $  -0.00529 $ & $   0.00285 $ & $  12.67640 $ & $ g$\\
$ 56433.90862 $ & $  -0.01009 $ & $   0.00284 $ & $  12.67160 $ & $ g$\\
$ 56433.90976 $ & $   0.00121 $ & $   0.00283 $ & $  12.68290 $ & $ g$\\
$ 56433.91035 $ & $   0.00661 $ & $   0.00283 $ & $  12.68830 $ & $ g$\\
$ 56433.91092 $ & $   0.00681 $ & $   0.00286 $ & $  12.68850 $ & $ g$\\
$ 56433.91206 $ & $   0.00091 $ & $   0.00283 $ & $  12.68260 $ & $ g$\\
$ 56433.91262 $ & $   0.00091 $ & $   0.00286 $ & $  12.68260 $ & $ g$\\
$ 56433.91318 $ & $   0.00021 $ & $   0.00283 $ & $  12.68190 $ & $ g$\\
$ 56433.91374 $ & $  -0.01119 $ & $   0.00284 $ & $  12.67050 $ & $ g$\\
$ 56433.91432 $ & $  -0.00309 $ & $   0.00283 $ & $  12.67860 $ & $ g$\\
$ 56433.91488 $ & $   0.00041 $ & $   0.00284 $ & $  12.68210 $ & $ g$\\
$ 56433.91603 $ & $  -0.00909 $ & $   0.00281 $ & $  12.67260 $ & $ g$\\
$ 56433.91659 $ & $  -0.00929 $ & $   0.00282 $ & $  12.67240 $ & $ g$\\
$ 56433.91725 $ & $  -0.00939 $ & $   0.00281 $ & $  12.67230 $ & $ g$\\
$ 56433.91906 $ & $  -0.00559 $ & $   0.00286 $ & $  12.67610 $ & $ g$\\
$ 56433.91964 $ & $   0.00261 $ & $   0.00288 $ & $  12.68430 $ & $ g$\\
$ 56433.92024 $ & $  -0.00079 $ & $   0.00286 $ & $  12.68090 $ & $ g$\\
$ 56433.92139 $ & $  -0.01319 $ & $   0.00282 $ & $  12.66850 $ & $ g$\\
$ 56433.92260 $ & $  -0.00279 $ & $   0.00285 $ & $  12.67890 $ & $ g$\\
$ 56433.92328 $ & $   0.00071 $ & $   0.00283 $ & $  12.68240 $ & $ g$\\
$ 56433.92440 $ & $   0.00321 $ & $   0.00285 $ & $  12.68490 $ & $ g$\\
$ 56433.92556 $ & $  -0.00739 $ & $   0.00283 $ & $  12.67430 $ & $ g$\\
$ 56433.92674 $ & $   0.01001 $ & $   0.00285 $ & $  12.69170 $ & $ g$\\
$ 56433.92742 $ & $  -0.00649 $ & $   0.00281 $ & $  12.67520 $ & $ g$\\
$ 56433.92866 $ & $   0.00821 $ & $   0.00282 $ & $  12.68990 $ & $ g$\\
$ 56433.92932 $ & $   0.00601 $ & $   0.00282 $ & $  12.68770 $ & $ g$\\
$ 56433.92999 $ & $  -0.01139 $ & $   0.00282 $ & $  12.67030 $ & $ g$\\
$ 56433.93055 $ & $  -0.00459 $ & $   0.00286 $ & $  12.67710 $ & $ g$\\
$ 56433.93283 $ & $  -0.00329 $ & $   0.00284 $ & $  12.67840 $ & $ g$\\
$ 56433.93340 $ & $   0.00361 $ & $   0.00286 $ & $  12.68530 $ & $ g$\\
$ 56433.93398 $ & $   0.00821 $ & $   0.00285 $ & $  12.68990 $ & $ g$\\
$ 56433.93455 $ & $  -0.00159 $ & $   0.00285 $ & $  12.68010 $ & $ g$\\
$ 56433.93512 $ & $  -0.00829 $ & $   0.00286 $ & $  12.67340 $ & $ g$\\
$ 56433.93568 $ & $   0.00031 $ & $   0.00284 $ & $  12.68200 $ & $ g$\\
$ 56433.93625 $ & $   0.00271 $ & $   0.00287 $ & $  12.68440 $ & $ g$\\
$ 56433.93737 $ & $   0.00491 $ & $   0.00284 $ & $  12.68660 $ & $ g$\\
$ 56433.93794 $ & $   0.00271 $ & $   0.00284 $ & $  12.68440 $ & $ g$\\
$ 56433.93908 $ & $  -0.01729 $ & $   0.00282 $ & $  12.66440 $ & $ g$\\
$ 56433.94023 $ & $   0.00711 $ & $   0.00283 $ & $  12.68880 $ & $ g$\\
$ 56433.94081 $ & $   0.00581 $ & $   0.00282 $ & $  12.68750 $ & $ g$\\
$ 56433.94138 $ & $   0.01071 $ & $   0.00284 $ & $  12.69240 $ & $ g$\\
$ 56433.94196 $ & $  -0.00489 $ & $   0.00282 $ & $  12.67680 $ & $ g$\\
$ 56433.94254 $ & $  -0.00069 $ & $   0.00283 $ & $  12.68100 $ & $ g$\\
$ 56433.94309 $ & $  -0.00519 $ & $   0.00282 $ & $  12.67650 $ & $ g$\\
$ 56433.94420 $ & $   0.01231 $ & $   0.00285 $ & $  12.69400 $ & $ g$\\
$ 56433.94477 $ & $   0.00511 $ & $   0.00286 $ & $  12.68680 $ & $ g$\\
$ 56433.94536 $ & $  -0.00029 $ & $   0.00284 $ & $  12.68140 $ & $ g$\\
$ 56433.94728 $ & $   0.00921 $ & $   0.00284 $ & $  12.69090 $ & $ g$\\
$ 56433.94783 $ & $   0.00811 $ & $   0.00285 $ & $  12.68980 $ & $ g$\\
$ 56433.94841 $ & $   0.00271 $ & $   0.00284 $ & $  12.68440 $ & $ g$\\
$ 56433.94897 $ & $   0.00921 $ & $   0.00285 $ & $  12.69090 $ & $ g$\\
$ 56433.94953 $ & $   0.01031 $ & $   0.00284 $ & $  12.69200 $ & $ g$\\
$ 56433.95011 $ & $   0.00951 $ & $   0.00285 $ & $  12.69120 $ & $ g$\\
$ 56433.95187 $ & $   0.00831 $ & $   0.00284 $ & $  12.69000 $ & $ g$\\
$ 56433.95243 $ & $   0.01181 $ & $   0.00284 $ & $  12.69350 $ & $ g$\\
$ 56433.95415 $ & $   0.01611 $ & $   0.00286 $ & $  12.69780 $ & $ g$\\
$ 56433.95472 $ & $   0.01941 $ & $   0.00285 $ & $  12.70110 $ & $ g$\\
$ 56433.95532 $ & $   0.00991 $ & $   0.00284 $ & $  12.69160 $ & $ g$\\
$ 56433.95587 $ & $   0.00811 $ & $   0.00285 $ & $  12.68980 $ & $ g$\\
$ 56433.95699 $ & $   0.01661 $ & $   0.00285 $ & $  12.69830 $ & $ g$\\
$ 56433.95758 $ & $   0.01571 $ & $   0.00286 $ & $  12.69740 $ & $ g$\\
$ 56433.95883 $ & $   0.01461 $ & $   0.00286 $ & $  12.69630 $ & $ g$\\
$ 56433.96065 $ & $   0.01111 $ & $   0.00284 $ & $  12.69280 $ & $ g$\\
$ 56433.96122 $ & $   0.01961 $ & $   0.00284 $ & $  12.70130 $ & $ g$\\
$ 56433.96177 $ & $   0.00401 $ & $   0.00285 $ & $  12.68570 $ & $ g$\\
$ 56433.96234 $ & $   0.01271 $ & $   0.00285 $ & $  12.69440 $ & $ g$\\
$ 56433.96301 $ & $   0.01771 $ & $   0.00286 $ & $  12.69940 $ & $ g$\\
$ 56433.96368 $ & $   0.02091 $ & $   0.00284 $ & $  12.70260 $ & $ g$\\
$ 56433.96718 $ & $   0.02011 $ & $   0.00287 $ & $  12.70180 $ & $ g$\\
$ 56433.96776 $ & $   0.01171 $ & $   0.00289 $ & $  12.69340 $ & $ g$\\
$ 56433.96889 $ & $   0.00571 $ & $   0.00293 $ & $  12.68740 $ & $ g$\\
$ 56433.97021 $ & $   0.01311 $ & $   0.00294 $ & $  12.69480 $ & $ g$\\
$ 56433.97078 $ & $   0.01051 $ & $   0.00292 $ & $  12.69220 $ & $ g$\\
$ 56433.97135 $ & $   0.02581 $ & $   0.00294 $ & $  12.70750 $ & $ g$\\
$ 56433.97191 $ & $   0.01381 $ & $   0.00297 $ & $  12.69550 $ & $ g$\\
$ 56433.97249 $ & $   0.01391 $ & $   0.00298 $ & $  12.69560 $ & $ g$\\
$ 56433.97315 $ & $   0.01241 $ & $   0.00300 $ & $  12.69410 $ & $ g$\\
$ 56433.97372 $ & $   0.02971 $ & $   0.00303 $ & $  12.71140 $ & $ g$\\
$ 56433.97602 $ & $   0.02351 $ & $   0.00312 $ & $  12.70520 $ & $ g$\\
$ 56433.97661 $ & $   0.01691 $ & $   0.00319 $ & $  12.69860 $ & $ g$\\
$ 56433.97826 $ & $   0.02291 $ & $   0.00335 $ & $  12.70460 $ & $ g$\\
$ 56433.97883 $ & $   0.03021 $ & $   0.00336 $ & $  12.71190 $ & $ g$\\


==> data/HTR433-003_phfu_tab_short.tex <==
$ 55654.89724 $ & $   0.01314 $ & $   0.00112 $ & $  11.34410 $ & $ i$\\
$ 55654.89809 $ & $   0.01315 $ & $   0.00112 $ & $  11.34380 $ & $ i$\\
$ 55654.89894 $ & $   0.01560 $ & $   0.00112 $ & $  11.34390 $ & $ i$\\
$ 55654.89981 $ & $   0.01522 $ & $   0.00112 $ & $  11.34580 $ & $ i$\\
$ 55654.90065 $ & $   0.01456 $ & $   0.00113 $ & $  11.34380 $ & $ i$\\
$ 55654.90152 $ & $   0.01758 $ & $   0.00112 $ & $  11.34740 $ & $ i$\\
$ 55654.90235 $ & $   0.01425 $ & $   0.00112 $ & $  11.34350 $ & $ i$\\
$ 55654.90322 $ & $   0.01632 $ & $   0.00112 $ & $  11.34700 $ & $ i$\\
$ 55654.90407 $ & $   0.01552 $ & $   0.00113 $ & $  11.34650 $ & $ i$\\
$ 55654.90491 $ & $   0.01267 $ & $   0.00112 $ & $  11.34330 $ & $ i$\\


==> data/HTR433-003_rvtable.tex <==
$ 1668.07265 $ & \nodata      & \nodata      & $   -16.03 $ & $     8.62 $ & $    0.1220 $ & $   0.213 $\\
$ 1696.93207 $ & $     5.66 $ & $     7.42 $ & $    21.27 $ & $     9.92 $ & $    0.1310 $ & $   0.436 $\\
$ 1697.91247 $ & \nodata      & \nodata      & $    25.71 $ & $     6.26 $ & $    0.1260 $ & $   0.750 $\\
$ 1697.92558 $ & $   123.23 $ & $     8.08 $ & $    18.73 $ & $    11.98 $ & $    0.1300 $ & $   0.754 $\\
$ 1698.91871 $ & $   -18.91 $ & $     7.81 $ & $    -1.89 $ & $    22.68 $ & $    0.1120 $ & $   0.071 $\\
$ 1699.90750 $ & $   -74.19 $ & $     6.89 $ & $    -2.21 $ & $    17.77 $ & $    0.1170 $ & $   0.387 $\\
$ 1701.10094 $ & $    97.43 $ & $     5.92 $ & $   -48.91 $ & $     8.94 $ & $    0.1040 $ & $   0.769 $\\
$ 1703.91095 $ & $    57.59 $ & $     6.41 $ & $   -18.46 $ & $    11.91 $ & $    0.1140 $ & $   0.667 $\\
$ 1705.88887 $ & $  -128.98 $ & $     6.28 $ & $    -8.37 $ & $     9.85 $ & $    0.1200 $ & $   0.299 $\\
$ 1706.88594 $ & $    69.84 $ & $     6.70 $ & $     4.78 $ & $     9.59 $ & $    0.1150 $ & $   0.617 $\\
$ 1853.73646 $ & $    28.34 $ & $     6.19 $ & \nodata      & \nodata      & \nodata      & $   0.550 $\\
$ 2020.03172 $ & $   124.79 $ & $     7.60 $ & \nodata      & \nodata      & \nodata      & $   0.696 $\\

